HAT-P-24b: An inflated hot-Jupiter on a 3.36d period transiting a hot, metal-poor star

We report the discovery of HAT-P-24b, a transiting extrasolar planet orbiting the moderately bright V=11.818 F8 dwarf star GSC 0774-01441, with a period P = 3.3552464 +/- 0.0000071 d, transit epoch Tc = 2455216.97669 +/- 0.00024 (BJD_UTC), and transit duration 3.653 +/- 0.025 hours. The host star has a mass of 1.191 +/- 0.042 Msun, radius of 1.317 +/- 0.068 Rsun, effective temperature 6373 +/- 80 K, and a low metallicity of [Fe/H] = -0.16 +/- 0.08. The planetary companion has a mass of 0.681 +/- 0.031 MJ, and radius of 1.243 +/- 0.072 RJ yielding a mean density of 0.439 +/- 0.069 g cm-3 . By repeating our global fits with different parameter sets, we have performed a critical investigation of the fitting techniques used for previous HAT planetary discoveries. We find that the system properties are robust against the choice of priors. The effects of fixed versus fitted limb darkening are also examined. HAT-P-24b probably maintains a small eccentricity of e = 0.052 +0.022 -0.017, which is accepted over the circular orbit model with false alarm probability 5.8%. In the absence of eccentricity pumping, this result suggests HAT-P-24b experiences less tidal dissipation than Jupiter. Due to relatively rapid stellar rotation, we estimate that HAT-P-24b should exhibit one of the largest known Rossiter-McLaughlin effect amplitudes for an exoplanet (deltaVRM ~ 95 m/s) and thus a precise measurement of the sky-projected spin-orbit alignment should be possible.

==> 10pt.rtx.tex <==
%%
%% This is file `10pt.rtx',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% revtex4.dtx  (with options: `10pt')
%% 
%% This file is part of the APS files in the REVTeX 4 distribution.
%% For the version number, search on the string 
%% Original version by David Carlisle
%% Modified by Arthur Ogawa (mailto:ogawa@teleport.com)
%% 
%% Copyright (c) 1999 The American Physical Society.
%% http://publish.aps.org/revtex4/
%% mailto:revtex4@aps.org
%% 
%% See the REVTeX 4 README file for restrictions and more information.
%% 
\ProvidesFile{10pt.rtx}
          [2001/08/03 v4.0 (http://publish.aps.org/revtex4/ for documentation)]%FileInfo
\def\normalsize{%
   \@setfontsize\normalsize\@xpt{11.5}%
   \abovedisplayskip 10\p@ \@plus2\p@ \@minus5\p@
   \belowdisplayskip \abovedisplayskip
   \abovedisplayshortskip  \abovedisplayskip
   \belowdisplayshortskip \abovedisplayskip
   \let\@listi\@listI
}%
\def\small{%
  \@setfontsize\small\@ixpt{10.5}%
  \abovedisplayskip 8.5\p@ \@plus3\p@ \@minus4\p@
  \belowdisplayskip \abovedisplayskip
  \abovedisplayshortskip \z@ \@plus2\p@
  \belowdisplayshortskip 4\p@ \@plus2\p@ \@minus2\p@
  \def\@listi{%
    \leftmargin\leftmargini
    \topsep 4\p@ \@plus2\p@ \@minus2\p@
    \parsep 2\p@ \@plus\p@ \@minus\p@
    \itemsep \parsep
  }%
}%
\def\footnotesize{%
  \@setfontsize\footnotesize\@viiipt{9.5pt}%
  \abovedisplayskip 6\p@ \@plus2\p@ \@minus4\p@
  \belowdisplayskip \abovedisplayskip
  \abovedisplayshortskip \z@ \@plus\p@
  \belowdisplayshortskip 3\p@ \@plus\p@ \@minus2\p@
  \def\@listi{%
    \leftmargin\leftmargini
    \topsep 3\p@ \@plus\p@ \@minus\p@
    \parsep 2\p@ \@plus\p@ \@minus\p@
    \itemsep \parsep
  }%
}%
\def\scriptsize{%
 \@setfontsize\scriptsize\@viipt\@viiipt
}%
\def\tiny{%
 \@setfontsize\tiny\@vpt\@vipt
}%
\def\large{%
 \@setfontsize\large\@xiipt{14pt}%
}%
\def\Large{%
 \@setfontsize\Large\@xivpt{18pt}%
}%
\def\LARGE{%
 \@setfontsize\LARGE\@xviipt{22pt}%
}%
\def\huge{%
 \@setfontsize\huge\@xxpt{25pt}%
}%
\def\Huge{%
 \@setfontsize\Huge\@xxvpt{30pt}%
}%
 \@ifxundefined\twoside@sw{\@booleanfalse\twoside@sw}{}%
 \twoside@sw{%
    \oddsidemargin  -20pt
    \evensidemargin -20pt
    \marginparwidth 107pt
 }{%
    \oddsidemargin  -.25in
    \evensidemargin -.25in
    \marginparwidth 30pt
 }%
\marginparsep 6pt
\topmargin -61pt
\headheight 25pt
\headsep 16pt
\topskip 10pt
\footskip 30pt
 \textheight = 56pc
\textwidth42.5pc
\columnsep 1.5pc
\columnseprule 0pt
\footnotesep 1pt
\skip\footins 39pt plus 4pt minus 2pt
\def\footnoterule{\kern-19pt\hrule width.5in\kern18.6pt\relax}%
\floatsep 12pt plus 2pt minus 2pt
\textfloatsep 20pt plus 2pt minus 4pt
\intextsep 12pt plus 2pt minus 2pt
\dblfloatsep 12pt plus 2pt minus 2pt
\dbltextfloatsep 20pt plus 2pt minus 4pt
\@fptop 0pt plus 1fil
\@fpsep 8pt plus 2fil
\@fpbot 0pt plus 1fil
\@dblfptop 0pt plus 1fil
\@dblfpsep 8pt plus 2fil
\@dblfpbot 0pt plus 1fil
\marginparpush 5pt
\parskip 0pt plus 1pt
\parindent 10pt
\emergencystretch8\p@
\partopsep 2pt plus 1pt minus 1pt
\leftmargini 25pt
\leftmarginii 22pt
\leftmarginiii 18.7pt
\leftmarginiv 17pt
\leftmarginv 10pt
\leftmarginvi 10pt
\def\@listI{%
  \leftmargin\leftmargini
  \parsep 4\p@ plus2\p@ minus\p@
  \topsep 8\p@ plus2\p@ minus4\p@
  \itemsep 4\p@ plus2\p@ minus\p@
}%
\labelsep 4pt
\def\@listii{%
  \leftmargin\leftmarginii
  \labelwidth\leftmarginii
  \advance\labelwidth-\labelsep
  \topsep 4\p@ plus2\p@ minus\p@
  \parsep 2\p@ plus\p@ minus\p@
  \itemsep \parsep
}%
\def\@listiii{%
  \leftmargin\leftmarginiii
  \labelwidth\leftmarginiii
  \advance\labelwidth-\labelsep
  \topsep 2\p@ plus\p@ minus\p@
  \parsep \z@
  \partopsep \p@ plus\z@ minus\p@
  \itemsep \topsep
}%
\def\@listiv{%
  \leftmargin\leftmarginiv
  \labelwidth\leftmarginiv
  \advance\labelwidth-\labelsep
}%
\def\@listv{%
  \leftmargin\leftmarginv
  \labelwidth\leftmarginv
  \advance\labelwidth-\labelsep
}%
\def\@listvi{%
  \leftmargin\leftmarginvi
  \labelwidth\leftmarginvi
  \advance\labelwidth-\labelsep
}%
\endinput
%%
%% End of file `10pt.rtx'.


==> aps.rtx.tex <==
%%
%% This is file `aps.rtx',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% revtex4.dtx  (with options: `aps')
%% 
%% This file is part of the APS files in the REVTeX 4 distribution.
%% For the version number, search on the string 
%% Original version by David Carlisle
%% Modified by Arthur Ogawa (mailto:ogawa@teleport.com)
%% 
%% Copyright (c) 1999 The American Physical Society.
%% http://publish.aps.org/revtex4/
%% mailto:revtex4@aps.org
%% 
%% See the REVTeX 4 README file for restrictions and more information.
%% 
\NeedsTeXFormat{LaTeX2e}[1996/12/01]
\ProvidesFile{aps.rtx}
          [2001/08/03 v4.0 (http://publish.aps.org/revtex4/ for documentation)]%FileInfo
\ifx\undefined\substyle@ext
 \def\@tempa{%
  \endinput
  \GenericWarning{I must be read in by REVTeX! (Bailing out)}%
 }%
 \expandafter\else
  \def\@tempa{}%
 \expandafter\fi\@tempa
\def\ao{Appl.\  Opt.\ }
\def\ap{Appl.\  Phys.\ }
\def\apl{Appl.\ Phys.\ Lett.\ }
\def\apj{Astrophys.\ J.\ }
\def\bell{Bell Syst.\ Tech.\ J.\ }
\def\jqe{IEEE J.\ Quantum Electron.\ }
\def\assp{IEEE Trans.\ Acoust.\ Speech Signal Process.\ }
\def\aprop{IEEE Trans.\ Antennas Propag.\ }
\def\mtt{IEEE Trans.\ Microwave Theory Tech.\ }
\def\iovs{Invest.\ Ophthalmol.\ Vis.\ Sci.\ }
\def\jcp{J.\ Chem.\ Phys.\ }
\def\jmo{J.\ Mod.\ Opt.\ }
\def\josa{J.\ Opt.\ Soc.\ Am.\ }
\def\josaa{J.\ Opt.\ Soc.\ Am.\ A }
\def\josab{J.\ Opt.\ Soc.\ Am.\ B }
\def\jpp{J.\ Phys.\ (Paris) }
\def\nat{Nature (London) }
\def\oc{Opt.\ Commun.\ }
\def\ol{Opt.\ Lett.\ }
\def\pl{Phys.\ Lett.\ }
\def\pra{Phys.\ Rev.\ A }
\def\prb{Phys.\ Rev.\ B }
\def\prc{Phys.\ Rev.\ C }
\def\prd{Phys.\ Rev.\ D }
\def\pre{Phys.\ Rev.\ E }
\def\prl{Phys.\ Rev.\ Lett.\ }
\def\rmp{Rev.\ Mod.\ Phys.\ }
\def\pspie{Proc.\ Soc.\ Photo-Opt.\ Instrum.\ Eng.\ }
\def\sjqe{Sov.\ J.\ Quantum Electron.\ }
\def\vr{Vision Res.\ }
\def\@fnsymbol#1{%
 \ensuremath{%
  \ifcase#1\or
   *\or                        \dagger                   \or
   \ddagger                \or \mathsection              \or
   \mathparagraph\or
   **\or                       \dagger\dagger            \or
   \ddagger\ddagger        \or \mathsection \mathsection \or
   \mathparagraph\mathparagraph\or
   *{*}*\ignorespaces      \or \dagger\dagger\dagger     \or
   \ddagger\ddagger\ddagger\or \mathsection \mathsection \mathsection \or
   \mathparagraph\mathparagraph\mathparagraph\or
  \else
   \@ctrerr
  \fi
 }%
}%
\renewenvironment{titlepage}{%
  \let\wastwocol@sw\twocolumn@sw
  \onecolumngrid
  \newpage
  \thispagestyle{titlepage}%
  \c@page\z@% article sets this to one not zero???
}{%
  \wastwocol@sw{\twocolumngrid}{\newpage}%
}%
\def\frontmatter@abstractheading{%
 \preprintsty@sw{%
  \begingroup
   \centering\large
   \abstractname
   \par
  \endgroup
 }{}%
}%
\def\frontmatter@abstractwidth{400\p@}%
\def\frontmatter@abstractfont{%
 \small
 \parindent1em\relax
 \adjust@abstractwidth
}%
\def\adjust@abstractwidth{%
 \dimen@\textwidth\advance\dimen@-\frontmatter@abstractwidth
 \divide\dimen@\tw@
 \galley@sw{%
  \advance\rightskip\tw@\dimen@
 }{%
  \advance\leftskip\dimen@
  \advance\rightskip\dimen@
 }%
}%
\appdef\class@documenthook{%
  \preprintsty@sw{%
   \@ifxundefined\titlepage@sw{\@booleantrue\titlepage@sw}{}%
   \def\frontmatter@abstractwidth{\textwidth}%
   \def\frontmatter@affiliationfont{\it}%
   \let\section\section@preprintsty
   \let\subsection\subsection@preprintsty
   \let\subsubsection\subsubsection@preprintsty
  }{}%
 }%
\def\frontmatter@authorformat{%
 \skip@\@flushglue
 \@flushglue\z@ plus.3\hsize\relax
 \centering
 \advance\baselineskip\p@
 \parskip11.5\p@\relax
 \@flushglue\skip@
}%
\def\frontmatter@above@affilgroup{%
}%
\def\frontmatter@above@affiliation@script{%
 \skip@\@flushglue
 \@flushglue\z@ plus.3\hsize\relax
 \centering
 \@flushglue\skip@
 \addvspace{3.5\p@}%
}%
\def\frontmatter@above@affiliation{%
 \preprintsty@sw{}{%
 }%
}%
\def\frontmatter@affiliationfont{%
 \small\it
}%
\def\frontmatter@collaboration@above{%
 \preprintsty@sw{%
 }{%
  \parskip1.5\p@\relax
 }%
}%
\@ifxundefined\groupauthors@sw{%
 \clo@groupedaddress
}{}%
\def\frontmatter@setup{%
 \normalfont
}%
\def\frontmatter@title@above{\addvspace{6\p@}}%
\def\frontmatter@title@format{\large\bfseries\centering\parskip\z@skip}%
\def\frontmatter@title@below{}%
\def\@author@parskip{3\p@}%
\def\frontmatter@makefnmark{%
 \@textsuperscript{%
  \normalfont\@thefnmark
 }%
}%
\def\frontmatter@authorbelow{%
\addvspace{3\p@}%
}%
\def\frontmatter@RRAP@format{%
  \small
  \centering
  \everypar{\hbox\bgroup(\@gobble@leavemode@uppercase}%
  \def\par{\@ifvmode{}{\unskip)\egroup\@@par}}%
}%
\def\punct@RRAP{;\egroup\ \hbox\bgroup}%
\def\@gobble@leavemode@uppercase#1#2{\expandafter\MakeTextUppercase}%
\def\frontmatter@PACS@format{%
   \addvspace{11\p@}%
   \footnotesize
   \adjust@abstractwidth
   \parindent\z@
   \parskip\z@skip
   \samepage
}%
\def\frontmatter@keys@format{%
   \footnotesize
   \adjust@abstractwidth
   \parindent\z@
   \samepage
}%
\def\ps@titlepage{%
  \def\@oddhead{%
   \hfill
   \produce@preprints\@preprint
  }%
  \let\@evenhead\@oddhead
  \def\@oddfoot{%
   \hb@xt@\z@{\byrevtex\hss}%
   \hfil
   \preprintsty@sw{\thepage}{}%
   \quad\checkindate
   \hfil
  }%
  \let\@evenfoot\@oddfoot
}%
\def\byrevtex{\byrevtex@sw{Typeset by REV\TeX}{}}%
\def\produce@preprints#1{%
 \preprint@sw{%
  \vtop to \z@{%
   \def\baselinestretch{1}%
   \small
   \let\preprint\preprint@count
   \count@\z@#1\@ifnum{\count@>\tw@}{%
    \hbox{%
     \let\preprint\preprint@hlist
     #1\setbox\z@\lastbox
    }%
   }{%
    \let\preprint\preprint@cr
    \halign{\hfil##\cr#1\crcr}%
    \par
    \vss
   }%
  }%
 }{}%
}%
\def\preprint@cr#1{#1\cr}%
\def\preprint@count#1{\advance\count@\@ne}%
\def\preprint@hlist#1{#1\hbox{, }}%
\def\@seccntformat#1{\csname the#1\endcsname.\quad}%
\def\@hang@from#1#2#3{#1#2#3}%
\def\section{%
  \@startsection
    {section}%
    {1}%
    {\z@}%
    {0.8cm \@plus1ex \@minus .2ex}%
    {0.5cm}%
    {%
      \normalfont\small\bfseries
      \centering
    }%
}%
\def\@hangfrom@section#1#2#3{\@hangfrom{#1#2}\MakeTextUppercase{#3}}%
\def\subsection{%
  \@startsection
    {subsection}%
    {2}%
    {\z@}%
    {.8cm \@plus1ex \@minus .2ex}%
    {.5cm}%
    {%
     \normalfont\small\bfseries
     \centering
    }%
}%
\def\subsubsection{%
  \@startsection
    {subsubsection}%
    {3}%
    {\z@}%
    {.8cm \@plus1ex \@minus .2ex}%
    {.5cm}%
    {%
     \normalfont\small\itshape
     \centering
    }%
}%
\def\paragraph{%
  \@startsection
    {paragraph}%
    {4}%
    {\parindent}%
    {\z@}%
    {-1em}%
    {\normalfont\normalsize\itshape}%
}%
\def\subparagraph{%
  \@startsection
    {subparagraph}%
    {5}%
    {\parindent}%
    {3.25ex \@plus1ex \@minus .2ex}%
    {-1em}%
    {\normalfont\normalsize\bfseries}%
}%
\def\section@preprintsty{%
  \@startsection
    {section}%
    {1}%
    {\z@}%
    {0.8cm \@plus1ex \@minus .2ex}%
    {0.5cm}%
    {%
      \normalfont\small\bfseries
    }%
}%
\def\subsection@preprintsty{%
  \@startsection
    {subsection}%
    {2}%
    {\z@}%
    {.8cm \@plus1ex \@minus .2ex}%
    {.5cm}%
    {%
     \normalfont\small\bfseries
    }%
}%
\def\subsubsection@preprintsty{%
  \@startsection
    {subsubsection}%
    {3}%
    {\z@}%
    {.8cm \@plus1ex \@minus .2ex}%
    {.5cm}%
    {%
     \normalfont\small\itshape
    }%
}%
 \@ifxundefined\frontmatter@footnote@produce{%
  \let\frontmatter@footnote@produce\frontmatter@footnote@produce@endnote
 }{}%
\def\@pnumwidth{1.55em}
\def\@tocrmarg {2.55em}
\def\@dotsep{4.5pt}
\setcounter{tocdepth}{3}
\def\tableofcontents{%
 \addtocontents{toc}{\string\tocdepth@munge}%
 \print@toc{toc}%
 \addtocontents{toc}{\string\tocdepth@restore}%
}%
\def\tocdepth@munge{%
  \let\l@section@saved\l@section
  \let\l@section\@gobble@tw@
}%
\def\@gobble@tw@#1#2{}%
\def\tocdepth@restore{%
  \let\l@section\l@section@saved
}%
\def\l@part#1#2{\addpenalty{\@secpenalty}%
 \begingroup
  \set@tocdim@pagenum{#2}%
  \parindent \z@
  \rightskip\tocleft@pagenum plus 1fil\relax
  \skip@\parfillskip\parfillskip\z@
  \addvspace{2.25em plus\p@}%
  \large \bf %
  \leavevmode\ignorespaces#1\unskip\nobreak\hskip\skip@
  \hb@xt@\rightskip{\hfil\unhbox\z@}\hskip-\rightskip\hskip\z@skip
  \par
  \nobreak %
 \endgroup
}%
\def\tocleft@{\z@}%
\def\tocdim@min{5\p@}%
\def\l@section{%
 \l@@sections{}{section}% Implicit #3#4
}%
\def\l@f@section{%
 \addpenalty{\@secpenalty}%
 \addvspace{1.0em plus\p@}%
 \bf
}%
\def\l@subsection{%
 \l@@sections{section}{subsection}% Implicit #3#4
}%
\def\l@subsubsection{%
 \l@@sections{subsection}{subsubsection}% Implicit #3#4
}%
\def\l@paragraph#1#2{}%
\def\l@subparagraph#1#2{}%
\let\toc@pre\toc@pre@auto
\let\toc@post\toc@post@auto
\def\listoffigures{\print@toc{lof}}%
\def\l@figure{\@dottedtocline{1}{1.5em}{2.3em}}
\def\listoftables{\print@toc{lot}}%
\let\l@table\l@figure
\appdef\class@documenthook{%
 \@ifxundefined\raggedcolumn@sw{\@booleantrue\raggedcolumn@sw}{}%
 \raggedcolumn@sw{\raggedbottom}{\flushbottom}%
}%
\def\tableft@skip@float{\z@ plus\hsize}%
\def\tabmid@skip@float{\@flushglue}%
\def\tabright@skip@float{\z@ plus\hsize}%
\def\array@row@pre@float{\hline\hline\noalign{\vskip\doublerulesep}}%
\def\array@row@pst@float{\noalign{\vskip\doublerulesep}\hline\hline}%
\def\@makefntext#1{%
 \def\baselinestretch{1}%
 \reset@font
 \footnotesize
 \leftskip1em
 \parindent1em
 \noindent\nobreak\hskip-\leftskip
 \hb@xt@\leftskip{%
  \Hy@raisedlink{\hyper@anchorstart{footnote@\the\c@footnote}\hyper@anchorend}%
  \hss\@makefnmark\
 }%
 #1%
 \par
}%
\prepdef\appendix{%
 \par
 \let\@hangfrom@section\@hangfrom@appendix
 \let\@hangfroms@section\@hangfroms@appendix
 \let\@sectioncntformat\@appendixcntformat
}%
\def\@hangfrom@appendix#1#2#3{%
 #1%
 \@if@empty{#2}{%
  \MakeTextUppercase{#3}%
 }{%
  #2\@if@empty{#3}{}{:\ \MakeTextUppercase{#3}}%
 }%
}%
\def\@hangfroms@appendix#1#2{%
 #1\MakeTextUppercase{#2}%
}%
\def\@appendixcntformat#1{\appendixname\ \csname the#1\endcsname}%
\def\appendixesname{APPENDICES}%
\def\appendixname{APPENDIX}%
 \bibpunct{[}{]}{,}{n}{}{,}%
 \def\bibsection{%
  \par
  \onecolumngrid@push
  \begingroup
   \baselineskip26\p@
   \bib@device{\textwidth}{245.5\p@}%
 \endgroup
  \nobreak\@nobreaktrue
  \addvspace{19\p@}%
  \par
  \onecolumngrid@pop
 }%
\def\bib@device#1#2{%
\hb@xt@#1{%
 \hfil
 \phantomsection
  \addcontentsline {toc}{section}{\protect\numberline{}\refname}%
 \hb@xt@#2{%
  \skip@\z@\@plus-1fil\relax
                        \leaders\hrule height.25 \p@ depth.25 \p@ \hskip\z@\@plus1fil
\hskip\skip@
\hskip\z@\@plus0.125fil\leaders\hrule height.375\p@ depth.375\p@ \hskip\z@\@plus0.75fil \hskip\z@\@plus0.125fil
\hskip\skip@
\hskip\z@\@plus0.25 fil\leaders\hrule height.5  \p@ depth.5  \p@ \hskip\z@\@plus0.5 fil \hskip\z@\@plus0.25 fil
\hskip\skip@
\hskip\z@\@plus0.375fil\leaders\hrule height.625\p@ depth.625\p@ \hskip\z@\@plus0.25fil \hskip\z@\@plus0.375fil
 }%
\hfil
}%
}%
\let\bibpreamble\@empty
\bibsep\z@\relax
\def\newblock{\ }%
 \def\bibfont{%
  \small
 }%
\newenvironment{theindex}{%
 \columnseprule \z@
 \columnsep 35\p@
 \c@secnumdepth-\maxdimen
 \onecolumngrid@push
 \section{\indexname}%
 \thispagestyle{plain}%
 \parindent\z@
 \parskip\z@ plus.3\p@\relax
 \let\item\@idxitem
 \onecolumngrid@pop
}{%
}%
\def\@idxitem{\par\hangindent 40\p@}
\def\subitem{\par\hangindent 40\p@ \hspace*{20\p@}}
\def\subsubitem{\par\hangindent 40\p@ \hspace*{30\p@}}
\def\indexspace{\par \vskip 10\p@ plus5\p@ minus3\p@\relax}
\def\journal@pra{pra}%
\def\journal@prb{prb}%
\def\journal@prc{prc}%
\def\journal@prd{prd}%
\def\journal@pre{pre}%
\def\journal@prl{prl}%
\def\journal@prstab{prstab}%
\def\journal@rmp{rmp}%
\@ifx{\@journal\journal@pra}{%
}{}%
\@ifx{\@journal\journal@prb}{%
 \@ifxundefined\bibnotes@sw{\@booleantrue\bibnotes@sw}{}%
 \bibpunct{}{}{,}{s}{}{\textsuperscript{,}}%
 \def\@onlinecite#1{\begingroup\let\@cite\NAT@citenum\citealp{#1}\endgroup}%
 \appdef\class@documenthook{%
  \@ifxundefined\place@bibnumber{%
   \let\place@bibnumber\place@bibnumber@sup
  }{}%
 }%
}{}%
\@ifx{\@journal\journal@prc}{%
}{}%
\@ifx{\@journal\journal@prd}{%
}{}%
\@ifx{\@journal\journal@pre}{%
}{}%
\@ifx{\@journal\journal@prl}{%
 \@ifxundefined\bibnotes@sw{\@booleantrue\bibnotes@sw}{}%
 \@booleanfalse\acknowledgments@sw
 \def\bibsection{%
  \par
  \begingroup
   \baselineskip26\p@
   \bib@device{\hsize}{72\p@}%
 \endgroup
  \nobreak\@nobreaktrue
  \addvspace{19\p@}%
 }%
 \@ifxundefined\lengthcheck@sw{\@booleanfalse\lengthcheck@sw}{}%
  \lengthcheck@sw{%
   \RequirePackage{times}%
  }{%
  }%
 \c@secnumdepth=-\maxdimen
 \appdef\set@typesize@hook{%
  \@ifnum{\@pointsize=10\relax}{%
   \lengthcheck@sw{%
    \def\large{%
     \@setfontsize\large{12.5}{14\p@}%
    }%
    \def\normalsize{%
     \@setfontsize\normalsize{10.5}\@xiipt
     \abovedisplayskip 6\p@ \@plus6\p@ \@minus5\p@
     \belowdisplayskip \abovedisplayskip
     \abovedisplayshortskip  \abovedisplayskip
     \belowdisplayshortskip \abovedisplayskip
     \let\@listi\@listI
    }%
    \def\small{%
     \@setfontsize\small{9.5}\@xipt
     \abovedisplayskip 5\p@ \@plus5\p@ \@minus4\p@
     \belowdisplayskip \abovedisplayskip
     \abovedisplayshortskip  \abovedisplayskip
     \belowdisplayshortskip \abovedisplayskip
     \let\@listi\@listI
    }%
    \DeclareMathSizes{12.5}{12.5}{9}{6}%
    \DeclareMathSizes{10.5}{10.5}{7.5}{5}%
    \DeclareMathSizes{9.5}{9.5}{7.0}{5}%
   }{%
    \def\normalsize{%
     \@setfontsize\normalsize\@xpt\@xiipt
     \abovedisplayskip 10\p@ \@plus2\p@ \@minus5\p@
     \belowdisplayskip \abovedisplayskip
     \abovedisplayshortskip  \abovedisplayskip
     \belowdisplayshortskip \abovedisplayskip
     \let\@listi\@listI
    }%
   }%
  }{}%
 }%
  \@ifnum{\@pointsize=10\relax}{%
   \textheight = 694.0\p@
  }{}%
}{}%
\@ifx{\@journal\journal@prstab}{%
}{}%
\@ifx{\@journal\journal@rmp}{\input{\@journal\substyle@ext}}{}%
\@ifxundefined\footinbib@sw{\@booleantrue\footinbib@sw}{}%
\appdef\class@documenthook{%
 \@ifxundefined\place@bibnumber{%
  \let\place@bibnumber\place@bibnumber@inl
 }{}%
 \@ifxundefined\@bibstyle{%
  \def\@bibstyle{apsrev}%
 }{}%
}%
\endinput
%%
%% End of file `aps.rtx'.


==> phfu_tab.tex <==
$ 55206.63289 $ & $  -0.00145 $ & $   0.00176 $ & $ i$\\
$ 55206.63724 $ & $   0.00220 $ & $   0.00181 $ & $ i$\\
$ 55206.63790 $ & $  -0.00278 $ & $   0.00173 $ & $ i$\\
$ 55206.64440 $ & $  -0.00213 $ & $   0.00174 $ & $ i$\\
$ 55206.64485 $ & $   0.00093 $ & $   0.00171 $ & $ i$\\
$ 55206.64548 $ & $  -0.00051 $ & $   0.00161 $ & $ i$\\
$ 55206.64594 $ & $   0.00535 $ & $   0.00161 $ & $ i$\\
$ 55206.64659 $ & $  -0.00391 $ & $   0.00141 $ & $ i$\\
$ 55206.64703 $ & $   0.00162 $ & $   0.00140 $ & $ i$\\
$ 55206.64767 $ & $  -0.00023 $ & $   0.00134 $ & $ i$\\
$ 55206.64813 $ & $   0.00046 $ & $   0.00136 $ & $ i$\\
$ 55206.64878 $ & $  -0.00166 $ & $   0.00135 $ & $ i$\\
$ 55206.64923 $ & $   0.00158 $ & $   0.00135 $ & $ i$\\
$ 55206.64985 $ & $  -0.00071 $ & $   0.00134 $ & $ i$\\
$ 55206.65030 $ & $   0.00200 $ & $   0.00137 $ & $ i$\\
$ 55206.65094 $ & $   0.00111 $ & $   0.00135 $ & $ i$\\
$ 55206.65139 $ & $  -0.00115 $ & $   0.00134 $ & $ i$\\
$ 55206.65206 $ & $  -0.00460 $ & $   0.00134 $ & $ i$\\
$ 55206.65253 $ & $   0.00106 $ & $   0.00134 $ & $ i$\\
$ 55206.65315 $ & $  -0.00252 $ & $   0.00134 $ & $ i$\\
$ 55206.65361 $ & $  -0.00263 $ & $   0.00133 $ & $ i$\\
$ 55206.65424 $ & $  -0.00108 $ & $   0.00133 $ & $ i$\\
$ 55206.65469 $ & $  -0.00119 $ & $   0.00136 $ & $ i$\\
$ 55206.65533 $ & $   0.00220 $ & $   0.00137 $ & $ i$\\
$ 55206.65579 $ & $  -0.00343 $ & $   0.00138 $ & $ i$\\
$ 55206.65644 $ & $   0.00155 $ & $   0.00144 $ & $ i$\\
$ 55206.65690 $ & $   0.00406 $ & $   0.00148 $ & $ i$\\
$ 55206.65756 $ & $   0.00578 $ & $   0.00146 $ & $ i$\\
$ 55206.65800 $ & $  -0.00268 $ & $   0.00146 $ & $ i$\\
$ 55206.65864 $ & $  -0.00107 $ & $   0.00147 $ & $ i$\\
$ 55206.65973 $ & $   0.00038 $ & $   0.00148 $ & $ i$\\
$ 55206.66018 $ & $   0.00085 $ & $   0.00146 $ & $ i$\\
$ 55206.66080 $ & $   0.00003 $ & $   0.00156 $ & $ i$\\
$ 55206.66125 $ & $  -0.00369 $ & $   0.00147 $ & $ i$\\
$ 55206.66189 $ & $   0.00081 $ & $   0.00154 $ & $ i$\\
$ 55206.66235 $ & $   0.00023 $ & $   0.00151 $ & $ i$\\
$ 55206.66301 $ & $   0.00220 $ & $   0.00146 $ & $ i$\\
$ 55206.66346 $ & $   0.00169 $ & $   0.00148 $ & $ i$\\
$ 55206.66410 $ & $  -0.00346 $ & $   0.00150 $ & $ i$\\
$ 55206.66455 $ & $  -0.00374 $ & $   0.00152 $ & $ i$\\
$ 55206.66519 $ & $   0.00261 $ & $   0.00155 $ & $ i$\\
$ 55206.66564 $ & $   0.00183 $ & $   0.00149 $ & $ i$\\
$ 55206.66627 $ & $   0.00251 $ & $   0.00146 $ & $ i$\\
$ 55206.66672 $ & $   0.00370 $ & $   0.00148 $ & $ i$\\
$ 55206.66735 $ & $   0.00130 $ & $   0.00148 $ & $ i$\\
$ 55206.66780 $ & $   0.00011 $ & $   0.00146 $ & $ i$\\
$ 55206.66846 $ & $   0.00316 $ & $   0.00152 $ & $ i$\\
$ 55206.66892 $ & $   0.00030 $ & $   0.00154 $ & $ i$\\
$ 55206.66956 $ & $  -0.00155 $ & $   0.00156 $ & $ i$\\
$ 55206.67002 $ & $   0.00061 $ & $   0.00156 $ & $ i$\\
$ 55206.67065 $ & $   0.00320 $ & $   0.00158 $ & $ i$\\
$ 55206.67109 $ & $  -0.00226 $ & $   0.00166 $ & $ i$\\
$ 55206.67175 $ & $  -0.00260 $ & $   0.00153 $ & $ i$\\
$ 55206.67220 $ & $  -0.00076 $ & $   0.00150 $ & $ i$\\
$ 55206.67283 $ & $   0.00307 $ & $   0.00150 $ & $ i$\\
$ 55206.67328 $ & $  -0.00619 $ & $   0.00159 $ & $ i$\\
$ 55206.67393 $ & $   0.00168 $ & $   0.00154 $ & $ i$\\
$ 55206.67438 $ & $  -0.00193 $ & $   0.00146 $ & $ i$\\
$ 55206.67500 $ & $  -0.00139 $ & $   0.00145 $ & $ i$\\
$ 55206.67545 $ & $   0.00030 $ & $   0.00144 $ & $ i$\\
$ 55206.67610 $ & $  -0.00019 $ & $   0.00142 $ & $ i$\\
$ 55206.67655 $ & $  -0.00338 $ & $   0.00141 $ & $ i$\\
$ 55206.67719 $ & $  -0.00146 $ & $   0.00141 $ & $ i$\\
$ 55206.67764 $ & $  -0.00358 $ & $   0.00139 $ & $ i$\\
$ 55206.67827 $ & $   0.00294 $ & $   0.00138 $ & $ i$\\
$ 55206.67873 $ & $  -0.00076 $ & $   0.00139 $ & $ i$\\
$ 55206.67939 $ & $   0.00076 $ & $   0.00139 $ & $ i$\\
$ 55206.67984 $ & $   0.00345 $ & $   0.00144 $ & $ i$\\
$ 55206.68048 $ & $  -0.00391 $ & $   0.00147 $ & $ i$\\
$ 55206.68093 $ & $   0.00310 $ & $   0.00148 $ & $ i$\\
$ 55206.68157 $ & $   0.00090 $ & $   0.00150 $ & $ i$\\
$ 55206.68202 $ & $   0.00212 $ & $   0.00149 $ & $ i$\\
$ 55206.68264 $ & $   0.00154 $ & $   0.00152 $ & $ i$\\
$ 55206.68309 $ & $   0.00130 $ & $   0.00156 $ & $ i$\\
$ 55206.68373 $ & $  -0.00466 $ & $   0.00158 $ & $ i$\\
$ 55206.68419 $ & $  -0.00298 $ & $   0.00153 $ & $ i$\\
$ 55206.68484 $ & $   0.00412 $ & $   0.00145 $ & $ i$\\
$ 55206.68530 $ & $  -0.00324 $ & $   0.00144 $ & $ i$\\
$ 55206.68595 $ & $  -0.00480 $ & $   0.00144 $ & $ i$\\
$ 55206.68640 $ & $   0.00075 $ & $   0.00144 $ & $ i$\\
$ 55206.68703 $ & $  -0.00137 $ & $   0.00146 $ & $ i$\\
$ 55206.68749 $ & $  -0.00018 $ & $   0.00154 $ & $ i$\\
$ 55206.68814 $ & $   0.00009 $ & $   0.00157 $ & $ i$\\
$ 55206.68858 $ & $   0.00144 $ & $   0.00155 $ & $ i$\\
$ 55206.68922 $ & $  -0.00044 $ & $   0.00149 $ & $ i$\\
$ 55206.68967 $ & $   0.00194 $ & $   0.00144 $ & $ i$\\
$ 55206.69033 $ & $  -0.00005 $ & $   0.00143 $ & $ i$\\
$ 55206.69077 $ & $  -0.00047 $ & $   0.00140 $ & $ i$\\
$ 55206.69140 $ & $  -0.00563 $ & $   0.00134 $ & $ i$\\
$ 55206.69186 $ & $   0.00071 $ & $   0.00133 $ & $ i$\\
$ 55206.69249 $ & $  -0.00157 $ & $   0.00132 $ & $ i$\\
$ 55206.69294 $ & $   0.00081 $ & $   0.00133 $ & $ i$\\
$ 55206.69359 $ & $  -0.00004 $ & $   0.00130 $ & $ i$\\
$ 55206.69404 $ & $   0.00056 $ & $   0.00130 $ & $ i$\\
$ 55206.69468 $ & $  -0.00011 $ & $   0.00130 $ & $ i$\\
$ 55206.69512 $ & $   0.00010 $ & $   0.00130 $ & $ i$\\
$ 55206.69579 $ & $   0.00247 $ & $   0.00130 $ & $ i$\\
$ 55206.69623 $ & $   0.00032 $ & $   0.00130 $ & $ i$\\
$ 55206.69688 $ & $   0.00097 $ & $   0.00131 $ & $ i$\\
$ 55206.69734 $ & $   0.00215 $ & $   0.00130 $ & $ i$\\
$ 55206.69798 $ & $   0.00389 $ & $   0.00131 $ & $ i$\\
$ 55206.69844 $ & $   0.00449 $ & $   0.00131 $ & $ i$\\
$ 55206.69907 $ & $   0.00251 $ & $   0.00132 $ & $ i$\\
$ 55206.69951 $ & $  -0.00112 $ & $   0.00133 $ & $ i$\\
$ 55206.70015 $ & $   0.00188 $ & $   0.00132 $ & $ i$\\
$ 55206.70059 $ & $  -0.00039 $ & $   0.00133 $ & $ i$\\
$ 55206.70125 $ & $  -0.00098 $ & $   0.00137 $ & $ i$\\
$ 55206.70170 $ & $  -0.00076 $ & $   0.00137 $ & $ i$\\
$ 55206.70233 $ & $   0.00052 $ & $   0.00137 $ & $ i$\\
$ 55206.70278 $ & $   0.00131 $ & $   0.00139 $ & $ i$\\
$ 55206.70343 $ & $  -0.00173 $ & $   0.00139 $ & $ i$\\
$ 55206.70388 $ & $   0.00324 $ & $   0.00142 $ & $ i$\\
$ 55206.70452 $ & $   0.00191 $ & $   0.00147 $ & $ i$\\
$ 55206.70497 $ & $  -0.00035 $ & $   0.00149 $ & $ i$\\
$ 55206.70562 $ & $   0.00347 $ & $   0.00154 $ & $ i$\\
$ 55206.70605 $ & $   0.00111 $ & $   0.00153 $ & $ i$\\
$ 55206.70670 $ & $  -0.00218 $ & $   0.00155 $ & $ i$\\
$ 55206.70716 $ & $   0.00387 $ & $   0.00154 $ & $ i$\\
$ 55206.70779 $ & $  -0.00029 $ & $   0.00153 $ & $ i$\\
$ 55206.70824 $ & $  -0.00036 $ & $   0.00150 $ & $ i$\\
$ 55206.70889 $ & $  -0.00216 $ & $   0.00153 $ & $ i$\\
$ 55206.70936 $ & $   0.00333 $ & $   0.00153 $ & $ i$\\
$ 55206.70998 $ & $  -0.00253 $ & $   0.00153 $ & $ i$\\
$ 55206.71042 $ & $  -0.00312 $ & $   0.00153 $ & $ i$\\
$ 55206.71103 $ & $   0.00068 $ & $   0.00154 $ & $ i$\\
$ 55206.71150 $ & $  -0.00014 $ & $   0.00157 $ & $ i$\\
$ 55206.71216 $ & $  -0.00161 $ & $   0.00161 $ & $ i$\\
$ 55206.71261 $ & $  -0.00023 $ & $   0.00171 $ & $ i$\\
$ 55206.71323 $ & $  -0.00451 $ & $   0.00164 $ & $ i$\\
$ 55206.71366 $ & $  -0.00053 $ & $   0.00173 $ & $ i$\\
$ 55206.71430 $ & $   0.00353 $ & $   0.00149 $ & $ i$\\
$ 55206.71475 $ & $  -0.00178 $ & $   0.00153 $ & $ i$\\
$ 55206.71537 $ & $  -0.00193 $ & $   0.00147 $ & $ i$\\
$ 55206.71583 $ & $  -0.00129 $ & $   0.00145 $ & $ i$\\
$ 55206.71646 $ & $   0.00063 $ & $   0.00135 $ & $ i$\\
$ 55206.71690 $ & $   0.00006 $ & $   0.00133 $ & $ i$\\
$ 55206.71756 $ & $   0.00251 $ & $   0.00135 $ & $ i$\\
$ 55206.71802 $ & $  -0.00103 $ & $   0.00137 $ & $ i$\\
$ 55206.71865 $ & $  -0.00239 $ & $   0.00132 $ & $ i$\\
$ 55206.71911 $ & $  -0.00376 $ & $   0.00133 $ & $ i$\\
$ 55206.71975 $ & $   0.00050 $ & $   0.00131 $ & $ i$\\
$ 55206.72020 $ & $   0.00315 $ & $   0.00132 $ & $ i$\\
$ 55206.72083 $ & $  -0.00112 $ & $   0.00134 $ & $ i$\\
$ 55206.72130 $ & $   0.00014 $ & $   0.00135 $ & $ i$\\
$ 55206.72194 $ & $   0.00057 $ & $   0.00133 $ & $ i$\\
$ 55206.72240 $ & $  -0.00052 $ & $   0.00135 $ & $ i$\\
$ 55206.72305 $ & $  -0.00251 $ & $   0.00134 $ & $ i$\\
$ 55206.72351 $ & $  -0.00180 $ & $   0.00134 $ & $ i$\\
$ 55206.72414 $ & $   0.00094 $ & $   0.00136 $ & $ i$\\
$ 55206.72459 $ & $   0.00099 $ & $   0.00135 $ & $ i$\\
$ 55206.72521 $ & $   0.00139 $ & $   0.00137 $ & $ i$\\
$ 55206.72567 $ & $   0.00086 $ & $   0.00136 $ & $ i$\\
$ 55206.72629 $ & $   0.00027 $ & $   0.00137 $ & $ i$\\
$ 55206.72675 $ & $   0.00168 $ & $   0.00137 $ & $ i$\\
$ 55206.72738 $ & $  -0.00144 $ & $   0.00136 $ & $ i$\\
$ 55206.72783 $ & $   0.00160 $ & $   0.00137 $ & $ i$\\
$ 55206.72849 $ & $   0.00180 $ & $   0.00139 $ & $ i$\\
$ 55206.72895 $ & $   0.00000 $ & $   0.00150 $ & $ i$\\
$ 55206.72956 $ & $  -0.00003 $ & $   0.00152 $ & $ i$\\
$ 55206.73002 $ & $  -0.00080 $ & $   0.00149 $ & $ i$\\
$ 55206.73064 $ & $   0.00267 $ & $   0.00154 $ & $ i$\\
$ 55206.73110 $ & $  -0.00287 $ & $   0.00154 $ & $ i$\\
$ 55206.73174 $ & $   0.00226 $ & $   0.00154 $ & $ i$\\
$ 55206.73218 $ & $  -0.00250 $ & $   0.00168 $ & $ i$\\
$ 55206.73283 $ & $  -0.00137 $ & $   0.00175 $ & $ i$\\
$ 55206.73328 $ & $   0.00052 $ & $   0.00169 $ & $ i$\\
$ 55206.73392 $ & $   0.00176 $ & $   0.00158 $ & $ i$\\
$ 55206.73437 $ & $  -0.00263 $ & $   0.00155 $ & $ i$\\
$ 55206.73500 $ & $   0.00349 $ & $   0.00147 $ & $ i$\\
$ 55206.73547 $ & $  -0.00090 $ & $   0.00146 $ & $ i$\\
$ 55206.73611 $ & $   0.00002 $ & $   0.00149 $ & $ i$\\
$ 55206.73654 $ & $   0.00488 $ & $   0.00153 $ & $ i$\\
$ 55206.73718 $ & $  -0.00217 $ & $   0.00147 $ & $ i$\\
$ 55206.73763 $ & $  -0.00250 $ & $   0.00144 $ & $ i$\\
$ 55206.73827 $ & $  -0.00639 $ & $   0.00148 $ & $ i$\\
$ 55206.73873 $ & $  -0.00363 $ & $   0.00154 $ & $ i$\\
$ 55206.73940 $ & $  -0.00130 $ & $   0.00140 $ & $ i$\\
$ 55206.73985 $ & $  -0.00035 $ & $   0.00136 $ & $ i$\\
$ 55206.74049 $ & $  -0.00167 $ & $   0.00133 $ & $ i$\\
$ 55206.74094 $ & $   0.00119 $ & $   0.00128 $ & $ i$\\
$ 55206.74160 $ & $   0.00262 $ & $   0.00130 $ & $ i$\\
$ 55206.74204 $ & $   0.00087 $ & $   0.00129 $ & $ i$\\
$ 55206.74270 $ & $  -0.00122 $ & $   0.00127 $ & $ i$\\
$ 55206.74317 $ & $  -0.00015 $ & $   0.00127 $ & $ i$\\
$ 55206.74379 $ & $  -0.00018 $ & $   0.00127 $ & $ i$\\
$ 55206.74424 $ & $   0.00286 $ & $   0.00126 $ & $ i$\\
$ 55206.74490 $ & $   0.00133 $ & $   0.00127 $ & $ i$\\
$ 55206.74534 $ & $  -0.00153 $ & $   0.00126 $ & $ i$\\
$ 55206.74596 $ & $   0.00247 $ & $   0.00127 $ & $ i$\\
$ 55206.74643 $ & $   0.00096 $ & $   0.00129 $ & $ i$\\
$ 55206.74704 $ & $   0.00110 $ & $   0.00131 $ & $ i$\\
$ 55206.74750 $ & $  -0.00252 $ & $   0.00132 $ & $ i$\\
$ 55206.74813 $ & $  -0.00288 $ & $   0.00129 $ & $ i$\\
$ 55206.74858 $ & $  -0.00114 $ & $   0.00129 $ & $ i$\\
$ 55206.74922 $ & $   0.00067 $ & $   0.00130 $ & $ i$\\
$ 55206.74967 $ & $  -0.00272 $ & $   0.00131 $ & $ i$\\
$ 55206.75032 $ & $  -0.00038 $ & $   0.00131 $ & $ i$\\
$ 55206.75074 $ & $   0.00258 $ & $   0.00131 $ & $ i$\\
$ 55206.75137 $ & $  -0.00184 $ & $   0.00133 $ & $ i$\\
$ 55206.75183 $ & $  -0.00103 $ & $   0.00133 $ & $ i$\\
$ 55206.75248 $ & $  -0.00129 $ & $   0.00134 $ & $ i$\\
$ 55206.75293 $ & $  -0.00284 $ & $   0.00135 $ & $ i$\\
$ 55206.75358 $ & $   0.00022 $ & $   0.00136 $ & $ i$\\
$ 55206.75403 $ & $  -0.00054 $ & $   0.00135 $ & $ i$\\
$ 55206.75468 $ & $   0.00474 $ & $   0.00136 $ & $ i$\\
$ 55206.75513 $ & $   0.00103 $ & $   0.00135 $ & $ i$\\
$ 55206.75580 $ & $   0.00277 $ & $   0.00134 $ & $ i$\\
$ 55206.75624 $ & $   0.00023 $ & $   0.00136 $ & $ i$\\
$ 55206.75688 $ & $  -0.00136 $ & $   0.00138 $ & $ i$\\
$ 55206.75732 $ & $  -0.00005 $ & $   0.00136 $ & $ i$\\
$ 55206.75797 $ & $   0.00155 $ & $   0.00137 $ & $ i$\\
$ 55206.75842 $ & $   0.00015 $ & $   0.00139 $ & $ i$\\
$ 55206.75904 $ & $  -0.00033 $ & $   0.00139 $ & $ i$\\
$ 55206.75949 $ & $  -0.00144 $ & $   0.00139 $ & $ i$\\
$ 55206.76012 $ & $   0.00150 $ & $   0.00138 $ & $ i$\\
$ 55206.76057 $ & $  -0.00195 $ & $   0.00136 $ & $ i$\\
$ 55206.76123 $ & $  -0.00171 $ & $   0.00135 $ & $ i$\\
$ 55206.76168 $ & $   0.00126 $ & $   0.00138 $ & $ i$\\
$ 55206.76232 $ & $  -0.00041 $ & $   0.00138 $ & $ i$\\
$ 55206.76277 $ & $   0.00038 $ & $   0.00138 $ & $ i$\\
$ 55206.76339 $ & $  -0.00185 $ & $   0.00137 $ & $ i$\\
$ 55206.76385 $ & $   0.00088 $ & $   0.00134 $ & $ i$\\
$ 55206.76448 $ & $   0.00213 $ & $   0.00132 $ & $ i$\\
$ 55206.76495 $ & $  -0.00174 $ & $   0.00132 $ & $ i$\\
$ 55206.76557 $ & $  -0.00078 $ & $   0.00131 $ & $ i$\\
$ 55206.76603 $ & $  -0.00032 $ & $   0.00131 $ & $ i$\\
$ 55206.76668 $ & $  -0.00094 $ & $   0.00135 $ & $ i$\\
$ 55206.76714 $ & $  -0.00004 $ & $   0.00137 $ & $ i$\\
$ 55206.76778 $ & $   0.00005 $ & $   0.00135 $ & $ i$\\
$ 55206.76824 $ & $  -0.00168 $ & $   0.00138 $ & $ i$\\
$ 55206.76887 $ & $   0.00041 $ & $   0.00132 $ & $ i$\\
$ 55206.76932 $ & $  -0.00024 $ & $   0.00130 $ & $ i$\\
$ 55206.76996 $ & $   0.00055 $ & $   0.00134 $ & $ i$\\
$ 55206.77041 $ & $   0.00164 $ & $   0.00131 $ & $ i$\\
$ 55206.77105 $ & $   0.00204 $ & $   0.00131 $ & $ i$\\
$ 55206.77147 $ & $  -0.00012 $ & $   0.00134 $ & $ i$\\
$ 55206.77213 $ & $   0.00032 $ & $   0.00127 $ & $ i$\\
$ 55206.77257 $ & $   0.00050 $ & $   0.00126 $ & $ i$\\
$ 55206.77320 $ & $   0.00138 $ & $   0.00126 $ & $ i$\\
$ 55206.77365 $ & $   0.00335 $ & $   0.00127 $ & $ i$\\
$ 55206.77427 $ & $   0.00110 $ & $   0.00126 $ & $ i$\\
$ 55206.77474 $ & $   0.00092 $ & $   0.00126 $ & $ i$\\
$ 55206.77539 $ & $   0.00004 $ & $   0.00126 $ & $ i$\\
$ 55206.77584 $ & $   0.00036 $ & $   0.00127 $ & $ i$\\
$ 55206.77646 $ & $   0.00061 $ & $   0.00128 $ & $ i$\\
$ 55206.77691 $ & $   0.00011 $ & $   0.00130 $ & $ i$\\
$ 55206.77756 $ & $  -0.00116 $ & $   0.00130 $ & $ i$\\
$ 55206.77801 $ & $   0.00236 $ & $   0.00131 $ & $ i$\\
$ 55206.77865 $ & $   0.00322 $ & $   0.00131 $ & $ i$\\
$ 55206.77911 $ & $  -0.00028 $ & $   0.00130 $ & $ i$\\
$ 55206.77974 $ & $   0.00072 $ & $   0.00127 $ & $ i$\\
$ 55206.78019 $ & $   0.00078 $ & $   0.00125 $ & $ i$\\
$ 55206.78081 $ & $   0.00228 $ & $   0.00124 $ & $ i$\\
$ 55206.78128 $ & $  -0.00347 $ & $   0.00124 $ & $ i$\\
$ 55206.78190 $ & $  -0.00067 $ & $   0.00123 $ & $ i$\\
$ 55206.78235 $ & $  -0.00118 $ & $   0.00123 $ & $ i$\\
$ 55206.78302 $ & $   0.00044 $ & $   0.00123 $ & $ i$\\
$ 55206.78345 $ & $  -0.00016 $ & $   0.00122 $ & $ i$\\
$ 55206.78409 $ & $  -0.00047 $ & $   0.00122 $ & $ i$\\
$ 55206.78454 $ & $   0.00011 $ & $   0.00122 $ & $ i$\\
$ 55206.78518 $ & $  -0.00368 $ & $   0.00122 $ & $ i$\\
$ 55206.78563 $ & $  -0.00033 $ & $   0.00122 $ & $ i$\\
$ 55206.78625 $ & $  -0.00073 $ & $   0.00122 $ & $ i$\\
$ 55206.78668 $ & $   0.00166 $ & $   0.00122 $ & $ i$\\
$ 55206.78732 $ & $   0.00147 $ & $   0.00122 $ & $ i$\\
$ 55206.78777 $ & $   0.00113 $ & $   0.00123 $ & $ i$\\
$ 55206.78843 $ & $   0.00103 $ & $   0.00123 $ & $ i$\\
$ 55206.78889 $ & $  -0.00044 $ & $   0.00123 $ & $ i$\\
$ 55206.78952 $ & $   0.00132 $ & $   0.00123 $ & $ i$\\
$ 55206.78997 $ & $   0.00110 $ & $   0.00123 $ & $ i$\\
$ 55206.79063 $ & $   0.00010 $ & $   0.00122 $ & $ i$\\
$ 55206.79107 $ & $  -0.00370 $ & $   0.00122 $ & $ i$\\
$ 55206.79170 $ & $  -0.00066 $ & $   0.00122 $ & $ i$\\
$ 55206.79216 $ & $   0.00124 $ & $   0.00122 $ & $ i$\\
$ 55206.79278 $ & $   0.00199 $ & $   0.00123 $ & $ i$\\
$ 55206.79324 $ & $   0.00387 $ & $   0.00123 $ & $ i$\\
$ 55206.79389 $ & $   0.00081 $ & $   0.00123 $ & $ i$\\
$ 55206.79436 $ & $  -0.00100 $ & $   0.00123 $ & $ i$\\
$ 55206.79500 $ & $  -0.00056 $ & $   0.00123 $ & $ i$\\
$ 55206.79548 $ & $   0.00124 $ & $   0.00123 $ & $ i$\\
$ 55206.79613 $ & $   0.00031 $ & $   0.00123 $ & $ i$\\
$ 55206.79658 $ & $  -0.00152 $ & $   0.00123 $ & $ i$\\
$ 55206.79720 $ & $  -0.00122 $ & $   0.00123 $ & $ i$\\
$ 55206.79765 $ & $   0.00170 $ & $   0.00124 $ & $ i$\\
$ 55206.79830 $ & $   0.00078 $ & $   0.00124 $ & $ i$\\
$ 55206.79874 $ & $  -0.00089 $ & $   0.00124 $ & $ i$\\
$ 55206.79941 $ & $   0.00186 $ & $   0.00125 $ & $ i$\\
$ 55206.79985 $ & $   0.00075 $ & $   0.00124 $ & $ i$\\
$ 55206.80049 $ & $  -0.00002 $ & $   0.00124 $ & $ i$\\
$ 55206.80094 $ & $  -0.00116 $ & $   0.00124 $ & $ i$\\
$ 55206.80159 $ & $   0.00076 $ & $   0.00123 $ & $ i$\\
$ 55206.80205 $ & $   0.00095 $ & $   0.00123 $ & $ i$\\
$ 55206.80269 $ & $   0.00051 $ & $   0.00122 $ & $ i$\\
$ 55206.80315 $ & $  -0.00063 $ & $   0.00122 $ & $ i$\\
$ 55206.80380 $ & $   0.00120 $ & $   0.00122 $ & $ i$\\
$ 55206.80426 $ & $  -0.00169 $ & $   0.00122 $ & $ i$\\
$ 55206.80491 $ & $  -0.00113 $ & $   0.00122 $ & $ i$\\
$ 55206.80535 $ & $   0.00006 $ & $   0.00123 $ & $ i$\\
$ 55206.80599 $ & $   0.00334 $ & $   0.00123 $ & $ i$\\
$ 55206.80640 $ & $  -0.00042 $ & $   0.00123 $ & $ i$\\
$ 55206.80704 $ & $  -0.00045 $ & $   0.00123 $ & $ i$\\
$ 55206.80747 $ & $   0.00159 $ & $   0.00124 $ & $ i$\\
$ 55206.80809 $ & $  -0.00196 $ & $   0.00124 $ & $ i$\\
$ 55206.80852 $ & $  -0.00320 $ & $   0.00123 $ & $ i$\\
$ 55206.80916 $ & $  -0.00085 $ & $   0.00123 $ & $ i$\\
$ 55206.80961 $ & $   0.00252 $ & $   0.00123 $ & $ i$\\
$ 55206.81027 $ & $  -0.00098 $ & $   0.00124 $ & $ i$\\
$ 55206.81070 $ & $  -0.00190 $ & $   0.00124 $ & $ i$\\
$ 55206.81133 $ & $  -0.00007 $ & $   0.00126 $ & $ i$\\
$ 55206.81179 $ & $   0.00023 $ & $   0.00127 $ & $ i$\\
$ 55206.81243 $ & $  -0.00136 $ & $   0.00127 $ & $ i$\\
$ 55206.81289 $ & $  -0.00135 $ & $   0.00126 $ & $ i$\\
$ 55206.81353 $ & $  -0.00016 $ & $   0.00128 $ & $ i$\\
$ 55206.81396 $ & $   0.00049 $ & $   0.00127 $ & $ i$\\
$ 55206.81461 $ & $  -0.00014 $ & $   0.00128 $ & $ i$\\
$ 55206.81506 $ & $   0.00029 $ & $   0.00130 $ & $ i$\\
$ 55206.81571 $ & $  -0.00062 $ & $   0.00131 $ & $ i$\\
$ 55206.81617 $ & $  -0.00123 $ & $   0.00132 $ & $ i$\\
$ 55206.81681 $ & $   0.00114 $ & $   0.00133 $ & $ i$\\
$ 55206.81727 $ & $  -0.00266 $ & $   0.00132 $ & $ i$\\
$ 55206.81790 $ & $   0.00086 $ & $   0.00130 $ & $ i$\\
$ 55206.81836 $ & $   0.00238 $ & $   0.00128 $ & $ i$\\
$ 55206.81897 $ & $   0.00044 $ & $   0.00131 $ & $ i$\\
$ 55206.81942 $ & $  -0.00097 $ & $   0.00133 $ & $ i$\\
$ 55206.82007 $ & $   0.00162 $ & $   0.00131 $ & $ i$\\
$ 55206.82051 $ & $   0.00211 $ & $   0.00133 $ & $ i$\\
$ 55206.82118 $ & $  -0.00262 $ & $   0.00128 $ & $ i$\\
$ 55206.82165 $ & $  -0.00095 $ & $   0.00129 $ & $ i$\\
$ 55206.82228 $ & $  -0.00148 $ & $   0.00134 $ & $ i$\\
$ 55206.82273 $ & $  -0.00233 $ & $   0.00133 $ & $ i$\\
$ 55206.82337 $ & $   0.00170 $ & $   0.00132 $ & $ i$\\
$ 55206.82381 $ & $  -0.00062 $ & $   0.00133 $ & $ i$\\
$ 55206.82445 $ & $  -0.00113 $ & $   0.00133 $ & $ i$\\
$ 55206.82489 $ & $   0.00079 $ & $   0.00134 $ & $ i$\\
$ 55206.82552 $ & $  -0.00344 $ & $   0.00137 $ & $ i$\\
$ 55206.82598 $ & $  -0.00214 $ & $   0.00141 $ & $ i$\\
$ 55206.82665 $ & $  -0.00162 $ & $   0.00146 $ & $ i$\\
$ 55206.82710 $ & $  -0.00019 $ & $   0.00142 $ & $ i$\\
$ 55206.82772 $ & $  -0.00074 $ & $   0.00143 $ & $ i$\\
$ 55206.82819 $ & $   0.00037 $ & $   0.00145 $ & $ i$\\
$ 55206.82881 $ & $   0.00273 $ & $   0.00148 $ & $ i$\\
$ 55206.82924 $ & $   0.00229 $ & $   0.00151 $ & $ i$\\
$ 55206.82986 $ & $   0.00054 $ & $   0.00146 $ & $ i$\\
$ 55206.83033 $ & $  -0.00152 $ & $   0.00147 $ & $ i$\\
$ 55206.83095 $ & $   0.00180 $ & $   0.00152 $ & $ i$\\
$ 55206.83138 $ & $  -0.00140 $ & $   0.00146 $ & $ i$\\
$ 55206.83204 $ & $   0.00068 $ & $   0.00143 $ & $ i$\\
$ 55206.83249 $ & $  -0.00177 $ & $   0.00144 $ & $ i$\\
$ 55206.83313 $ & $  -0.00253 $ & $   0.00146 $ & $ i$\\
$ 55206.83358 $ & $   0.00060 $ & $   0.00148 $ & $ i$\\
$ 55206.83420 $ & $  -0.00121 $ & $   0.00148 $ & $ i$\\
$ 55206.83466 $ & $  -0.00003 $ & $   0.00146 $ & $ i$\\
$ 55206.83528 $ & $  -0.00061 $ & $   0.00150 $ & $ i$\\
$ 55206.83574 $ & $  -0.00221 $ & $   0.00152 $ & $ i$\\
$ 55206.83638 $ & $   0.00092 $ & $   0.00148 $ & $ i$\\
$ 55206.83683 $ & $  -0.00082 $ & $   0.00146 $ & $ i$\\
$ 55206.83749 $ & $  -0.00058 $ & $   0.00143 $ & $ i$\\
$ 55206.83794 $ & $   0.00380 $ & $   0.00145 $ & $ i$\\
$ 55206.83859 $ & $   0.00358 $ & $   0.00144 $ & $ i$\\
$ 55206.83904 $ & $   0.00181 $ & $   0.00143 $ & $ i$\\
$ 55206.83968 $ & $   0.00375 $ & $   0.00149 $ & $ i$\\
$ 55206.84013 $ & $   0.00296 $ & $   0.00147 $ & $ i$\\
$ 55206.84077 $ & $   0.00169 $ & $   0.00151 $ & $ i$\\
$ 55206.84121 $ & $   0.00808 $ & $   0.00160 $ & $ i$\\
$ 55206.84184 $ & $   0.00644 $ & $   0.00148 $ & $ i$\\
$ 55206.84231 $ & $   0.00221 $ & $   0.00153 $ & $ i$\\
$ 55206.84295 $ & $   0.00323 $ & $   0.00152 $ & $ i$\\
$ 55206.84339 $ & $   0.00812 $ & $   0.00150 $ & $ i$\\
$ 55206.84405 $ & $   0.00350 $ & $   0.00146 $ & $ i$\\
$ 55206.84452 $ & $   0.00562 $ & $   0.00151 $ & $ i$\\
$ 55206.84517 $ & $   0.00902 $ & $   0.00157 $ & $ i$\\
$ 55206.84559 $ & $   0.00570 $ & $   0.00157 $ & $ i$\\
$ 55206.84624 $ & $   0.00875 $ & $   0.00153 $ & $ i$\\
$ 55206.84668 $ & $   0.01197 $ & $   0.00154 $ & $ i$\\
$ 55206.84733 $ & $   0.00830 $ & $   0.00150 $ & $ i$\\
$ 55206.84777 $ & $   0.01264 $ & $   0.00146 $ & $ i$\\
$ 55206.84842 $ & $   0.00905 $ & $   0.00143 $ & $ i$\\
$ 55206.84886 $ & $   0.01002 $ & $   0.00144 $ & $ i$\\
$ 55206.84949 $ & $   0.01105 $ & $   0.00140 $ & $ i$\\
$ 55206.84993 $ & $   0.01186 $ & $   0.00139 $ & $ i$\\
$ 55206.85056 $ & $   0.00965 $ & $   0.00139 $ & $ i$\\
$ 55206.85102 $ & $   0.00885 $ & $   0.00138 $ & $ i$\\
$ 55206.85165 $ & $   0.00843 $ & $   0.00136 $ & $ i$\\
$ 55206.85210 $ & $   0.01252 $ & $   0.00133 $ & $ i$\\
$ 55206.85272 $ & $   0.01006 $ & $   0.00132 $ & $ i$\\
$ 55206.85315 $ & $   0.01316 $ & $   0.00134 $ & $ i$\\
$ 55206.85381 $ & $   0.01053 $ & $   0.00135 $ & $ i$\\
$ 55206.85425 $ & $   0.01262 $ & $   0.00136 $ & $ i$\\
$ 55206.85488 $ & $   0.00925 $ & $   0.00134 $ & $ i$\\
$ 55206.85534 $ & $   0.00579 $ & $   0.00134 $ & $ i$\\
$ 55206.85602 $ & $   0.01047 $ & $   0.00135 $ & $ i$\\
$ 55206.85647 $ & $   0.00694 $ & $   0.00135 $ & $ i$\\
$ 55206.85717 $ & $   0.00919 $ & $   0.00137 $ & $ i$\\
$ 55206.85764 $ & $   0.00967 $ & $   0.00138 $ & $ i$\\
$ 55206.85827 $ & $   0.01172 $ & $   0.00140 $ & $ i$\\
$ 55206.85871 $ & $   0.00777 $ & $   0.00141 $ & $ i$\\
$ 55206.85936 $ & $   0.01137 $ & $   0.00139 $ & $ i$\\
$ 55206.85981 $ & $   0.01001 $ & $   0.00140 $ & $ i$\\
$ 55206.86045 $ & $   0.00859 $ & $   0.00140 $ & $ i$\\
$ 55206.86091 $ & $   0.00797 $ & $   0.00141 $ & $ i$\\
$ 55206.86153 $ & $   0.00929 $ & $   0.00143 $ & $ i$\\
$ 55206.86197 $ & $   0.00967 $ & $   0.00145 $ & $ i$\\
$ 55206.86262 $ & $   0.01069 $ & $   0.00144 $ & $ i$\\
$ 55206.86307 $ & $   0.01180 $ & $   0.00146 $ & $ i$\\
$ 55206.86370 $ & $   0.00973 $ & $   0.00141 $ & $ i$\\
$ 55206.86416 $ & $   0.01099 $ & $   0.00142 $ & $ i$\\
$ 55206.86481 $ & $   0.00784 $ & $   0.00142 $ & $ i$\\
$ 55206.86525 $ & $   0.00989 $ & $   0.00140 $ & $ i$\\
$ 55206.86589 $ & $   0.00851 $ & $   0.00143 $ & $ i$\\
$ 55206.86635 $ & $   0.01189 $ & $   0.00143 $ & $ i$\\
$ 55206.86698 $ & $   0.00685 $ & $   0.00140 $ & $ i$\\
$ 55206.86743 $ & $   0.01137 $ & $   0.00139 $ & $ i$\\
$ 55206.86807 $ & $   0.01115 $ & $   0.00137 $ & $ i$\\
$ 55206.86850 $ & $   0.01248 $ & $   0.00139 $ & $ i$\\
$ 55206.86914 $ & $   0.01190 $ & $   0.00141 $ & $ i$\\
$ 55206.86959 $ & $   0.01019 $ & $   0.00141 $ & $ i$\\
$ 55206.87025 $ & $   0.00921 $ & $   0.00145 $ & $ i$\\
$ 55206.87066 $ & $   0.01054 $ & $   0.00150 $ & $ i$\\
$ 55206.87130 $ & $   0.01124 $ & $   0.00153 $ & $ i$\\
$ 55206.87174 $ & $   0.00735 $ & $   0.00152 $ & $ i$\\
$ 55206.87238 $ & $   0.01180 $ & $   0.00148 $ & $ i$\\
$ 55206.87283 $ & $   0.01640 $ & $   0.00151 $ & $ i$\\
$ 55206.87346 $ & $   0.01129 $ & $   0.00146 $ & $ i$\\
$ 55206.87390 $ & $   0.00821 $ & $   0.00133 $ & $ i$\\
$ 55206.87456 $ & $   0.00994 $ & $   0.00132 $ & $ i$\\
$ 55206.87499 $ & $   0.00995 $ & $   0.00130 $ & $ i$\\
$ 55206.87565 $ & $   0.00932 $ & $   0.00129 $ & $ i$\\
$ 55206.87610 $ & $   0.01091 $ & $   0.00130 $ & $ i$\\
$ 55206.87675 $ & $   0.01085 $ & $   0.00131 $ & $ i$\\
$ 55206.87721 $ & $   0.01179 $ & $   0.00132 $ & $ i$\\
$ 55206.87784 $ & $   0.01364 $ & $   0.00133 $ & $ i$\\
$ 55206.87826 $ & $   0.01516 $ & $   0.00135 $ & $ i$\\
$ 55206.87892 $ & $   0.01122 $ & $   0.00141 $ & $ i$\\
$ 55206.87936 $ & $   0.01269 $ & $   0.00140 $ & $ i$\\
$ 55206.87999 $ & $   0.01170 $ & $   0.00145 $ & $ i$\\
$ 55206.88042 $ & $   0.01149 $ & $   0.00142 $ & $ i$\\
$ 55206.88108 $ & $   0.01420 $ & $   0.00141 $ & $ i$\\
$ 55206.88153 $ & $   0.01221 $ & $   0.00143 $ & $ i$\\
$ 55206.88218 $ & $   0.01345 $ & $   0.00144 $ & $ i$\\
$ 55206.88261 $ & $   0.01085 $ & $   0.00145 $ & $ i$\\
$ 55206.88326 $ & $   0.01132 $ & $   0.00154 $ & $ i$\\
$ 55206.88368 $ & $   0.01102 $ & $   0.00179 $ & $ i$\\
$ 55206.88432 $ & $   0.01090 $ & $   0.00176 $ & $ i$\\
$ 55206.88477 $ & $   0.01649 $ & $   0.00159 $ & $ i$\\
$ 55206.88541 $ & $   0.01036 $ & $   0.00162 $ & $ i$\\
$ 55206.88581 $ & $   0.00976 $ & $   0.00153 $ & $ i$\\
$ 55206.88648 $ & $   0.01123 $ & $   0.00152 $ & $ i$\\
$ 55206.88692 $ & $   0.01461 $ & $   0.00156 $ & $ i$\\
$ 55206.88757 $ & $   0.01508 $ & $   0.00161 $ & $ i$\\
$ 55206.88802 $ & $   0.01054 $ & $   0.00165 $ & $ i$\\
$ 55206.88866 $ & $   0.01351 $ & $   0.00164 $ & $ i$\\
$ 55206.88911 $ & $   0.00838 $ & $   0.00164 $ & $ i$\\
$ 55206.88975 $ & $   0.01243 $ & $   0.00172 $ & $ i$\\
$ 55206.89020 $ & $   0.01512 $ & $   0.00169 $ & $ i$\\
$ 55206.89084 $ & $   0.01355 $ & $   0.00175 $ & $ i$\\
$ 55206.89129 $ & $   0.01024 $ & $   0.00175 $ & $ i$\\
$ 55206.89785 $ & $   0.00823 $ & $   0.00178 $ & $ i$\\
$ 55206.89849 $ & $   0.00674 $ & $   0.00176 $ & $ i$\\
$ 55206.89893 $ & $   0.01276 $ & $   0.00173 $ & $ i$\\
$ 55206.89956 $ & $   0.00958 $ & $   0.00176 $ & $ i$\\
$ 55206.90003 $ & $   0.01039 $ & $   0.00176 $ & $ i$\\
$ 55206.90390 $ & $   0.00809 $ & $   0.00172 $ & $ i$\\
$ 55206.90434 $ & $   0.01120 $ & $   0.00170 $ & $ i$\\
$ 55206.90497 $ & $   0.01585 $ & $   0.00164 $ & $ i$\\
$ 55206.90541 $ & $   0.01482 $ & $   0.00165 $ & $ i$\\
$ 55206.90603 $ & $   0.01325 $ & $   0.00159 $ & $ i$\\
$ 55206.90646 $ & $   0.01129 $ & $   0.00157 $ & $ i$\\
$ 55206.90710 $ & $   0.01268 $ & $   0.00161 $ & $ i$\\
$ 55206.90754 $ & $   0.00752 $ & $   0.00167 $ & $ i$\\
$ 55206.90821 $ & $   0.00680 $ & $   0.00167 $ & $ i$\\
$ 55206.90864 $ & $   0.01467 $ & $   0.00163 $ & $ i$\\
$ 55206.90927 $ & $   0.00812 $ & $   0.00157 $ & $ i$\\
$ 55206.90974 $ & $   0.01199 $ & $   0.00161 $ & $ i$\\
$ 55206.91039 $ & $   0.01011 $ & $   0.00162 $ & $ i$\\
$ 55206.91081 $ & $   0.01448 $ & $   0.00163 $ & $ i$\\
$ 55206.91145 $ & $   0.00894 $ & $   0.00160 $ & $ i$\\
$ 55206.91189 $ & $   0.01243 $ & $   0.00158 $ & $ i$\\
$ 55206.91250 $ & $   0.00966 $ & $   0.00162 $ & $ i$\\
$ 55206.91293 $ & $   0.01149 $ & $   0.00166 $ & $ i$\\
$ 55206.91359 $ & $   0.01291 $ & $   0.00163 $ & $ i$\\
$ 55206.91402 $ & $   0.01324 $ & $   0.00161 $ & $ i$\\
$ 55206.91469 $ & $   0.01369 $ & $   0.00157 $ & $ i$\\
$ 55206.91513 $ & $   0.01129 $ & $   0.00165 $ & $ i$\\
$ 55206.91575 $ & $   0.00899 $ & $   0.00165 $ & $ i$\\
$ 55206.91619 $ & $   0.00937 $ & $   0.00160 $ & $ i$\\
$ 55206.91682 $ & $   0.00972 $ & $   0.00160 $ & $ i$\\
$ 55206.91725 $ & $   0.01278 $ & $   0.00158 $ & $ i$\\
$ 55206.91788 $ & $   0.01361 $ & $   0.00158 $ & $ i$\\
$ 55206.91834 $ & $   0.01386 $ & $   0.00155 $ & $ i$\\
$ 55206.91901 $ & $   0.01343 $ & $   0.00155 $ & $ i$\\
$ 55206.91946 $ & $   0.00885 $ & $   0.00154 $ & $ i$\\
$ 55206.92010 $ & $   0.01363 $ & $   0.00154 $ & $ i$\\
$ 55206.92053 $ & $   0.01689 $ & $   0.00149 $ & $ i$\\
$ 55206.92118 $ & $   0.01160 $ & $   0.00151 $ & $ i$\\
$ 55206.92163 $ & $   0.01217 $ & $   0.00150 $ & $ i$\\
$ 55206.92227 $ & $   0.01175 $ & $   0.00152 $ & $ i$\\
$ 55206.92272 $ & $   0.01206 $ & $   0.00151 $ & $ i$\\
$ 55206.92336 $ & $   0.01059 $ & $   0.00151 $ & $ i$\\
$ 55206.92380 $ & $   0.01161 $ & $   0.00152 $ & $ i$\\
$ 55206.92447 $ & $   0.01145 $ & $   0.00153 $ & $ i$\\
$ 55206.92492 $ & $   0.01140 $ & $   0.00156 $ & $ i$\\
$ 55206.92556 $ & $   0.00743 $ & $   0.00156 $ & $ i$\\
$ 55206.92602 $ & $   0.01200 $ & $   0.00153 $ & $ i$\\
$ 55206.92663 $ & $   0.01389 $ & $   0.00155 $ & $ i$\\
$ 55206.92710 $ & $   0.01302 $ & $   0.00155 $ & $ i$\\
$ 55206.92772 $ & $   0.00892 $ & $   0.00155 $ & $ i$\\
$ 55206.92817 $ & $   0.01084 $ & $   0.00161 $ & $ i$\\
$ 55206.92924 $ & $   0.01176 $ & $   0.00154 $ & $ i$\\
$ 55206.92989 $ & $   0.01078 $ & $   0.00151 $ & $ i$\\
$ 55206.93033 $ & $   0.01139 $ & $   0.00149 $ & $ i$\\
$ 55206.93097 $ & $   0.01136 $ & $   0.00148 $ & $ i$\\
$ 55206.93144 $ & $   0.01290 $ & $   0.00150 $ & $ i$\\
$ 55206.93207 $ & $   0.01230 $ & $   0.00147 $ & $ i$\\
$ 55206.93253 $ & $   0.01395 $ & $   0.00146 $ & $ i$\\
$ 55206.93316 $ & $   0.01214 $ & $   0.00146 $ & $ i$\\
$ 55206.93363 $ & $   0.01282 $ & $   0.00147 $ & $ i$\\
$ 55206.93426 $ & $   0.01332 $ & $   0.00147 $ & $ i$\\
$ 55206.93471 $ & $   0.01173 $ & $   0.00149 $ & $ i$\\
$ 55206.93540 $ & $   0.00912 $ & $   0.00154 $ & $ i$\\
$ 55206.93586 $ & $   0.01591 $ & $   0.00156 $ & $ i$\\
$ 55206.93650 $ & $   0.01024 $ & $   0.00160 $ & $ i$\\
$ 55206.93691 $ & $   0.00804 $ & $   0.00170 $ & $ i$\\
$ 55206.93757 $ & $   0.00715 $ & $   0.00170 $ & $ i$\\
$ 55206.93802 $ & $   0.01182 $ & $   0.00171 $ & $ i$\\
$ 55206.93865 $ & $   0.01117 $ & $   0.00178 $ & $ i$\\
$ 55213.61564 $ & $   0.00905 $ & $   0.00103 $ & $ i$\\
$ 55213.61626 $ & $   0.00783 $ & $   0.00103 $ & $ i$\\
$ 55213.61688 $ & $   0.00998 $ & $   0.00103 $ & $ i$\\
$ 55213.61810 $ & $   0.01010 $ & $   0.00103 $ & $ i$\\
$ 55213.61890 $ & $   0.01592 $ & $   0.00103 $ & $ i$\\
$ 55213.61951 $ & $   0.01021 $ & $   0.00103 $ & $ i$\\
$ 55213.62012 $ & $   0.01210 $ & $   0.00102 $ & $ i$\\
$ 55213.62074 $ & $   0.01505 $ & $   0.00102 $ & $ i$\\
$ 55213.62136 $ & $   0.01395 $ & $   0.00102 $ & $ i$\\
$ 55213.62216 $ & $   0.01276 $ & $   0.00102 $ & $ i$\\
$ 55213.62277 $ & $   0.01062 $ & $   0.00102 $ & $ i$\\
$ 55213.62339 $ & $   0.01507 $ & $   0.00102 $ & $ i$\\
$ 55213.62401 $ & $   0.01098 $ & $   0.00102 $ & $ i$\\
$ 55213.62464 $ & $   0.01089 $ & $   0.00102 $ & $ i$\\
$ 55213.62547 $ & $   0.01315 $ & $   0.00102 $ & $ i$\\
$ 55213.62608 $ & $   0.01359 $ & $   0.00102 $ & $ i$\\
$ 55213.62672 $ & $   0.01283 $ & $   0.00102 $ & $ i$\\
$ 55213.62735 $ & $   0.01181 $ & $   0.00102 $ & $ i$\\
$ 55213.62797 $ & $   0.01232 $ & $   0.00102 $ & $ i$\\
$ 55213.62876 $ & $   0.01235 $ & $   0.00101 $ & $ i$\\
$ 55213.62938 $ & $   0.01512 $ & $   0.00102 $ & $ i$\\
$ 55213.63001 $ & $   0.01170 $ & $   0.00102 $ & $ i$\\
$ 55213.63063 $ & $   0.00872 $ & $   0.00102 $ & $ i$\\
$ 55213.63127 $ & $   0.01102 $ & $   0.00102 $ & $ i$\\
$ 55213.63207 $ & $   0.01394 $ & $   0.00101 $ & $ i$\\
$ 55213.63268 $ & $   0.00958 $ & $   0.00102 $ & $ i$\\
$ 55213.63330 $ & $   0.01098 $ & $   0.00101 $ & $ i$\\
$ 55213.63392 $ & $   0.00978 $ & $   0.00101 $ & $ i$\\
$ 55213.63455 $ & $   0.01158 $ & $   0.00102 $ & $ i$\\
$ 55213.63537 $ & $   0.00819 $ & $   0.00101 $ & $ i$\\
$ 55213.63598 $ & $   0.01115 $ & $   0.00101 $ & $ i$\\
$ 55213.63658 $ & $   0.01618 $ & $   0.00101 $ & $ i$\\
$ 55213.63718 $ & $   0.01157 $ & $   0.00101 $ & $ i$\\
$ 55213.63780 $ & $   0.01380 $ & $   0.00101 $ & $ i$\\
$ 55213.63861 $ & $   0.01235 $ & $   0.00101 $ & $ i$\\
$ 55213.63923 $ & $   0.00971 $ & $   0.00101 $ & $ i$\\
$ 55213.63986 $ & $   0.00987 $ & $   0.00101 $ & $ i$\\
$ 55213.64048 $ & $   0.01040 $ & $   0.00101 $ & $ i$\\
$ 55213.64111 $ & $   0.01179 $ & $   0.00101 $ & $ i$\\
$ 55213.64191 $ & $   0.01120 $ & $   0.00100 $ & $ i$\\
$ 55213.64253 $ & $   0.01512 $ & $   0.00101 $ & $ i$\\
$ 55213.64314 $ & $   0.01068 $ & $   0.00101 $ & $ i$\\
$ 55213.64376 $ & $   0.01281 $ & $   0.00100 $ & $ i$\\
$ 55213.64438 $ & $   0.01399 $ & $   0.00101 $ & $ i$\\
$ 55213.64522 $ & $   0.01143 $ & $   0.00100 $ & $ i$\\
$ 55213.64583 $ & $   0.01080 $ & $   0.00100 $ & $ i$\\
$ 55213.64647 $ & $   0.01204 $ & $   0.00101 $ & $ i$\\
$ 55213.64709 $ & $   0.00984 $ & $   0.00100 $ & $ i$\\
$ 55213.64771 $ & $   0.01292 $ & $   0.00100 $ & $ i$\\
$ 55213.64852 $ & $   0.00876 $ & $   0.00100 $ & $ i$\\
$ 55213.64913 $ & $   0.00970 $ & $   0.00100 $ & $ i$\\
$ 55213.64974 $ & $   0.00968 $ & $   0.00100 $ & $ i$\\
$ 55213.65036 $ & $   0.01152 $ & $   0.00100 $ & $ i$\\
$ 55213.65099 $ & $   0.00833 $ & $   0.00100 $ & $ i$\\
$ 55213.65180 $ & $   0.01352 $ & $   0.00100 $ & $ i$\\
$ 55213.65243 $ & $   0.01289 $ & $   0.00100 $ & $ i$\\
$ 55213.65304 $ & $   0.01016 $ & $   0.00100 $ & $ i$\\
$ 55213.65367 $ & $   0.01005 $ & $   0.00100 $ & $ i$\\
$ 55213.65428 $ & $   0.00766 $ & $   0.00100 $ & $ i$\\
$ 55213.65509 $ & $   0.01081 $ & $   0.00101 $ & $ i$\\
$ 55213.65570 $ & $   0.01159 $ & $   0.00100 $ & $ i$\\
$ 55213.65630 $ & $   0.00893 $ & $   0.00100 $ & $ i$\\
$ 55213.65692 $ & $   0.00981 $ & $   0.00100 $ & $ i$\\
$ 55213.65754 $ & $   0.00898 $ & $   0.00100 $ & $ i$\\
$ 55213.65839 $ & $   0.00818 $ & $   0.00100 $ & $ i$\\
$ 55213.65900 $ & $   0.01257 $ & $   0.00100 $ & $ i$\\
$ 55213.65960 $ & $   0.01182 $ & $   0.00101 $ & $ i$\\
$ 55213.66022 $ & $   0.01061 $ & $   0.00100 $ & $ i$\\
$ 55213.66083 $ & $   0.01050 $ & $   0.00100 $ & $ i$\\
$ 55213.66163 $ & $   0.01016 $ & $   0.00100 $ & $ i$\\
$ 55213.66224 $ & $   0.01026 $ & $   0.00100 $ & $ i$\\
$ 55213.66286 $ & $   0.01155 $ & $   0.00100 $ & $ i$\\
$ 55213.66347 $ & $   0.01159 $ & $   0.00100 $ & $ i$\\
$ 55213.66409 $ & $   0.01150 $ & $   0.00100 $ & $ i$\\
$ 55213.66490 $ & $   0.01103 $ & $   0.00100 $ & $ i$\\
$ 55213.66553 $ & $   0.01195 $ & $   0.00101 $ & $ i$\\
$ 55213.66615 $ & $   0.01107 $ & $   0.00100 $ & $ i$\\
$ 55213.66676 $ & $   0.01176 $ & $   0.00100 $ & $ i$\\
$ 55213.66738 $ & $   0.01185 $ & $   0.00100 $ & $ i$\\
$ 55213.66825 $ & $   0.01241 $ & $   0.00100 $ & $ i$\\
$ 55213.66887 $ & $   0.00864 $ & $   0.00101 $ & $ i$\\
$ 55213.66949 $ & $   0.01422 $ & $   0.00101 $ & $ i$\\
$ 55213.67010 $ & $   0.01201 $ & $   0.00101 $ & $ i$\\
$ 55213.67071 $ & $   0.01332 $ & $   0.00101 $ & $ i$\\
$ 55213.67151 $ & $   0.01026 $ & $   0.00101 $ & $ i$\\
$ 55213.67214 $ & $   0.01039 $ & $   0.00101 $ & $ i$\\
$ 55213.67276 $ & $   0.00831 $ & $   0.00101 $ & $ i$\\
$ 55213.67339 $ & $   0.00951 $ & $   0.00103 $ & $ i$\\
$ 55213.67399 $ & $   0.00984 $ & $   0.00100 $ & $ i$\\
$ 55213.67479 $ & $   0.01076 $ & $   0.00104 $ & $ i$\\
$ 55213.67541 $ & $   0.00992 $ & $   0.00102 $ & $ i$\\
$ 55213.67604 $ & $   0.01189 $ & $   0.00101 $ & $ i$\\
$ 55213.67665 $ & $   0.00926 $ & $   0.00101 $ & $ i$\\
$ 55213.67728 $ & $   0.01056 $ & $   0.00100 $ & $ i$\\
$ 55213.67810 $ & $   0.01136 $ & $   0.00101 $ & $ i$\\
$ 55213.67872 $ & $   0.00741 $ & $   0.00101 $ & $ i$\\
$ 55213.67935 $ & $   0.01336 $ & $   0.00106 $ & $ i$\\
$ 55213.67996 $ & $   0.00957 $ & $   0.00101 $ & $ i$\\
$ 55213.68057 $ & $   0.01105 $ & $   0.00099 $ & $ i$\\
$ 55213.68140 $ & $   0.01048 $ & $   0.00100 $ & $ i$\\
$ 55213.68201 $ & $   0.01030 $ & $   0.00099 $ & $ i$\\
$ 55213.68263 $ & $   0.00558 $ & $   0.00100 $ & $ i$\\
$ 55213.68326 $ & $   0.00789 $ & $   0.00099 $ & $ i$\\
$ 55213.68388 $ & $   0.00899 $ & $   0.00100 $ & $ i$\\
$ 55213.68468 $ & $   0.00695 $ & $   0.00100 $ & $ i$\\
$ 55213.68530 $ & $   0.01099 $ & $   0.00100 $ & $ i$\\
$ 55213.68590 $ & $   0.00829 $ & $   0.00100 $ & $ i$\\
$ 55213.68651 $ & $   0.01063 $ & $   0.00099 $ & $ i$\\
$ 55213.68714 $ & $   0.00738 $ & $   0.00099 $ & $ i$\\
$ 55213.68795 $ & $   0.00531 $ & $   0.00099 $ & $ i$\\
$ 55213.68858 $ & $   0.00737 $ & $   0.00099 $ & $ i$\\
$ 55213.68920 $ & $   0.00535 $ & $   0.00099 $ & $ i$\\
$ 55213.68981 $ & $   0.00587 $ & $   0.00099 $ & $ i$\\
$ 55213.69044 $ & $   0.00124 $ & $   0.00099 $ & $ i$\\
$ 55213.69127 $ & $   0.00274 $ & $   0.00099 $ & $ i$\\
$ 55213.69188 $ & $   0.00439 $ & $   0.00099 $ & $ i$\\
$ 55213.69251 $ & $   0.00183 $ & $   0.00099 $ & $ i$\\
$ 55213.69312 $ & $  -0.00031 $ & $   0.00099 $ & $ i$\\
$ 55213.69373 $ & $   0.00016 $ & $   0.00099 $ & $ i$\\
$ 55213.69453 $ & $   0.00245 $ & $   0.00100 $ & $ i$\\
$ 55213.69515 $ & $   0.00213 $ & $   0.00101 $ & $ i$\\
$ 55213.69575 $ & $  -0.00001 $ & $   0.00106 $ & $ i$\\
$ 55213.70177 $ & $   0.00258 $ & $   0.00121 $ & $ i$\\
$ 55213.70239 $ & $  -0.00121 $ & $   0.00114 $ & $ i$\\
$ 55213.70302 $ & $  -0.00243 $ & $   0.00108 $ & $ i$\\
$ 55213.70365 $ & $  -0.00155 $ & $   0.00102 $ & $ i$\\
$ 55213.70447 $ & $  -0.00023 $ & $   0.00103 $ & $ i$\\
$ 55213.70510 $ & $   0.00127 $ & $   0.00106 $ & $ i$\\
$ 55213.70571 $ & $   0.00168 $ & $   0.00108 $ & $ i$\\
$ 55213.70633 $ & $  -0.00140 $ & $   0.00111 $ & $ i$\\
$ 55213.70773 $ & $   0.00078 $ & $   0.00113 $ & $ i$\\
$ 55213.71020 $ & $   0.00344 $ & $   0.00120 $ & $ i$\\
$ 55213.71290 $ & $   0.00037 $ & $   0.00123 $ & $ i$\\
$ 55213.71351 $ & $  -0.00023 $ & $   0.00123 $ & $ i$\\
$ 55213.71434 $ & $  -0.00001 $ & $   0.00119 $ & $ i$\\
$ 55213.71496 $ & $  -0.00115 $ & $   0.00119 $ & $ i$\\
$ 55213.71556 $ & $  -0.00049 $ & $   0.00107 $ & $ i$\\
$ 55213.71616 $ & $   0.00094 $ & $   0.00107 $ & $ i$\\
$ 55213.71680 $ & $   0.00115 $ & $   0.00102 $ & $ i$\\
$ 55213.71761 $ & $  -0.00037 $ & $   0.00102 $ & $ i$\\
$ 55213.71822 $ & $   0.00377 $ & $   0.00102 $ & $ i$\\
$ 55213.71885 $ & $   0.00138 $ & $   0.00106 $ & $ i$\\
$ 55213.71947 $ & $  -0.00213 $ & $   0.00106 $ & $ i$\\
$ 55213.72009 $ & $  -0.00006 $ & $   0.00114 $ & $ i$\\
$ 55213.72149 $ & $  -0.00166 $ & $   0.00115 $ & $ i$\\
$ 55213.72210 $ & $   0.00392 $ & $   0.00111 $ & $ i$\\
$ 55213.72273 $ & $   0.00237 $ & $   0.00110 $ & $ i$\\
$ 55213.72336 $ & $  -0.00037 $ & $   0.00104 $ & $ i$\\
$ 55213.72420 $ & $  -0.00171 $ & $   0.00111 $ & $ i$\\
$ 55213.72481 $ & $  -0.00241 $ & $   0.00114 $ & $ i$\\
$ 55213.72542 $ & $   0.00191 $ & $   0.00107 $ & $ i$\\
$ 55213.72604 $ & $  -0.00097 $ & $   0.00104 $ & $ i$\\
$ 55213.72665 $ & $   0.00189 $ & $   0.00106 $ & $ i$\\
$ 55213.72747 $ & $  -0.00201 $ & $   0.00106 $ & $ i$\\
$ 55213.72810 $ & $   0.00026 $ & $   0.00111 $ & $ i$\\
$ 55213.73794 $ & $  -0.00027 $ & $   0.00115 $ & $ i$\\
$ 55213.73855 $ & $  -0.00016 $ & $   0.00109 $ & $ i$\\
$ 55213.73919 $ & $  -0.00127 $ & $   0.00109 $ & $ i$\\
$ 55213.73980 $ & $  -0.00165 $ & $   0.00122 $ & $ i$\\
$ 55213.74061 $ & $   0.00048 $ & $   0.00108 $ & $ i$\\
$ 55213.74122 $ & $   0.00278 $ & $   0.00106 $ & $ i$\\
$ 55213.74184 $ & $   0.00225 $ & $   0.00103 $ & $ i$\\
$ 55213.74245 $ & $   0.00152 $ & $   0.00100 $ & $ i$\\
$ 55213.74306 $ & $   0.00229 $ & $   0.00098 $ & $ i$\\
$ 55213.74390 $ & $   0.00232 $ & $   0.00098 $ & $ i$\\
$ 55213.74451 $ & $   0.00092 $ & $   0.00098 $ & $ i$\\
$ 55213.74512 $ & $   0.00010 $ & $   0.00098 $ & $ i$\\
$ 55213.74572 $ & $  -0.00040 $ & $   0.00098 $ & $ i$\\
$ 55213.74636 $ & $   0.00085 $ & $   0.00098 $ & $ i$\\
$ 55213.74718 $ & $  -0.00123 $ & $   0.00098 $ & $ i$\\
$ 55213.74779 $ & $   0.00036 $ & $   0.00098 $ & $ i$\\
$ 55213.74839 $ & $   0.00059 $ & $   0.00099 $ & $ i$\\
$ 55213.74902 $ & $  -0.00034 $ & $   0.00098 $ & $ i$\\
$ 55213.74966 $ & $   0.00035 $ & $   0.00098 $ & $ i$\\
$ 55213.75046 $ & $  -0.00117 $ & $   0.00098 $ & $ i$\\
$ 55213.75107 $ & $   0.00068 $ & $   0.00098 $ & $ i$\\
$ 55213.75168 $ & $   0.00129 $ & $   0.00098 $ & $ i$\\
$ 55213.75229 $ & $   0.00096 $ & $   0.00097 $ & $ i$\\
$ 55213.75290 $ & $   0.00048 $ & $   0.00098 $ & $ i$\\
$ 55213.75371 $ & $  -0.00178 $ & $   0.00098 $ & $ i$\\
$ 55213.75434 $ & $  -0.00028 $ & $   0.00098 $ & $ i$\\
$ 55213.75496 $ & $  -0.00208 $ & $   0.00098 $ & $ i$\\
$ 55213.75557 $ & $  -0.00016 $ & $   0.00097 $ & $ i$\\
$ 55213.75619 $ & $  -0.00169 $ & $   0.00098 $ & $ i$\\
$ 55213.75701 $ & $   0.00144 $ & $   0.00098 $ & $ i$\\
$ 55213.75761 $ & $  -0.00006 $ & $   0.00098 $ & $ i$\\
$ 55213.75825 $ & $  -0.00127 $ & $   0.00098 $ & $ i$\\
$ 55213.75886 $ & $   0.00307 $ & $   0.00098 $ & $ i$\\
$ 55213.75947 $ & $   0.00164 $ & $   0.00098 $ & $ i$\\
$ 55213.76028 $ & $   0.00070 $ & $   0.00098 $ & $ i$\\
$ 55213.76089 $ & $   0.00156 $ & $   0.00098 $ & $ i$\\
$ 55213.76151 $ & $   0.00145 $ & $   0.00097 $ & $ i$\\
$ 55213.76214 $ & $   0.00031 $ & $   0.00098 $ & $ i$\\
$ 55213.76277 $ & $  -0.00100 $ & $   0.00098 $ & $ i$\\
$ 55213.76358 $ & $  -0.00211 $ & $   0.00098 $ & $ i$\\
$ 55213.76420 $ & $  -0.00094 $ & $   0.00098 $ & $ i$\\
$ 55213.76481 $ & $  -0.00013 $ & $   0.00098 $ & $ i$\\
$ 55213.76540 $ & $  -0.00092 $ & $   0.00097 $ & $ i$\\
$ 55213.76600 $ & $   0.00081 $ & $   0.00098 $ & $ i$\\
$ 55213.76685 $ & $   0.00004 $ & $   0.00098 $ & $ i$\\
$ 55213.76746 $ & $   0.00134 $ & $   0.00098 $ & $ i$\\
$ 55213.76806 $ & $   0.00069 $ & $   0.00098 $ & $ i$\\
$ 55213.76868 $ & $  -0.00092 $ & $   0.00098 $ & $ i$\\
$ 55213.76930 $ & $  -0.00044 $ & $   0.00099 $ & $ i$\\
$ 55213.77010 $ & $   0.00017 $ & $   0.00102 $ & $ i$\\
$ 55213.77071 $ & $  -0.00149 $ & $   0.00101 $ & $ i$\\
$ 55213.77134 $ & $  -0.00320 $ & $   0.00098 $ & $ i$\\
$ 55213.77195 $ & $  -0.00003 $ & $   0.00098 $ & $ i$\\
$ 55213.77258 $ & $  -0.00030 $ & $   0.00098 $ & $ i$\\
$ 55213.77341 $ & $  -0.00220 $ & $   0.00098 $ & $ i$\\
$ 55213.77405 $ & $   0.00010 $ & $   0.00098 $ & $ i$\\
$ 55213.77468 $ & $   0.00121 $ & $   0.00101 $ & $ i$\\
$ 55213.77532 $ & $   0.00065 $ & $   0.00101 $ & $ i$\\
$ 55213.77594 $ & $  -0.00231 $ & $   0.00108 $ & $ i$\\
$ 55213.77677 $ & $  -0.00194 $ & $   0.00123 $ & $ i$\\
$ 55213.77740 $ & $   0.00008 $ & $   0.00119 $ & $ i$\\
$ 55213.77802 $ & $  -0.00063 $ & $   0.00114 $ & $ i$\\
$ 55213.77863 $ & $  -0.00163 $ & $   0.00103 $ & $ i$\\
$ 55213.77924 $ & $  -0.00212 $ & $   0.00100 $ & $ i$\\
$ 55213.78006 $ & $   0.00103 $ & $   0.00104 $ & $ i$\\
$ 55213.78070 $ & $  -0.00239 $ & $   0.00112 $ & $ i$\\
$ 55213.78193 $ & $   0.00024 $ & $   0.00099 $ & $ i$\\
$ 55213.78256 $ & $  -0.00101 $ & $   0.00098 $ & $ i$\\
$ 55213.78337 $ & $  -0.00185 $ & $   0.00099 $ & $ i$\\
$ 55213.78399 $ & $   0.00033 $ & $   0.00098 $ & $ i$\\
$ 55213.78460 $ & $   0.00047 $ & $   0.00098 $ & $ i$\\
$ 55213.78521 $ & $   0.00110 $ & $   0.00098 $ & $ i$\\
$ 55213.78582 $ & $   0.00520 $ & $   0.00100 $ & $ i$\\
$ 55213.78662 $ & $   0.00172 $ & $   0.00097 $ & $ i$\\
$ 55213.78724 $ & $  -0.00118 $ & $   0.00097 $ & $ i$\\
$ 55213.78785 $ & $   0.00102 $ & $   0.00098 $ & $ i$\\
$ 55213.78848 $ & $   0.00094 $ & $   0.00098 $ & $ i$\\
$ 55213.78912 $ & $   0.00298 $ & $   0.00098 $ & $ i$\\
$ 55213.78994 $ & $   0.00004 $ & $   0.00098 $ & $ i$\\
$ 55213.79056 $ & $   0.00036 $ & $   0.00098 $ & $ i$\\
$ 55213.79119 $ & $   0.00458 $ & $   0.00099 $ & $ i$\\
$ 55213.79182 $ & $  -0.00086 $ & $   0.00098 $ & $ i$\\
$ 55213.79244 $ & $  -0.00107 $ & $   0.00098 $ & $ i$\\
$ 55213.79324 $ & $  -0.00035 $ & $   0.00098 $ & $ i$\\
$ 55213.79386 $ & $  -0.00222 $ & $   0.00098 $ & $ i$\\
$ 55213.79449 $ & $   0.00005 $ & $   0.00097 $ & $ i$\\
$ 55213.79511 $ & $  -0.00164 $ & $   0.00098 $ & $ i$\\
$ 55213.79574 $ & $  -0.00181 $ & $   0.00098 $ & $ i$\\
$ 55213.79653 $ & $  -0.00089 $ & $   0.00098 $ & $ i$\\
$ 55233.59370 $ & $  -0.00158 $ & $   0.00135 $ & $ i$\\
$ 55233.59415 $ & $  -0.00214 $ & $   0.00140 $ & $ i$\\
$ 55233.59476 $ & $   0.00469 $ & $   0.00133 $ & $ i$\\
$ 55233.59521 $ & $  -0.00314 $ & $   0.00134 $ & $ i$\\
$ 55233.59796 $ & $  -0.00108 $ & $   0.00133 $ & $ i$\\
$ 55233.59840 $ & $   0.00515 $ & $   0.00132 $ & $ i$\\
$ 55233.59905 $ & $  -0.00009 $ & $   0.00131 $ & $ i$\\
$ 55233.59950 $ & $   0.00136 $ & $   0.00130 $ & $ i$\\
$ 55233.60011 $ & $   0.00143 $ & $   0.00130 $ & $ i$\\
$ 55233.60056 $ & $  -0.00176 $ & $   0.00130 $ & $ i$\\
$ 55233.60120 $ & $  -0.00468 $ & $   0.00131 $ & $ i$\\
$ 55233.60376 $ & $   0.00123 $ & $   0.00131 $ & $ i$\\
$ 55233.60439 $ & $   0.00187 $ & $   0.00130 $ & $ i$\\
$ 55233.60484 $ & $   0.00122 $ & $   0.00129 $ & $ i$\\
$ 55233.60546 $ & $   0.00006 $ & $   0.00130 $ & $ i$\\
$ 55233.60591 $ & $   0.00031 $ & $   0.00130 $ & $ i$\\
$ 55233.60652 $ & $   0.00138 $ & $   0.00130 $ & $ i$\\
$ 55233.60697 $ & $   0.00099 $ & $   0.00131 $ & $ i$\\
$ 55233.60759 $ & $  -0.00238 $ & $   0.00132 $ & $ i$\\
$ 55233.60805 $ & $  -0.00080 $ & $   0.00131 $ & $ i$\\
$ 55233.60865 $ & $  -0.00264 $ & $   0.00129 $ & $ i$\\
$ 55233.60910 $ & $   0.00020 $ & $   0.00129 $ & $ i$\\
$ 55233.60975 $ & $  -0.00095 $ & $   0.00129 $ & $ i$\\
$ 55233.61021 $ & $  -0.00238 $ & $   0.00132 $ & $ i$\\
$ 55233.61131 $ & $   0.00312 $ & $   0.00140 $ & $ i$\\
$ 55233.61344 $ & $  -0.00085 $ & $   0.00139 $ & $ i$\\
$ 55233.62487 $ & $   0.00063 $ & $   0.00128 $ & $ i$\\
$ 55233.62533 $ & $  -0.00201 $ & $   0.00129 $ & $ i$\\
$ 55233.63636 $ & $   0.00311 $ & $   0.00142 $ & $ i$\\
$ 55233.63681 $ & $  -0.00403 $ & $   0.00133 $ & $ i$\\
$ 55233.63742 $ & $  -0.00008 $ & $   0.00131 $ & $ i$\\
$ 55233.63786 $ & $   0.00115 $ & $   0.00134 $ & $ i$\\
$ 55233.63849 $ & $   0.00004 $ & $   0.00141 $ & $ i$\\
$ 55233.63894 $ & $   0.00001 $ & $   0.00138 $ & $ i$\\
$ 55233.63959 $ & $   0.00240 $ & $   0.00138 $ & $ i$\\
$ 55233.66165 $ & $   0.00386 $ & $   0.00132 $ & $ i$\\
$ 55233.66227 $ & $  -0.00015 $ & $   0.00132 $ & $ i$\\
$ 55233.66272 $ & $  -0.00014 $ & $   0.00132 $ & $ i$\\
$ 55233.66334 $ & $  -0.00160 $ & $   0.00128 $ & $ i$\\
$ 55233.66380 $ & $   0.00025 $ & $   0.00133 $ & $ i$\\
$ 55233.66555 $ & $   0.00045 $ & $   0.00132 $ & $ i$\\
$ 55233.66600 $ & $  -0.00069 $ & $   0.00130 $ & $ i$\\
$ 55233.66661 $ & $  -0.00095 $ & $   0.00130 $ & $ i$\\
$ 55233.66708 $ & $   0.00299 $ & $   0.00128 $ & $ i$\\
$ 55233.66770 $ & $  -0.00056 $ & $   0.00128 $ & $ i$\\
$ 55233.66814 $ & $   0.00003 $ & $   0.00128 $ & $ i$\\
$ 55233.66876 $ & $  -0.00275 $ & $   0.00129 $ & $ i$\\
$ 55233.66922 $ & $  -0.00313 $ & $   0.00128 $ & $ i$\\
$ 55233.66985 $ & $   0.00033 $ & $   0.00131 $ & $ i$\\
$ 55233.67030 $ & $  -0.00244 $ & $   0.00134 $ & $ i$\\
$ 55233.68070 $ & $  -0.00274 $ & $   0.00137 $ & $ i$\\
$ 55233.68374 $ & $   0.00679 $ & $   0.00138 $ & $ i$\\
$ 55233.68435 $ & $   0.00598 $ & $   0.00138 $ & $ i$\\
$ 55233.68479 $ & $   0.00458 $ & $   0.00132 $ & $ i$\\
$ 55233.68544 $ & $   0.00435 $ & $   0.00132 $ & $ i$\\
$ 55233.68588 $ & $   0.00166 $ & $   0.00133 $ & $ i$\\
$ 55233.68651 $ & $   0.00802 $ & $   0.00128 $ & $ i$\\
$ 55233.68696 $ & $   0.00951 $ & $   0.00130 $ & $ i$\\
$ 55233.68757 $ & $   0.00513 $ & $   0.00128 $ & $ i$\\
$ 55233.68801 $ & $   0.01013 $ & $   0.00127 $ & $ i$\\
$ 55233.68864 $ & $   0.00755 $ & $   0.00128 $ & $ i$\\
$ 55233.68909 $ & $   0.01245 $ & $   0.00128 $ & $ i$\\
$ 55233.68969 $ & $   0.01114 $ & $   0.00128 $ & $ i$\\
$ 55233.69015 $ & $   0.00822 $ & $   0.00128 $ & $ i$\\
$ 55233.69079 $ & $   0.00688 $ & $   0.00128 $ & $ i$\\
$ 55233.69124 $ & $   0.00736 $ & $   0.00128 $ & $ i$\\
$ 55233.69184 $ & $   0.00907 $ & $   0.00128 $ & $ i$\\
$ 55233.69231 $ & $   0.00972 $ & $   0.00128 $ & $ i$\\
$ 55233.69291 $ & $   0.01350 $ & $   0.00128 $ & $ i$\\
$ 55233.69334 $ & $   0.01276 $ & $   0.00128 $ & $ i$\\
$ 55233.69397 $ & $   0.00739 $ & $   0.00128 $ & $ i$\\
$ 55233.69445 $ & $   0.01061 $ & $   0.00128 $ & $ i$\\
$ 55233.69508 $ & $   0.01162 $ & $   0.00129 $ & $ i$\\
$ 55233.69556 $ & $   0.00900 $ & $   0.00129 $ & $ i$\\
$ 55233.69621 $ & $   0.01129 $ & $   0.00128 $ & $ i$\\
$ 55233.69666 $ & $   0.01242 $ & $   0.00129 $ & $ i$\\
$ 55233.69727 $ & $   0.01326 $ & $   0.00129 $ & $ i$\\
$ 55233.69772 $ & $   0.01235 $ & $   0.00129 $ & $ i$\\
$ 55233.69833 $ & $   0.01102 $ & $   0.00128 $ & $ i$\\
$ 55233.69879 $ & $   0.00903 $ & $   0.00129 $ & $ i$\\
$ 55233.69940 $ & $   0.00903 $ & $   0.00129 $ & $ i$\\
$ 55233.69985 $ & $   0.01263 $ & $   0.00129 $ & $ i$\\
$ 55233.70046 $ & $   0.00848 $ & $   0.00128 $ & $ i$\\
$ 55233.70092 $ & $   0.01156 $ & $   0.00129 $ & $ i$\\
$ 55233.70155 $ & $   0.00956 $ & $   0.00129 $ & $ i$\\
$ 55233.70199 $ & $   0.01091 $ & $   0.00128 $ & $ i$\\
$ 55233.70261 $ & $   0.01206 $ & $   0.00129 $ & $ i$\\
$ 55233.70306 $ & $   0.01360 $ & $   0.00129 $ & $ i$\\
$ 55233.70368 $ & $   0.01021 $ & $   0.00129 $ & $ i$\\
$ 55233.70413 $ & $   0.00985 $ & $   0.00129 $ & $ i$\\
$ 55233.70475 $ & $   0.00995 $ & $   0.00129 $ & $ i$\\
$ 55233.70521 $ & $   0.01092 $ & $   0.00129 $ & $ i$\\
$ 55233.70583 $ & $   0.01468 $ & $   0.00129 $ & $ i$\\
$ 55233.70629 $ & $   0.00934 $ & $   0.00129 $ & $ i$\\
$ 55233.70692 $ & $   0.01233 $ & $   0.00129 $ & $ i$\\
$ 55233.70739 $ & $   0.00905 $ & $   0.00129 $ & $ i$\\
$ 55233.70801 $ & $   0.00986 $ & $   0.00129 $ & $ i$\\
$ 55233.70844 $ & $   0.00958 $ & $   0.00129 $ & $ i$\\
$ 55233.70905 $ & $   0.01192 $ & $   0.00129 $ & $ i$\\
$ 55233.70950 $ & $   0.01229 $ & $   0.00129 $ & $ i$\\
$ 55233.71012 $ & $   0.00632 $ & $   0.00129 $ & $ i$\\
$ 55233.71057 $ & $   0.00963 $ & $   0.00129 $ & $ i$\\
$ 55233.71118 $ & $   0.01097 $ & $   0.00131 $ & $ i$\\
$ 55233.71162 $ & $   0.01223 $ & $   0.00135 $ & $ i$\\
$ 55233.71227 $ & $   0.01316 $ & $   0.00134 $ & $ i$\\
$ 55233.71272 $ & $   0.01180 $ & $   0.00133 $ & $ i$\\
$ 55233.71333 $ & $   0.01227 $ & $   0.00131 $ & $ i$\\
$ 55233.71379 $ & $   0.01200 $ & $   0.00132 $ & $ i$\\
$ 55233.71440 $ & $   0.01102 $ & $   0.00130 $ & $ i$\\
$ 55233.71485 $ & $   0.01012 $ & $   0.00130 $ & $ i$\\
$ 55233.71546 $ & $   0.01405 $ & $   0.00130 $ & $ i$\\
$ 55233.71590 $ & $   0.00996 $ & $   0.00130 $ & $ i$\\
$ 55233.71652 $ & $   0.01125 $ & $   0.00130 $ & $ i$\\
$ 55233.71696 $ & $   0.00972 $ & $   0.00130 $ & $ i$\\
$ 55233.71761 $ & $   0.01222 $ & $   0.00130 $ & $ i$\\
$ 55233.71806 $ & $   0.01202 $ & $   0.00130 $ & $ i$\\
$ 55233.71869 $ & $   0.01164 $ & $   0.00130 $ & $ i$\\
$ 55233.71913 $ & $   0.00874 $ & $   0.00131 $ & $ i$\\
$ 55233.71975 $ & $   0.00715 $ & $   0.00134 $ & $ i$\\
$ 55233.72020 $ & $   0.00736 $ & $   0.00136 $ & $ i$\\
$ 55233.72185 $ & $   0.01020 $ & $   0.00135 $ & $ i$\\
$ 55233.72230 $ & $   0.01351 $ & $   0.00135 $ & $ i$\\
$ 55233.72295 $ & $   0.01188 $ & $   0.00133 $ & $ i$\\
$ 55233.72340 $ & $   0.00945 $ & $   0.00133 $ & $ i$\\
$ 55233.72402 $ & $   0.00776 $ & $   0.00134 $ & $ i$\\
$ 55233.72446 $ & $   0.00789 $ & $   0.00135 $ & $ i$\\
$ 55233.72508 $ & $   0.01294 $ & $   0.00136 $ & $ i$\\
$ 55233.72553 $ & $   0.00662 $ & $   0.00137 $ & $ i$\\
$ 55233.72613 $ & $   0.01063 $ & $   0.00132 $ & $ i$\\
$ 55233.72659 $ & $   0.01129 $ & $   0.00137 $ & $ i$\\
$ 55233.72721 $ & $   0.01578 $ & $   0.00137 $ & $ i$\\
$ 55233.72766 $ & $   0.01395 $ & $   0.00139 $ & $ i$\\
$ 55233.72830 $ & $   0.01398 $ & $   0.00139 $ & $ i$\\
$ 55233.72936 $ & $   0.01035 $ & $   0.00133 $ & $ i$\\
$ 55233.72982 $ & $   0.00984 $ & $   0.00133 $ & $ i$\\
$ 55233.73043 $ & $   0.01495 $ & $   0.00134 $ & $ i$\\
$ 55233.73088 $ & $   0.01058 $ & $   0.00140 $ & $ i$\\
$ 55233.73301 $ & $   0.00798 $ & $   0.00138 $ & $ i$\\
$ 55233.73365 $ & $   0.01209 $ & $   0.00133 $ & $ i$\\
$ 55233.73409 $ & $   0.01145 $ & $   0.00136 $ & $ i$\\
$ 55233.73471 $ & $   0.01085 $ & $   0.00132 $ & $ i$\\
$ 55233.73516 $ & $   0.00704 $ & $   0.00131 $ & $ i$\\
$ 55233.73576 $ & $   0.01005 $ & $   0.00131 $ & $ i$\\
$ 55233.73619 $ & $   0.01440 $ & $   0.00131 $ & $ i$\\
$ 55233.73682 $ & $   0.01633 $ & $   0.00131 $ & $ i$\\
$ 55233.73727 $ & $   0.01453 $ & $   0.00131 $ & $ i$\\
$ 55233.73788 $ & $   0.00914 $ & $   0.00131 $ & $ i$\\
$ 55233.73832 $ & $   0.01006 $ & $   0.00131 $ & $ i$\\
$ 55233.73897 $ & $   0.01113 $ & $   0.00131 $ & $ i$\\
$ 55233.73941 $ & $   0.01454 $ & $   0.00131 $ & $ i$\\
$ 55233.74004 $ & $   0.01192 $ & $   0.00130 $ & $ i$\\
$ 55233.74049 $ & $   0.01148 $ & $   0.00131 $ & $ i$\\
$ 55233.74109 $ & $   0.01325 $ & $   0.00132 $ & $ i$\\
$ 55233.74153 $ & $   0.01634 $ & $   0.00132 $ & $ i$\\
$ 55233.74214 $ & $   0.01245 $ & $   0.00131 $ & $ i$\\
$ 55233.74258 $ & $   0.01246 $ & $   0.00132 $ & $ i$\\
$ 55233.74319 $ & $   0.01395 $ & $   0.00131 $ & $ i$\\
$ 55233.74365 $ & $   0.00949 $ & $   0.00131 $ & $ i$\\
$ 55233.74429 $ & $   0.01030 $ & $   0.00132 $ & $ i$\\
$ 55233.74473 $ & $   0.01357 $ & $   0.00132 $ & $ i$\\
$ 55233.74536 $ & $   0.01164 $ & $   0.00132 $ & $ i$\\
$ 55233.74580 $ & $   0.01104 $ & $   0.00132 $ & $ i$\\
$ 55233.74641 $ & $   0.01441 $ & $   0.00132 $ & $ i$\\
$ 55233.74687 $ & $   0.00740 $ & $   0.00132 $ & $ i$\\
$ 55233.74749 $ & $   0.01130 $ & $   0.00132 $ & $ i$\\
$ 55233.74795 $ & $   0.01166 $ & $   0.00133 $ & $ i$\\
$ 55233.74855 $ & $   0.01386 $ & $   0.00132 $ & $ i$\\
$ 55233.74900 $ & $   0.01350 $ & $   0.00132 $ & $ i$\\
$ 55233.74964 $ & $   0.00802 $ & $   0.00132 $ & $ i$\\
$ 55233.75008 $ & $   0.01126 $ & $   0.00133 $ & $ i$\\
$ 55233.75071 $ & $   0.01041 $ & $   0.00132 $ & $ i$\\
$ 55233.75116 $ & $   0.01400 $ & $   0.00133 $ & $ i$\\
$ 55233.75177 $ & $   0.01288 $ & $   0.00133 $ & $ i$\\
$ 55233.75223 $ & $   0.01418 $ & $   0.00133 $ & $ i$\\
$ 55233.75286 $ & $   0.01079 $ & $   0.00132 $ & $ i$\\
$ 55233.75331 $ & $   0.00988 $ & $   0.00132 $ & $ i$\\
$ 55233.75395 $ & $   0.01314 $ & $   0.00133 $ & $ i$\\
$ 55233.75440 $ & $   0.01268 $ & $   0.00133 $ & $ i$\\
$ 55233.75507 $ & $   0.01100 $ & $   0.00133 $ & $ i$\\
$ 55233.75552 $ & $   0.01055 $ & $   0.00133 $ & $ i$\\
$ 55233.75612 $ & $   0.01092 $ & $   0.00133 $ & $ i$\\
$ 55233.75657 $ & $   0.01252 $ & $   0.00133 $ & $ i$\\
$ 55233.75720 $ & $   0.01140 $ & $   0.00133 $ & $ i$\\
$ 55233.75765 $ & $   0.01172 $ & $   0.00133 $ & $ i$\\
$ 55233.75826 $ & $   0.01144 $ & $   0.00132 $ & $ i$\\
$ 55233.75870 $ & $   0.00920 $ & $   0.00133 $ & $ i$\\
$ 55233.75932 $ & $   0.00774 $ & $   0.00133 $ & $ i$\\
$ 55233.75978 $ & $   0.01077 $ & $   0.00133 $ & $ i$\\
$ 55233.76044 $ & $   0.01326 $ & $   0.00135 $ & $ i$\\
$ 55233.76089 $ & $   0.01087 $ & $   0.00135 $ & $ i$\\
$ 55233.76150 $ & $   0.01230 $ & $   0.00135 $ & $ i$\\
$ 55233.76197 $ & $   0.01089 $ & $   0.00137 $ & $ i$\\
$ 55233.76900 $ & $   0.01067 $ & $   0.00140 $ & $ i$\\
$ 55233.76945 $ & $   0.01222 $ & $   0.00137 $ & $ i$\\
$ 55233.79082 $ & $   0.01085 $ & $   0.00152 $ & $ i$\\
$ 55233.79125 $ & $   0.00693 $ & $   0.00141 $ & $ i$\\
$ 55233.79186 $ & $   0.00861 $ & $   0.00141 $ & $ i$\\
$ 55233.79231 $ & $   0.00733 $ & $   0.00141 $ & $ i$\\
$ 55233.79293 $ & $   0.01044 $ & $   0.00140 $ & $ i$\\
$ 55233.79337 $ & $   0.01024 $ & $   0.00140 $ & $ i$\\
$ 55233.79399 $ & $   0.00850 $ & $   0.00145 $ & $ i$\\
$ 55233.79445 $ & $   0.01201 $ & $   0.00144 $ & $ i$\\
$ 55233.79506 $ & $   0.01167 $ & $   0.00147 $ & $ i$\\
$ 55233.79551 $ & $   0.01145 $ & $   0.00142 $ & $ i$\\
$ 55233.79614 $ & $   0.01343 $ & $   0.00143 $ & $ i$\\
$ 55233.79661 $ & $   0.01313 $ & $   0.00145 $ & $ i$\\
$ 55233.79723 $ & $   0.00749 $ & $   0.00144 $ & $ i$\\
$ 55233.79768 $ & $   0.00964 $ & $   0.00143 $ & $ i$\\
$ 55233.79830 $ & $   0.01114 $ & $   0.00143 $ & $ i$\\
$ 55233.79875 $ & $   0.01331 $ & $   0.00144 $ & $ i$\\
$ 55233.79937 $ & $   0.00961 $ & $   0.00145 $ & $ i$\\
$ 55233.79982 $ & $   0.01661 $ & $   0.00146 $ & $ i$\\
$ 55233.80044 $ & $   0.01183 $ & $   0.00145 $ & $ i$\\
$ 55233.80089 $ & $   0.00941 $ & $   0.00146 $ & $ i$\\
$ 55233.80153 $ & $   0.01067 $ & $   0.00148 $ & $ i$\\
$ 55233.80194 $ & $   0.01066 $ & $   0.00146 $ & $ i$\\
$ 55233.80257 $ & $   0.00618 $ & $   0.00146 $ & $ i$\\
$ 55233.80303 $ & $   0.00873 $ & $   0.00148 $ & $ i$\\
$ 55233.80365 $ & $   0.01256 $ & $   0.00148 $ & $ i$\\
$ 55233.80411 $ & $   0.01168 $ & $   0.00149 $ & $ i$\\
$ 55233.80473 $ & $   0.00941 $ & $   0.00152 $ & $ i$\\
$ 55233.80518 $ & $   0.00955 $ & $   0.00151 $ & $ i$\\
$ 55233.80581 $ & $   0.00882 $ & $   0.00151 $ & $ i$\\
$ 55233.80626 $ & $   0.01396 $ & $   0.00150 $ & $ i$\\
$ 55233.80689 $ & $   0.01187 $ & $   0.00148 $ & $ i$\\
$ 55233.80735 $ & $   0.01388 $ & $   0.00148 $ & $ i$\\
$ 55233.80796 $ & $   0.01037 $ & $   0.00148 $ & $ i$\\
$ 55233.80841 $ & $   0.00698 $ & $   0.00147 $ & $ i$\\
$ 55233.80902 $ & $   0.00978 $ & $   0.00154 $ & $ i$\\
$ 55233.86332 $ & $   0.00261 $ & $   0.00150 $ & $ i$\\
$ 55233.86379 $ & $  -0.00258 $ & $   0.00149 $ & $ i$\\
$ 55233.86442 $ & $   0.00312 $ & $   0.00145 $ & $ i$\\
$ 55233.86487 $ & $  -0.00023 $ & $   0.00142 $ & $ i$\\
$ 55233.86547 $ & $   0.00010 $ & $   0.00144 $ & $ i$\\
$ 55233.86592 $ & $   0.00160 $ & $   0.00136 $ & $ i$\\
$ 55233.86657 $ & $  -0.00373 $ & $   0.00142 $ & $ i$\\
$ 55233.86703 $ & $   0.00092 $ & $   0.00150 $ & $ i$\\
$ 55233.86766 $ & $   0.00189 $ & $   0.00147 $ & $ i$\\
$ 55233.86811 $ & $  -0.00101 $ & $   0.00142 $ & $ i$\\
$ 55233.86872 $ & $   0.00028 $ & $   0.00144 $ & $ i$\\
$ 55233.86917 $ & $   0.00316 $ & $   0.00146 $ & $ i$\\
$ 55233.86978 $ & $   0.00294 $ & $   0.00139 $ & $ i$\\
$ 55233.87024 $ & $   0.00190 $ & $   0.00138 $ & $ i$\\
$ 55233.87085 $ & $  -0.00080 $ & $   0.00136 $ & $ i$\\
$ 55233.87129 $ & $  -0.00636 $ & $   0.00137 $ & $ i$\\
$ 55233.87194 $ & $   0.00118 $ & $   0.00153 $ & $ i$\\
$ 55233.87239 $ & $  -0.00300 $ & $   0.00139 $ & $ i$\\
$ 55233.87300 $ & $   0.00006 $ & $   0.00138 $ & $ i$\\
$ 55233.87343 $ & $   0.00115 $ & $   0.00142 $ & $ i$\\
$ 55233.87404 $ & $   0.00233 $ & $   0.00134 $ & $ i$\\
$ 55233.87446 $ & $  -0.00351 $ & $   0.00134 $ & $ i$\\
$ 55233.87509 $ & $   0.00129 $ & $   0.00136 $ & $ i$\\
$ 55233.87555 $ & $   0.00056 $ & $   0.00137 $ & $ i$\\
$ 55233.87726 $ & $   0.00061 $ & $   0.00144 $ & $ i$\\
$ 55233.87772 $ & $  -0.00100 $ & $   0.00156 $ & $ i$\\
$ 55233.87835 $ & $  -0.00053 $ & $   0.00154 $ & $ i$\\
$ 55243.72943 $ & $   0.00153 $ & $   0.00090 $ & $ i$\\
$ 55243.72979 $ & $   0.00040 $ & $   0.00090 $ & $ i$\\
$ 55243.73013 $ & $   0.00200 $ & $   0.00090 $ & $ i$\\
$ 55243.73048 $ & $   0.00143 $ & $   0.00090 $ & $ i$\\
$ 55243.73083 $ & $  -0.00022 $ & $   0.00090 $ & $ i$\\
$ 55243.73118 $ & $  -0.00186 $ & $   0.00090 $ & $ i$\\
$ 55243.73153 $ & $   0.00033 $ & $   0.00090 $ & $ i$\\
$ 55243.73189 $ & $   0.00227 $ & $   0.00090 $ & $ i$\\
$ 55243.73224 $ & $   0.00247 $ & $   0.00090 $ & $ i$\\
$ 55243.73259 $ & $   0.00037 $ & $   0.00090 $ & $ i$\\
$ 55243.73295 $ & $   0.00123 $ & $   0.00090 $ & $ i$\\
$ 55243.73333 $ & $  -0.00093 $ & $   0.00090 $ & $ i$\\
$ 55243.73372 $ & $   0.00071 $ & $   0.00090 $ & $ i$\\
$ 55243.73447 $ & $   0.00038 $ & $   0.00090 $ & $ i$\\
$ 55243.73483 $ & $   0.00094 $ & $   0.00090 $ & $ i$\\
$ 55243.73522 $ & $   0.00141 $ & $   0.00090 $ & $ i$\\
$ 55243.73563 $ & $  -0.00298 $ & $   0.00090 $ & $ i$\\
$ 55243.73598 $ & $  -0.00061 $ & $   0.00090 $ & $ i$\\
$ 55243.73633 $ & $   0.00147 $ & $   0.00090 $ & $ i$\\
$ 55243.73670 $ & $   0.00075 $ & $   0.00090 $ & $ i$\\
$ 55243.73705 $ & $  -0.00192 $ & $   0.00090 $ & $ i$\\
$ 55243.73741 $ & $   0.00013 $ & $   0.00090 $ & $ i$\\
$ 55243.73777 $ & $   0.00033 $ & $   0.00090 $ & $ i$\\
$ 55243.73812 $ & $   0.00097 $ & $   0.00090 $ & $ i$\\
$ 55243.73847 $ & $   0.00066 $ & $   0.00090 $ & $ i$\\
$ 55243.73883 $ & $   0.00048 $ & $   0.00090 $ & $ i$\\
$ 55243.73918 $ & $  -0.00124 $ & $   0.00090 $ & $ i$\\
$ 55243.73957 $ & $   0.00103 $ & $   0.00090 $ & $ i$\\
$ 55243.73997 $ & $   0.00114 $ & $   0.00090 $ & $ i$\\
$ 55243.74033 $ & $  -0.00079 $ & $   0.00089 $ & $ i$\\
$ 55243.74068 $ & $  -0.00273 $ & $   0.00090 $ & $ i$\\
$ 55243.74105 $ & $  -0.00181 $ & $   0.00090 $ & $ i$\\
$ 55243.74144 $ & $   0.00128 $ & $   0.00090 $ & $ i$\\
$ 55243.74219 $ & $   0.00164 $ & $   0.00090 $ & $ i$\\
$ 55243.74254 $ & $  -0.00123 $ & $   0.00090 $ & $ i$\\
$ 55243.74289 $ & $   0.00287 $ & $   0.00090 $ & $ i$\\
$ 55243.74325 $ & $  -0.00310 $ & $   0.00089 $ & $ i$\\
$ 55243.74360 $ & $   0.00259 $ & $   0.00090 $ & $ i$\\
$ 55243.74395 $ & $   0.00165 $ & $   0.00090 $ & $ i$\\
$ 55243.74429 $ & $   0.00101 $ & $   0.00090 $ & $ i$\\
$ 55243.74464 $ & $   0.00235 $ & $   0.00090 $ & $ i$\\
$ 55243.74499 $ & $  -0.00053 $ & $   0.00090 $ & $ i$\\
$ 55243.74535 $ & $   0.00192 $ & $   0.00090 $ & $ i$\\
$ 55243.74570 $ & $   0.00142 $ & $   0.00090 $ & $ i$\\
$ 55243.74605 $ & $   0.00416 $ & $   0.00090 $ & $ i$\\
$ 55243.74640 $ & $   0.00198 $ & $   0.00090 $ & $ i$\\
$ 55243.74675 $ & $  -0.00001 $ & $   0.00090 $ & $ i$\\
$ 55243.74711 $ & $   0.00355 $ & $   0.00090 $ & $ i$\\
$ 55243.74747 $ & $   0.00639 $ & $   0.00090 $ & $ i$\\
$ 55243.74787 $ & $   0.00560 $ & $   0.00090 $ & $ i$\\
$ 55243.74827 $ & $   0.00455 $ & $   0.00090 $ & $ i$\\
$ 55243.74862 $ & $   0.00172 $ & $   0.00090 $ & $ i$\\
$ 55243.74899 $ & $   0.00652 $ & $   0.00090 $ & $ i$\\
$ 55243.74934 $ & $   0.00424 $ & $   0.00090 $ & $ i$\\
$ 55243.74971 $ & $   0.00177 $ & $   0.00090 $ & $ i$\\
$ 55243.75006 $ & $   0.00234 $ & $   0.00090 $ & $ i$\\
$ 55243.75042 $ & $   0.00698 $ & $   0.00090 $ & $ i$\\
$ 55243.75077 $ & $   0.00717 $ & $   0.00090 $ & $ i$\\
$ 55243.75154 $ & $   0.00603 $ & $   0.00090 $ & $ i$\\
$ 55243.75193 $ & $   0.00503 $ & $   0.00090 $ & $ i$\\
$ 55243.75229 $ & $   0.00615 $ & $   0.00090 $ & $ i$\\
$ 55243.75263 $ & $   0.00619 $ & $   0.00090 $ & $ i$\\
$ 55243.75302 $ & $   0.00940 $ & $   0.00090 $ & $ i$\\
$ 55243.75343 $ & $   0.00929 $ & $   0.00090 $ & $ i$\\
$ 55243.75378 $ & $   0.00695 $ & $   0.00090 $ & $ i$\\
$ 55243.75414 $ & $   0.00922 $ & $   0.00090 $ & $ i$\\
$ 55243.75448 $ & $   0.00488 $ & $   0.00090 $ & $ i$\\
$ 55243.75488 $ & $   0.01113 $ & $   0.00090 $ & $ i$\\
$ 55243.75529 $ & $   0.00658 $ & $   0.00090 $ & $ i$\\
$ 55243.75564 $ & $   0.01147 $ & $   0.00090 $ & $ i$\\
$ 55243.75600 $ & $   0.00935 $ & $   0.00090 $ & $ i$\\
$ 55243.75634 $ & $   0.01014 $ & $   0.00090 $ & $ i$\\
$ 55243.75673 $ & $   0.00984 $ & $   0.00090 $ & $ i$\\
$ 55243.75714 $ & $   0.00856 $ & $   0.00090 $ & $ i$\\
$ 55243.75749 $ & $   0.00851 $ & $   0.00090 $ & $ i$\\
$ 55243.75785 $ & $   0.00692 $ & $   0.00090 $ & $ i$\\
$ 55243.75820 $ & $   0.01170 $ & $   0.00090 $ & $ i$\\
$ 55243.75859 $ & $   0.01028 $ & $   0.00090 $ & $ i$\\
$ 55243.75898 $ & $   0.01171 $ & $   0.00090 $ & $ i$\\
$ 55243.75970 $ & $   0.00988 $ & $   0.00090 $ & $ i$\\
$ 55243.76005 $ & $   0.00786 $ & $   0.00090 $ & $ i$\\
$ 55243.76044 $ & $   0.01001 $ & $   0.00090 $ & $ i$\\
$ 55243.76083 $ & $   0.00835 $ & $   0.00090 $ & $ i$\\
$ 55243.76119 $ & $   0.01161 $ & $   0.00090 $ & $ i$\\
$ 55243.76156 $ & $   0.00898 $ & $   0.00090 $ & $ i$\\
$ 55243.76191 $ & $   0.00897 $ & $   0.00090 $ & $ i$\\
$ 55243.76226 $ & $   0.00963 $ & $   0.00090 $ & $ i$\\
$ 55243.76261 $ & $   0.00750 $ & $   0.00090 $ & $ i$\\
$ 55243.76296 $ & $   0.00720 $ & $   0.00090 $ & $ i$\\
$ 55243.76330 $ & $   0.01059 $ & $   0.00090 $ & $ i$\\
$ 55243.76410 $ & $   0.01503 $ & $   0.00090 $ & $ i$\\
$ 55243.76445 $ & $   0.00976 $ & $   0.00090 $ & $ i$\\
$ 55243.76481 $ & $   0.00960 $ & $   0.00090 $ & $ i$\\
$ 55243.76516 $ & $   0.01014 $ & $   0.00090 $ & $ i$\\
$ 55243.76551 $ & $   0.01358 $ & $   0.00090 $ & $ i$\\
$ 55243.76586 $ & $   0.00883 $ & $   0.00090 $ & $ i$\\
$ 55243.76621 $ & $   0.01161 $ & $   0.00090 $ & $ i$\\
$ 55243.76655 $ & $   0.01163 $ & $   0.00090 $ & $ i$\\
$ 55243.76690 $ & $   0.00919 $ & $   0.00090 $ & $ i$\\
$ 55243.76728 $ & $   0.01066 $ & $   0.00090 $ & $ i$\\
$ 55243.76769 $ & $   0.00931 $ & $   0.00090 $ & $ i$\\
$ 55243.76809 $ & $   0.00919 $ & $   0.00090 $ & $ i$\\
$ 55243.76844 $ & $   0.01250 $ & $   0.00090 $ & $ i$\\
$ 55243.76879 $ & $   0.01015 $ & $   0.00090 $ & $ i$\\
$ 55243.76949 $ & $   0.01014 $ & $   0.00090 $ & $ i$\\
$ 55243.76985 $ & $   0.00809 $ & $   0.00090 $ & $ i$\\
$ 55243.77020 $ & $   0.00796 $ & $   0.00090 $ & $ i$\\
$ 55243.77056 $ & $   0.01123 $ & $   0.00090 $ & $ i$\\
$ 55243.77092 $ & $   0.00934 $ & $   0.00090 $ & $ i$\\
$ 55243.77129 $ & $   0.01015 $ & $   0.00090 $ & $ i$\\
$ 55243.77164 $ & $   0.00962 $ & $   0.00090 $ & $ i$\\
$ 55243.77238 $ & $   0.01222 $ & $   0.00090 $ & $ i$\\
$ 55243.77277 $ & $   0.01386 $ & $   0.00090 $ & $ i$\\
$ 55243.77314 $ & $   0.01173 $ & $   0.00090 $ & $ i$\\
$ 55243.77349 $ & $   0.00971 $ & $   0.00090 $ & $ i$\\
$ 55243.77388 $ & $   0.01206 $ & $   0.00090 $ & $ i$\\
$ 55243.77428 $ & $   0.01078 $ & $   0.00090 $ & $ i$\\
$ 55243.77463 $ & $   0.01187 $ & $   0.00090 $ & $ i$\\
$ 55243.77571 $ & $   0.01223 $ & $   0.00090 $ & $ i$\\
$ 55243.77609 $ & $   0.01242 $ & $   0.00090 $ & $ i$\\
$ 55243.77649 $ & $   0.01071 $ & $   0.00090 $ & $ i$\\
$ 55243.77686 $ & $   0.01294 $ & $   0.00090 $ & $ i$\\
$ 55243.77721 $ & $   0.01155 $ & $   0.00090 $ & $ i$\\
$ 55243.77795 $ & $   0.00705 $ & $   0.00090 $ & $ i$\\
$ 55243.77835 $ & $   0.00819 $ & $   0.00090 $ & $ i$\\
$ 55243.77907 $ & $   0.01183 $ & $   0.00090 $ & $ i$\\
$ 55243.77942 $ & $   0.00999 $ & $   0.00090 $ & $ i$\\
$ 55243.77977 $ & $   0.01277 $ & $   0.00090 $ & $ i$\\
$ 55243.78013 $ & $   0.00938 $ & $   0.00090 $ & $ i$\\
$ 55243.78047 $ & $   0.01206 $ & $   0.00090 $ & $ i$\\
$ 55243.78082 $ & $   0.01343 $ & $   0.00090 $ & $ i$\\
$ 55243.78117 $ & $   0.00984 $ & $   0.00090 $ & $ i$\\
$ 55243.78155 $ & $   0.00965 $ & $   0.00090 $ & $ i$\\
$ 55243.78195 $ & $   0.01192 $ & $   0.00090 $ & $ i$\\
$ 55243.78231 $ & $   0.00941 $ & $   0.00090 $ & $ i$\\
$ 55243.78270 $ & $   0.00978 $ & $   0.00090 $ & $ i$\\
$ 55243.78309 $ & $   0.00821 $ & $   0.00090 $ & $ i$\\
$ 55243.78346 $ & $   0.01072 $ & $   0.00090 $ & $ i$\\
$ 55243.78385 $ & $   0.01126 $ & $   0.00090 $ & $ i$\\
$ 55243.78425 $ & $   0.01183 $ & $   0.00090 $ & $ i$\\
$ 55243.78460 $ & $   0.00763 $ & $   0.00090 $ & $ i$\\
$ 55243.78497 $ & $   0.01322 $ & $   0.00090 $ & $ i$\\
$ 55243.78532 $ & $   0.01081 $ & $   0.00090 $ & $ i$\\
$ 55243.78572 $ & $   0.01157 $ & $   0.00090 $ & $ i$\\
$ 55243.78683 $ & $   0.01207 $ & $   0.00090 $ & $ i$\\
$ 55243.78719 $ & $   0.01148 $ & $   0.00090 $ & $ i$\\
$ 55243.78757 $ & $   0.01285 $ & $   0.00090 $ & $ i$\\
$ 55243.78797 $ & $   0.00927 $ & $   0.00090 $ & $ i$\\
$ 55243.78833 $ & $   0.01197 $ & $   0.00090 $ & $ i$\\
$ 55243.78869 $ & $   0.01115 $ & $   0.00090 $ & $ i$\\
$ 55243.78904 $ & $   0.00926 $ & $   0.00090 $ & $ i$\\
$ 55243.78942 $ & $   0.01010 $ & $   0.00090 $ & $ i$\\
$ 55243.78982 $ & $   0.01093 $ & $   0.00090 $ & $ i$\\
$ 55243.79018 $ & $   0.01312 $ & $   0.00090 $ & $ i$\\
$ 55243.79058 $ & $   0.01039 $ & $   0.00090 $ & $ i$\\
$ 55243.79097 $ & $   0.01080 $ & $   0.00090 $ & $ i$\\
$ 55243.79133 $ & $   0.00863 $ & $   0.00090 $ & $ i$\\
$ 55243.79170 $ & $   0.01418 $ & $   0.00090 $ & $ i$\\
$ 55243.79205 $ & $   0.01293 $ & $   0.00090 $ & $ i$\\
$ 55243.79241 $ & $   0.01013 $ & $   0.00090 $ & $ i$\\
$ 55243.79276 $ & $   0.01146 $ & $   0.00090 $ & $ i$\\
$ 55243.79311 $ & $   0.01227 $ & $   0.00090 $ & $ i$\\
$ 55243.79346 $ & $   0.00869 $ & $   0.00090 $ & $ i$\\
$ 55243.79380 $ & $   0.00940 $ & $   0.00090 $ & $ i$\\
$ 55243.79416 $ & $   0.00967 $ & $   0.00090 $ & $ i$\\
$ 55243.79451 $ & $   0.01064 $ & $   0.00090 $ & $ i$\\
$ 55243.79486 $ & $   0.01081 $ & $   0.00090 $ & $ i$\\
$ 55243.79555 $ & $   0.01223 $ & $   0.00090 $ & $ i$\\
$ 55243.79590 $ & $   0.01084 $ & $   0.00090 $ & $ i$\\
$ 55243.79625 $ & $   0.01353 $ & $   0.00090 $ & $ i$\\
$ 55243.79659 $ & $   0.01121 $ & $   0.00090 $ & $ i$\\
$ 55243.79694 $ & $   0.01229 $ & $   0.00090 $ & $ i$\\
$ 55243.79733 $ & $   0.00940 $ & $   0.00090 $ & $ i$\\
$ 55243.79772 $ & $   0.01104 $ & $   0.00090 $ & $ i$\\
$ 55243.79808 $ & $   0.01273 $ & $   0.00090 $ & $ i$\\
$ 55243.79848 $ & $   0.00859 $ & $   0.00089 $ & $ i$\\
$ 55243.79887 $ & $   0.00906 $ & $   0.00090 $ & $ i$\\
$ 55243.79923 $ & $   0.00796 $ & $   0.00090 $ & $ i$\\
$ 55243.79959 $ & $   0.01291 $ & $   0.00090 $ & $ i$\\
$ 55243.80072 $ & $   0.01178 $ & $   0.00090 $ & $ i$\\
$ 55243.80108 $ & $   0.01068 $ & $   0.00090 $ & $ i$\\
$ 55243.80145 $ & $   0.00982 $ & $   0.00090 $ & $ i$\\
$ 55243.80180 $ & $   0.01253 $ & $   0.00090 $ & $ i$\\
$ 55243.80219 $ & $   0.01173 $ & $   0.00090 $ & $ i$\\
$ 55243.80258 $ & $   0.01316 $ & $   0.00090 $ & $ i$\\
$ 55243.80294 $ & $   0.01018 $ & $   0.00090 $ & $ i$\\
$ 55243.80331 $ & $   0.01285 $ & $   0.00090 $ & $ i$\\
$ 55243.80366 $ & $   0.01052 $ & $   0.00090 $ & $ i$\\
$ 55243.80401 $ & $   0.01341 $ & $   0.00090 $ & $ i$\\
$ 55243.80436 $ & $   0.01056 $ & $   0.00090 $ & $ i$\\
$ 55243.80471 $ & $   0.00922 $ & $   0.00090 $ & $ i$\\
$ 55243.80506 $ & $   0.01049 $ & $   0.00090 $ & $ i$\\
$ 55243.80540 $ & $   0.01067 $ & $   0.00090 $ & $ i$\\
$ 55243.80575 $ & $   0.00891 $ & $   0.00090 $ & $ i$\\
$ 55243.80610 $ & $   0.01162 $ & $   0.00090 $ & $ i$\\
$ 55243.80645 $ & $   0.01035 $ & $   0.00090 $ & $ i$\\
$ 55243.80679 $ & $   0.01213 $ & $   0.00090 $ & $ i$\\
$ 55243.80714 $ & $   0.00933 $ & $   0.00090 $ & $ i$\\
$ 55243.80749 $ & $   0.01271 $ & $   0.00090 $ & $ i$\\
$ 55243.80784 $ & $   0.01398 $ & $   0.00090 $ & $ i$\\
$ 55243.80819 $ & $   0.01431 $ & $   0.00090 $ & $ i$\\
$ 55243.80854 $ & $   0.01253 $ & $   0.00090 $ & $ i$\\
$ 55243.80888 $ & $   0.01013 $ & $   0.00090 $ & $ i$\\
$ 55243.80923 $ & $   0.01303 $ & $   0.00090 $ & $ i$\\
$ 55243.80958 $ & $   0.01142 $ & $   0.00090 $ & $ i$\\
$ 55243.80993 $ & $   0.01057 $ & $   0.00090 $ & $ i$\\
$ 55243.81027 $ & $   0.01141 $ & $   0.00090 $ & $ i$\\
$ 55243.81062 $ & $   0.01285 $ & $   0.00090 $ & $ i$\\
$ 55243.81097 $ & $   0.00975 $ & $   0.00090 $ & $ i$\\
$ 55243.81132 $ & $   0.00973 $ & $   0.00090 $ & $ i$\\
$ 55243.81167 $ & $   0.01071 $ & $   0.00090 $ & $ i$\\
$ 55243.81236 $ & $   0.01212 $ & $   0.00090 $ & $ i$\\
$ 55243.81271 $ & $   0.01112 $ & $   0.00090 $ & $ i$\\
$ 55243.81306 $ & $   0.00907 $ & $   0.00090 $ & $ i$\\
$ 55243.81340 $ & $   0.00833 $ & $   0.00090 $ & $ i$\\
$ 55243.81421 $ & $   0.01180 $ & $   0.00090 $ & $ i$\\
$ 55243.81457 $ & $   0.01227 $ & $   0.00090 $ & $ i$\\
$ 55243.81492 $ & $   0.01275 $ & $   0.00090 $ & $ i$\\
$ 55243.81526 $ & $   0.01310 $ & $   0.00090 $ & $ i$\\
$ 55243.81562 $ & $   0.00805 $ & $   0.00090 $ & $ i$\\
$ 55243.81631 $ & $   0.01216 $ & $   0.00090 $ & $ i$\\
$ 55243.81666 $ & $   0.01313 $ & $   0.00090 $ & $ i$\\
$ 55243.81700 $ & $   0.01078 $ & $   0.00090 $ & $ i$\\
$ 55243.81735 $ & $   0.01080 $ & $   0.00090 $ & $ i$\\
$ 55243.81770 $ & $   0.01301 $ & $   0.00090 $ & $ i$\\
$ 55243.81840 $ & $   0.01284 $ & $   0.00090 $ & $ i$\\
$ 55243.81875 $ & $   0.01116 $ & $   0.00090 $ & $ i$\\
$ 55243.81909 $ & $   0.01170 $ & $   0.00090 $ & $ i$\\
$ 55243.81944 $ & $   0.01030 $ & $   0.00090 $ & $ i$\\
$ 55243.82049 $ & $   0.00905 $ & $   0.00089 $ & $ i$\\
$ 55243.82118 $ & $   0.01042 $ & $   0.00090 $ & $ i$\\
$ 55243.82153 $ & $   0.01037 $ & $   0.00090 $ & $ i$\\
$ 55243.82188 $ & $   0.01009 $ & $   0.00090 $ & $ i$\\
$ 55243.82223 $ & $   0.01146 $ & $   0.00090 $ & $ i$\\
$ 55243.82257 $ & $   0.01132 $ & $   0.00090 $ & $ i$\\
$ 55243.82293 $ & $   0.01440 $ & $   0.00090 $ & $ i$\\
$ 55243.82327 $ & $   0.01248 $ & $   0.00089 $ & $ i$\\
$ 55243.82362 $ & $   0.01084 $ & $   0.00089 $ & $ i$\\
$ 55243.82397 $ & $   0.01317 $ & $   0.00090 $ & $ i$\\
$ 55243.82432 $ & $   0.00926 $ & $   0.00090 $ & $ i$\\
$ 55243.82466 $ & $   0.01118 $ & $   0.00090 $ & $ i$\\
$ 55243.82501 $ & $   0.01536 $ & $   0.00090 $ & $ i$\\
$ 55243.82536 $ & $   0.01149 $ & $   0.00090 $ & $ i$\\
$ 55243.82571 $ & $   0.01066 $ & $   0.00090 $ & $ i$\\
$ 55243.82606 $ & $   0.01363 $ & $   0.00090 $ & $ i$\\
$ 55243.82640 $ & $   0.01230 $ & $   0.00090 $ & $ i$\\
$ 55243.82675 $ & $   0.00843 $ & $   0.00090 $ & $ i$\\
$ 55243.82710 $ & $   0.01094 $ & $   0.00090 $ & $ i$\\
$ 55243.82744 $ & $   0.01123 $ & $   0.00090 $ & $ i$\\
$ 55243.82779 $ & $   0.01113 $ & $   0.00090 $ & $ i$\\
$ 55243.82814 $ & $   0.01131 $ & $   0.00090 $ & $ i$\\
$ 55243.82849 $ & $   0.01302 $ & $   0.00090 $ & $ i$\\
$ 55243.82884 $ & $   0.01536 $ & $   0.00090 $ & $ i$\\
$ 55243.82918 $ & $   0.01063 $ & $   0.00090 $ & $ i$\\
$ 55243.82988 $ & $   0.00973 $ & $   0.00090 $ & $ i$\\
$ 55243.83023 $ & $   0.01221 $ & $   0.00090 $ & $ i$\\
$ 55243.83058 $ & $   0.01205 $ & $   0.00090 $ & $ i$\\
$ 55243.83093 $ & $   0.01342 $ & $   0.00090 $ & $ i$\\
$ 55243.83128 $ & $   0.00971 $ & $   0.00090 $ & $ i$\\
$ 55243.83163 $ & $   0.01123 $ & $   0.00090 $ & $ i$\\
$ 55243.83197 $ & $   0.01298 $ & $   0.00090 $ & $ i$\\
$ 55243.83232 $ & $   0.00985 $ & $   0.00090 $ & $ i$\\
$ 55243.83267 $ & $   0.01123 $ & $   0.00090 $ & $ i$\\
$ 55243.83301 $ & $   0.01084 $ & $   0.00090 $ & $ i$\\
$ 55243.83336 $ & $   0.01131 $ & $   0.00090 $ & $ i$\\
$ 55243.83406 $ & $   0.01221 $ & $   0.00090 $ & $ i$\\
$ 55243.83440 $ & $   0.01340 $ & $   0.00090 $ & $ i$\\
$ 55243.83475 $ & $   0.01134 $ & $   0.00090 $ & $ i$\\
$ 55243.83510 $ & $   0.01208 $ & $   0.00090 $ & $ i$\\
$ 55243.83545 $ & $   0.01393 $ & $   0.00090 $ & $ i$\\
$ 55243.83579 $ & $   0.00972 $ & $   0.00090 $ & $ i$\\
$ 55243.83614 $ & $   0.01105 $ & $   0.00090 $ & $ i$\\
$ 55243.83649 $ & $   0.00975 $ & $   0.00090 $ & $ i$\\
$ 55243.83719 $ & $   0.01602 $ & $   0.00090 $ & $ i$\\
$ 55243.83754 $ & $   0.01364 $ & $   0.00090 $ & $ i$\\
$ 55243.83788 $ & $   0.00996 $ & $   0.00090 $ & $ i$\\
$ 55243.83823 $ & $   0.01178 $ & $   0.00090 $ & $ i$\\
$ 55243.83858 $ & $   0.01034 $ & $   0.00090 $ & $ i$\\
$ 55243.83893 $ & $   0.01177 $ & $   0.00090 $ & $ i$\\
$ 55243.83927 $ & $   0.01251 $ & $   0.00090 $ & $ i$\\
$ 55243.83962 $ & $   0.00961 $ & $   0.00090 $ & $ i$\\
$ 55243.83997 $ & $   0.01216 $ & $   0.00090 $ & $ i$\\
$ 55243.84032 $ & $   0.01558 $ & $   0.00090 $ & $ i$\\
$ 55243.84067 $ & $   0.01324 $ & $   0.00090 $ & $ i$\\
$ 55243.84138 $ & $   0.01601 $ & $   0.00090 $ & $ i$\\
$ 55243.84173 $ & $   0.00852 $ & $   0.00089 $ & $ i$\\
$ 55243.84247 $ & $   0.01031 $ & $   0.00089 $ & $ i$\\
$ 55243.84290 $ & $   0.01404 $ & $   0.00090 $ & $ i$\\
$ 55243.84325 $ & $   0.01364 $ & $   0.00090 $ & $ i$\\
$ 55243.84360 $ & $   0.01101 $ & $   0.00090 $ & $ i$\\
$ 55243.84395 $ & $   0.01163 $ & $   0.00089 $ & $ i$\\
$ 55243.84434 $ & $   0.00820 $ & $   0.00089 $ & $ i$\\
$ 55243.84475 $ & $   0.00972 $ & $   0.00090 $ & $ i$\\
$ 55243.84511 $ & $   0.01253 $ & $   0.00090 $ & $ i$\\
$ 55243.84546 $ & $   0.01268 $ & $   0.00090 $ & $ i$\\
$ 55243.84585 $ & $   0.01137 $ & $   0.00090 $ & $ i$\\
$ 55243.84626 $ & $   0.01051 $ & $   0.00090 $ & $ i$\\
$ 55243.84661 $ & $   0.01035 $ & $   0.00090 $ & $ i$\\
$ 55243.84697 $ & $   0.01532 $ & $   0.00090 $ & $ i$\\
$ 55243.84732 $ & $   0.00989 $ & $   0.00090 $ & $ i$\\
$ 55243.84767 $ & $   0.01063 $ & $   0.00090 $ & $ i$\\
$ 55243.84802 $ & $   0.01208 $ & $   0.00090 $ & $ i$\\
$ 55243.84837 $ & $   0.01214 $ & $   0.00090 $ & $ i$\\
$ 55243.84872 $ & $   0.01048 $ & $   0.00090 $ & $ i$\\
$ 55243.84906 $ & $   0.00870 $ & $   0.00090 $ & $ i$\\
$ 55243.84941 $ & $   0.01238 $ & $   0.00090 $ & $ i$\\
$ 55243.84976 $ & $   0.01188 $ & $   0.00090 $ & $ i$\\
$ 55243.85011 $ & $   0.01175 $ & $   0.00090 $ & $ i$\\
$ 55243.85046 $ & $   0.01134 $ & $   0.00090 $ & $ i$\\
$ 55243.85081 $ & $   0.01175 $ & $   0.00089 $ & $ i$\\
$ 55243.85115 $ & $   0.01222 $ & $   0.00090 $ & $ i$\\
$ 55243.85150 $ & $   0.01104 $ & $   0.00090 $ & $ i$\\
$ 55243.85185 $ & $   0.00685 $ & $   0.00090 $ & $ i$\\
$ 55243.85220 $ & $   0.01285 $ & $   0.00090 $ & $ i$\\
$ 55243.85255 $ & $   0.01247 $ & $   0.00090 $ & $ i$\\
$ 55243.85289 $ & $   0.00855 $ & $   0.00090 $ & $ i$\\
$ 55243.85324 $ & $   0.01094 $ & $   0.00090 $ & $ i$\\
$ 55243.85359 $ & $   0.01337 $ & $   0.00090 $ & $ i$\\
$ 55243.85394 $ & $   0.00983 $ & $   0.00090 $ & $ i$\\
$ 55243.85463 $ & $   0.01024 $ & $   0.00090 $ & $ i$\\
$ 55243.85498 $ & $   0.00927 $ & $   0.00090 $ & $ i$\\
$ 55243.85533 $ & $   0.00964 $ & $   0.00090 $ & $ i$\\
$ 55243.85568 $ & $   0.01056 $ & $   0.00090 $ & $ i$\\
$ 55243.85602 $ & $   0.00821 $ & $   0.00090 $ & $ i$\\
$ 55243.85637 $ & $   0.00920 $ & $   0.00090 $ & $ i$\\
$ 55243.85672 $ & $   0.01283 $ & $   0.00090 $ & $ i$\\
$ 55243.85707 $ & $   0.01030 $ & $   0.00090 $ & $ i$\\
$ 55243.85742 $ & $   0.01021 $ & $   0.00090 $ & $ i$\\
$ 55243.85776 $ & $   0.01111 $ & $   0.00090 $ & $ i$\\
$ 55243.85846 $ & $   0.01240 $ & $   0.00090 $ & $ i$\\
$ 55243.85881 $ & $   0.01254 $ & $   0.00090 $ & $ i$\\
$ 55243.85916 $ & $   0.00826 $ & $   0.00090 $ & $ i$\\
$ 55243.85951 $ & $   0.01186 $ & $   0.00090 $ & $ i$\\
$ 55243.85986 $ & $   0.01445 $ & $   0.00090 $ & $ i$\\
$ 55243.86055 $ & $   0.01207 $ & $   0.00090 $ & $ i$\\
$ 55243.86090 $ & $   0.01032 $ & $   0.00090 $ & $ i$\\
$ 55243.86125 $ & $   0.01222 $ & $   0.00090 $ & $ i$\\
$ 55243.86159 $ & $   0.01105 $ & $   0.00090 $ & $ i$\\
$ 55243.86194 $ & $   0.01078 $ & $   0.00090 $ & $ i$\\
$ 55243.86264 $ & $   0.01518 $ & $   0.00090 $ & $ i$\\
$ 55243.86298 $ & $   0.01056 $ & $   0.00090 $ & $ i$\\
$ 55243.86333 $ & $   0.01225 $ & $   0.00090 $ & $ i$\\
$ 55243.86438 $ & $   0.01168 $ & $   0.00089 $ & $ i$\\
$ 55243.86473 $ & $   0.01323 $ & $   0.00090 $ & $ i$\\
$ 55243.86507 $ & $   0.01130 $ & $   0.00090 $ & $ i$\\
$ 55243.86577 $ & $   0.01098 $ & $   0.00090 $ & $ i$\\
$ 55243.86612 $ & $   0.01179 $ & $   0.00090 $ & $ i$\\
$ 55243.86646 $ & $   0.00989 $ & $   0.00090 $ & $ i$\\
$ 55243.86681 $ & $   0.01062 $ & $   0.00090 $ & $ i$\\
$ 55243.86716 $ & $   0.01259 $ & $   0.00090 $ & $ i$\\
$ 55243.86751 $ & $   0.01041 $ & $   0.00090 $ & $ i$\\
$ 55243.86786 $ & $   0.01178 $ & $   0.00090 $ & $ i$\\
$ 55243.86820 $ & $   0.01094 $ & $   0.00090 $ & $ i$\\
$ 55243.86855 $ & $   0.01119 $ & $   0.00090 $ & $ i$\\
$ 55243.86890 $ & $   0.00939 $ & $   0.00090 $ & $ i$\\
$ 55243.86960 $ & $   0.01168 $ & $   0.00090 $ & $ i$\\
$ 55243.86995 $ & $   0.01327 $ & $   0.00090 $ & $ i$\\
$ 55243.87064 $ & $   0.01195 $ & $   0.00090 $ & $ i$\\
$ 55243.87168 $ & $   0.01064 $ & $   0.00090 $ & $ i$\\
$ 55243.87203 $ & $   0.01301 $ & $   0.00090 $ & $ i$\\
$ 55243.87238 $ & $   0.01062 $ & $   0.00090 $ & $ i$\\
$ 55243.87273 $ & $   0.00953 $ & $   0.00090 $ & $ i$\\
$ 55243.87307 $ & $   0.01105 $ & $   0.00090 $ & $ i$\\
$ 55243.87377 $ & $   0.01030 $ & $   0.00089 $ & $ i$\\
$ 55243.87412 $ & $   0.01278 $ & $   0.00090 $ & $ i$\\
$ 55243.87447 $ & $   0.00885 $ & $   0.00090 $ & $ i$\\
$ 55243.87551 $ & $   0.01327 $ & $   0.00090 $ & $ i$\\
$ 55243.87586 $ & $   0.00922 $ & $   0.00089 $ & $ i$\\
$ 55243.87656 $ & $   0.00596 $ & $   0.00089 $ & $ i$\\
$ 55243.87726 $ & $   0.01076 $ & $   0.00090 $ & $ i$\\
$ 55243.87760 $ & $   0.00822 $ & $   0.00090 $ & $ i$\\
$ 55243.87795 $ & $   0.01060 $ & $   0.00090 $ & $ i$\\
$ 55243.87830 $ & $   0.01094 $ & $   0.00090 $ & $ i$\\
$ 55243.87865 $ & $   0.01182 $ & $   0.00090 $ & $ i$\\
$ 55243.87900 $ & $   0.01160 $ & $   0.00089 $ & $ i$\\
$ 55243.87934 $ & $   0.01131 $ & $   0.00090 $ & $ i$\\
$ 55243.87969 $ & $   0.01167 $ & $   0.00090 $ & $ i$\\
$ 55243.88004 $ & $   0.01034 $ & $   0.00090 $ & $ i$\\
$ 55243.88039 $ & $   0.01225 $ & $   0.00090 $ & $ i$\\
$ 55243.88074 $ & $   0.01124 $ & $   0.00090 $ & $ i$\\
$ 55243.88108 $ & $   0.00476 $ & $   0.00090 $ & $ i$\\
$ 55243.88143 $ & $   0.00893 $ & $   0.00090 $ & $ i$\\
$ 55243.88213 $ & $   0.00726 $ & $   0.00090 $ & $ i$\\
$ 55243.88247 $ & $   0.01231 $ & $   0.00090 $ & $ i$\\
$ 55243.88282 $ & $   0.00987 $ & $   0.00090 $ & $ i$\\
$ 55243.88317 $ & $   0.00793 $ & $   0.00090 $ & $ i$\\
$ 55243.88352 $ & $   0.00928 $ & $   0.00089 $ & $ i$\\
$ 55243.88387 $ & $   0.00867 $ & $   0.00090 $ & $ i$\\
$ 55243.88422 $ & $   0.00755 $ & $   0.00090 $ & $ i$\\
$ 55243.88456 $ & $   0.00870 $ & $   0.00090 $ & $ i$\\
$ 55243.88491 $ & $   0.00931 $ & $   0.00090 $ & $ i$\\
$ 55243.88526 $ & $   0.00589 $ & $   0.00089 $ & $ i$\\
$ 55243.88561 $ & $   0.00816 $ & $   0.00089 $ & $ i$\\
$ 55243.88596 $ & $   0.00459 $ & $   0.00089 $ & $ i$\\
$ 55243.88630 $ & $   0.00535 $ & $   0.00089 $ & $ i$\\
$ 55243.88665 $ & $   0.00680 $ & $   0.00090 $ & $ i$\\
$ 55243.88700 $ & $   0.00572 $ & $   0.00089 $ & $ i$\\
$ 55243.88735 $ & $   0.00500 $ & $   0.00089 $ & $ i$\\
$ 55243.88770 $ & $   0.00462 $ & $   0.00089 $ & $ i$\\
$ 55243.88805 $ & $   0.00228 $ & $   0.00089 $ & $ i$\\
$ 55243.88840 $ & $   0.00275 $ & $   0.00089 $ & $ i$\\
$ 55243.88874 $ & $   0.00643 $ & $   0.00089 $ & $ i$\\
$ 55243.88909 $ & $   0.00692 $ & $   0.00089 $ & $ i$\\
$ 55243.88944 $ & $   0.00415 $ & $   0.00090 $ & $ i$\\
$ 55243.88979 $ & $   0.00330 $ & $   0.00089 $ & $ i$\\
$ 55243.89013 $ & $   0.00101 $ & $   0.00089 $ & $ i$\\
$ 55243.89048 $ & $   0.00250 $ & $   0.00089 $ & $ i$\\
$ 55243.89118 $ & $   0.00240 $ & $   0.00089 $ & $ i$\\
$ 55243.89153 $ & $   0.00149 $ & $   0.00089 $ & $ i$\\
$ 55243.89187 $ & $   0.00368 $ & $   0.00089 $ & $ i$\\
$ 55243.89222 $ & $  -0.00188 $ & $   0.00089 $ & $ i$\\
$ 55243.89256 $ & $   0.00304 $ & $   0.00089 $ & $ i$\\
$ 55243.89291 $ & $   0.00019 $ & $   0.00089 $ & $ i$\\
$ 55243.89326 $ & $  -0.00094 $ & $   0.00089 $ & $ i$\\
$ 55243.89361 $ & $  -0.00282 $ & $   0.00090 $ & $ i$\\
$ 55243.89430 $ & $  -0.00078 $ & $   0.00089 $ & $ i$\\
$ 55243.89466 $ & $   0.00153 $ & $   0.00089 $ & $ i$\\
$ 55243.89501 $ & $   0.00177 $ & $   0.00089 $ & $ i$\\
$ 55243.89535 $ & $  -0.00087 $ & $   0.00089 $ & $ i$\\
$ 55243.89570 $ & $   0.00065 $ & $   0.00089 $ & $ i$\\
$ 55243.89604 $ & $   0.00043 $ & $   0.00089 $ & $ i$\\
$ 55243.89639 $ & $   0.00053 $ & $   0.00089 $ & $ i$\\
$ 55243.89674 $ & $   0.00154 $ & $   0.00089 $ & $ i$\\
$ 55243.89709 $ & $   0.00232 $ & $   0.00089 $ & $ i$\\
$ 55243.89744 $ & $  -0.00230 $ & $   0.00089 $ & $ i$\\
$ 55243.89778 $ & $   0.00068 $ & $   0.00089 $ & $ i$\\
$ 55243.89883 $ & $   0.00394 $ & $   0.00089 $ & $ i$\\
$ 55243.89918 $ & $  -0.00127 $ & $   0.00089 $ & $ i$\\
$ 55243.89952 $ & $   0.00186 $ & $   0.00089 $ & $ i$\\
$ 55243.89987 $ & $  -0.00073 $ & $   0.00090 $ & $ i$\\
$ 55243.90022 $ & $  -0.00073 $ & $   0.00090 $ & $ i$\\
$ 55243.90057 $ & $   0.00001 $ & $   0.00089 $ & $ i$\\
$ 55243.90092 $ & $   0.00291 $ & $   0.00090 $ & $ i$\\
$ 55243.90126 $ & $  -0.00124 $ & $   0.00089 $ & $ i$\\
$ 55243.90161 $ & $   0.00007 $ & $   0.00090 $ & $ i$\\
$ 55243.90196 $ & $  -0.00271 $ & $   0.00089 $ & $ i$\\
$ 55243.90231 $ & $  -0.00059 $ & $   0.00089 $ & $ i$\\
$ 55243.90266 $ & $  -0.00011 $ & $   0.00089 $ & $ i$\\
$ 55243.90300 $ & $   0.00115 $ & $   0.00089 $ & $ i$\\
$ 55243.90335 $ & $   0.00172 $ & $   0.00090 $ & $ i$\\
$ 55243.90370 $ & $   0.00039 $ & $   0.00089 $ & $ i$\\
$ 55243.90405 $ & $   0.00119 $ & $   0.00089 $ & $ i$\\
$ 55243.90440 $ & $  -0.00055 $ & $   0.00089 $ & $ i$\\
$ 55243.90474 $ & $  -0.00192 $ & $   0.00089 $ & $ i$\\
$ 55243.90510 $ & $   0.00081 $ & $   0.00089 $ & $ i$\\
$ 55243.90580 $ & $  -0.00055 $ & $   0.00089 $ & $ i$\\
$ 55243.90614 $ & $  -0.00077 $ & $   0.00089 $ & $ i$\\
$ 55243.90649 $ & $   0.00019 $ & $   0.00089 $ & $ i$\\
$ 55243.90719 $ & $  -0.00164 $ & $   0.00089 $ & $ i$\\
$ 55243.90788 $ & $   0.00026 $ & $   0.00089 $ & $ i$\\
$ 55243.90823 $ & $  -0.00118 $ & $   0.00089 $ & $ i$\\
$ 55243.90858 $ & $   0.00098 $ & $   0.00089 $ & $ i$\\
$ 55243.90892 $ & $   0.00163 $ & $   0.00089 $ & $ i$\\
$ 55243.90927 $ & $   0.00314 $ & $   0.00089 $ & $ i$\\
$ 55243.90962 $ & $   0.00063 $ & $   0.00089 $ & $ i$\\
$ 55243.90997 $ & $  -0.00111 $ & $   0.00089 $ & $ i$\\
$ 55243.91032 $ & $  -0.00134 $ & $   0.00089 $ & $ i$\\
$ 55243.91066 $ & $  -0.00039 $ & $   0.00089 $ & $ i$\\
$ 55243.91101 $ & $  -0.00269 $ & $   0.00089 $ & $ i$\\
$ 55243.91136 $ & $  -0.00121 $ & $   0.00089 $ & $ i$\\
$ 55243.91170 $ & $  -0.00027 $ & $   0.00089 $ & $ i$\\
$ 55243.91206 $ & $  -0.00171 $ & $   0.00089 $ & $ i$\\
$ 55243.91240 $ & $  -0.00129 $ & $   0.00089 $ & $ i$\\
$ 55243.91310 $ & $  -0.00206 $ & $   0.00089 $ & $ i$\\
$ 55243.91345 $ & $   0.00197 $ & $   0.00089 $ & $ i$\\
$ 55243.91380 $ & $   0.00009 $ & $   0.00089 $ & $ i$\\
$ 55243.91415 $ & $  -0.00093 $ & $   0.00089 $ & $ i$\\
$ 55243.91449 $ & $  -0.00155 $ & $   0.00089 $ & $ i$\\
$ 55243.91519 $ & $   0.00038 $ & $   0.00089 $ & $ i$\\
$ 55243.91554 $ & $   0.00079 $ & $   0.00089 $ & $ i$\\
$ 55243.91588 $ & $  -0.00140 $ & $   0.00089 $ & $ i$\\
$ 55243.91623 $ & $   0.00054 $ & $   0.00089 $ & $ i$\\
$ 55243.91693 $ & $  -0.00241 $ & $   0.00089 $ & $ i$\\
$ 55243.91728 $ & $   0.00141 $ & $   0.00089 $ & $ i$\\
$ 55243.91762 $ & $  -0.00088 $ & $   0.00089 $ & $ i$\\
$ 55243.91797 $ & $   0.00270 $ & $   0.00089 $ & $ i$\\
$ 55243.91831 $ & $   0.00213 $ & $   0.00089 $ & $ i$\\
$ 55243.91867 $ & $  -0.00258 $ & $   0.00089 $ & $ i$\\
$ 55243.91902 $ & $   0.00181 $ & $   0.00089 $ & $ i$\\
$ 55243.91936 $ & $  -0.00353 $ & $   0.00089 $ & $ i$\\
$ 55243.91971 $ & $  -0.00066 $ & $   0.00089 $ & $ i$\\
$ 55243.92005 $ & $  -0.00351 $ & $   0.00089 $ & $ i$\\
$ 55243.92044 $ & $  -0.00315 $ & $   0.00090 $ & $ i$\\
$ 55243.92085 $ & $   0.00048 $ & $   0.00090 $ & $ i$\\
$ 55243.92124 $ & $  -0.00138 $ & $   0.00089 $ & $ i$\\
$ 55243.92168 $ & $   0.00144 $ & $   0.00090 $ & $ i$\\
$ 55243.92203 $ & $   0.00236 $ & $   0.00089 $ & $ i$\\
$ 55243.92238 $ & $  -0.00013 $ & $   0.00089 $ & $ i$\\
$ 55243.92273 $ & $  -0.00226 $ & $   0.00089 $ & $ i$\\
$ 55243.92308 $ & $  -0.00069 $ & $   0.00090 $ & $ i$\\
$ 55243.92342 $ & $  -0.00159 $ & $   0.00089 $ & $ i$\\
$ 55243.92377 $ & $   0.00080 $ & $   0.00089 $ & $ i$\\
$ 55243.92412 $ & $   0.00302 $ & $   0.00089 $ & $ i$\\
$ 55243.92447 $ & $  -0.00069 $ & $   0.00089 $ & $ i$\\
$ 55243.92482 $ & $   0.00132 $ & $   0.00089 $ & $ i$\\
$ 55243.92516 $ & $   0.00209 $ & $   0.00089 $ & $ i$\\
$ 55243.92551 $ & $   0.00153 $ & $   0.00089 $ & $ i$\\
$ 55243.92586 $ & $   0.00300 $ & $   0.00090 $ & $ i$\\
$ 55243.92621 $ & $  -0.00220 $ & $   0.00089 $ & $ i$\\
$ 55243.92656 $ & $   0.00013 $ & $   0.00090 $ & $ i$\\
$ 55243.92691 $ & $  -0.00140 $ & $   0.00089 $ & $ i$\\
$ 55243.92725 $ & $   0.00134 $ & $   0.00089 $ & $ i$\\
$ 55243.92761 $ & $   0.00038 $ & $   0.00089 $ & $ i$\\
$ 55243.92795 $ & $   0.00014 $ & $   0.00089 $ & $ i$\\
$ 55243.92830 $ & $   0.00006 $ & $   0.00089 $ & $ i$\\
$ 55243.92865 $ & $   0.00017 $ & $   0.00089 $ & $ i$\\
$ 55243.92899 $ & $  -0.00028 $ & $   0.00089 $ & $ i$\\
$ 55243.92934 $ & $   0.00022 $ & $   0.00089 $ & $ i$\\
$ 55243.92969 $ & $  -0.00355 $ & $   0.00089 $ & $ i$\\
$ 55243.93004 $ & $   0.00147 $ & $   0.00090 $ & $ i$\\
$ 55243.93039 $ & $  -0.00104 $ & $   0.00090 $ & $ i$\\
$ 55243.93074 $ & $  -0.00183 $ & $   0.00089 $ & $ i$\\
$ 55243.93109 $ & $   0.00177 $ & $   0.00089 $ & $ i$\\
$ 55243.93143 $ & $   0.00026 $ & $   0.00089 $ & $ i$\\
$ 55243.93178 $ & $  -0.00123 $ & $   0.00089 $ & $ i$\\
$ 55243.93213 $ & $   0.00181 $ & $   0.00089 $ & $ i$\\
$ 55243.93248 $ & $  -0.00416 $ & $   0.00089 $ & $ i$\\
$ 55243.93283 $ & $   0.00128 $ & $   0.00090 $ & $ i$\\
$ 55243.93317 $ & $  -0.00028 $ & $   0.00089 $ & $ i$\\
$ 55243.93352 $ & $   0.00134 $ & $   0.00089 $ & $ i$\\
$ 55243.93387 $ & $  -0.00002 $ & $   0.00089 $ & $ i$\\
$ 55243.93457 $ & $   0.00184 $ & $   0.00090 $ & $ i$\\
$ 55243.93491 $ & $  -0.00360 $ & $   0.00089 $ & $ i$\\
$ 55243.93526 $ & $   0.00194 $ & $   0.00090 $ & $ i$\\
$ 55243.93561 $ & $   0.00166 $ & $   0.00089 $ & $ i$\\
$ 55243.93596 $ & $  -0.00143 $ & $   0.00089 $ & $ i$\\
$ 55243.93631 $ & $  -0.00422 $ & $   0.00089 $ & $ i$\\
$ 55243.93666 $ & $   0.00231 $ & $   0.00089 $ & $ i$\\
$ 55243.93700 $ & $  -0.00107 $ & $   0.00089 $ & $ i$\\
$ 55243.93735 $ & $  -0.00474 $ & $   0.00089 $ & $ i$\\
$ 55243.93769 $ & $   0.00122 $ & $   0.00089 $ & $ i$\\
$ 55243.93805 $ & $   0.00077 $ & $   0.00090 $ & $ i$\\


==> phfu_tab0.tex <==
$ 55206.63289 $ & $  -0.00145 $ & $   0.00176 $ & $  10.80170 $ & $ i$\\
$ 55206.63724 $ & $   0.00220 $ & $   0.00181 $ & $  10.80640 $ & $ i$\\
$ 55206.63790 $ & $  -0.00278 $ & $   0.00173 $ & $  10.80040 $ & $ i$\\
$ 55206.64440 $ & $  -0.00213 $ & $   0.00174 $ & $  10.80220 $ & $ i$\\
$ 55206.64485 $ & $   0.00093 $ & $   0.00171 $ & $  10.80450 $ & $ i$\\
$ 55206.64548 $ & $  -0.00051 $ & $   0.00161 $ & $  10.80300 $ & $ i$\\
$ 55206.64594 $ & $   0.00535 $ & $   0.00161 $ & $  10.80670 $ & $ i$\\
$ 55206.64659 $ & $  -0.00391 $ & $   0.00141 $ & $  10.80170 $ & $ i$\\
$ 55206.64703 $ & $   0.00162 $ & $   0.00140 $ & $  10.80520 $ & $ i$\\
$ 55206.64767 $ & $  -0.00023 $ & $   0.00134 $ & $  10.80330 $ & $ i$\\
$ 55206.64813 $ & $   0.00046 $ & $   0.00136 $ & $  10.80590 $ & $ i$\\
$ 55206.64878 $ & $  -0.00166 $ & $   0.00135 $ & $  10.80250 $ & $ i$\\
$ 55206.64923 $ & $   0.00158 $ & $   0.00135 $ & $  10.80550 $ & $ i$\\
$ 55206.64985 $ & $  -0.00071 $ & $   0.00134 $ & $  10.80160 $ & $ i$\\
$ 55206.65030 $ & $   0.00200 $ & $   0.00137 $ & $  10.80510 $ & $ i$\\
$ 55206.65094 $ & $   0.00111 $ & $   0.00135 $ & $  10.80430 $ & $ i$\\
$ 55206.65139 $ & $  -0.00115 $ & $   0.00134 $ & $  10.80240 $ & $ i$\\
$ 55206.65206 $ & $  -0.00460 $ & $   0.00134 $ & $  10.79930 $ & $ i$\\
$ 55206.65253 $ & $   0.00106 $ & $   0.00134 $ & $  10.80560 $ & $ i$\\
$ 55206.65315 $ & $  -0.00252 $ & $   0.00134 $ & $  10.80210 $ & $ i$\\
$ 55206.65361 $ & $  -0.00263 $ & $   0.00133 $ & $  10.80120 $ & $ i$\\
$ 55206.65424 $ & $  -0.00108 $ & $   0.00133 $ & $  10.80320 $ & $ i$\\
$ 55206.65469 $ & $  -0.00119 $ & $   0.00136 $ & $  10.80260 $ & $ i$\\
$ 55206.65533 $ & $   0.00220 $ & $   0.00137 $ & $  10.80630 $ & $ i$\\
$ 55206.65579 $ & $  -0.00343 $ & $   0.00138 $ & $  10.79970 $ & $ i$\\
$ 55206.65644 $ & $   0.00155 $ & $   0.00144 $ & $  10.80480 $ & $ i$\\
$ 55206.65690 $ & $   0.00406 $ & $   0.00148 $ & $  10.80730 $ & $ i$\\
$ 55206.65756 $ & $   0.00578 $ & $   0.00146 $ & $  10.80860 $ & $ i$\\
$ 55206.65800 $ & $  -0.00268 $ & $   0.00146 $ & $  10.80180 $ & $ i$\\
$ 55206.65864 $ & $  -0.00107 $ & $   0.00147 $ & $  10.80140 $ & $ i$\\
$ 55206.65973 $ & $   0.00038 $ & $   0.00148 $ & $  10.80390 $ & $ i$\\
$ 55206.66018 $ & $   0.00085 $ & $   0.00146 $ & $  10.80460 $ & $ i$\\
$ 55206.66080 $ & $   0.00003 $ & $   0.00156 $ & $  10.80480 $ & $ i$\\
$ 55206.66125 $ & $  -0.00369 $ & $   0.00147 $ & $  10.80130 $ & $ i$\\
$ 55206.66189 $ & $   0.00081 $ & $   0.00154 $ & $  10.80430 $ & $ i$\\
$ 55206.66235 $ & $   0.00023 $ & $   0.00151 $ & $  10.80520 $ & $ i$\\
$ 55206.66301 $ & $   0.00220 $ & $   0.00146 $ & $  10.80630 $ & $ i$\\
$ 55206.66346 $ & $   0.00169 $ & $   0.00148 $ & $  10.80580 $ & $ i$\\
$ 55206.66410 $ & $  -0.00346 $ & $   0.00150 $ & $  10.80140 $ & $ i$\\
$ 55206.66455 $ & $  -0.00374 $ & $   0.00152 $ & $  10.80010 $ & $ i$\\
$ 55206.66519 $ & $   0.00261 $ & $   0.00155 $ & $  10.80520 $ & $ i$\\
$ 55206.66564 $ & $   0.00183 $ & $   0.00149 $ & $  10.80460 $ & $ i$\\
$ 55206.66627 $ & $   0.00251 $ & $   0.00146 $ & $  10.80650 $ & $ i$\\
$ 55206.66672 $ & $   0.00370 $ & $   0.00148 $ & $  10.80760 $ & $ i$\\
$ 55206.66735 $ & $   0.00130 $ & $   0.00148 $ & $  10.80620 $ & $ i$\\
$ 55206.66780 $ & $   0.00011 $ & $   0.00146 $ & $  10.80480 $ & $ i$\\
$ 55206.66846 $ & $   0.00316 $ & $   0.00152 $ & $  10.80640 $ & $ i$\\
$ 55206.66892 $ & $   0.00030 $ & $   0.00154 $ & $  10.80440 $ & $ i$\\
$ 55206.66956 $ & $  -0.00155 $ & $   0.00156 $ & $  10.80160 $ & $ i$\\
$ 55206.67002 $ & $   0.00061 $ & $   0.00156 $ & $  10.80330 $ & $ i$\\
$ 55206.67065 $ & $   0.00320 $ & $   0.00158 $ & $  10.80680 $ & $ i$\\
$ 55206.67109 $ & $  -0.00226 $ & $   0.00166 $ & $  10.80270 $ & $ i$\\
$ 55206.67175 $ & $  -0.00260 $ & $   0.00153 $ & $  10.80110 $ & $ i$\\
$ 55206.67220 $ & $  -0.00076 $ & $   0.00150 $ & $  10.80320 $ & $ i$\\
$ 55206.67283 $ & $   0.00307 $ & $   0.00150 $ & $  10.80640 $ & $ i$\\
$ 55206.67328 $ & $  -0.00619 $ & $   0.00159 $ & $  10.79950 $ & $ i$\\
$ 55206.67393 $ & $   0.00168 $ & $   0.00154 $ & $  10.80640 $ & $ i$\\
$ 55206.67438 $ & $  -0.00193 $ & $   0.00146 $ & $  10.80280 $ & $ i$\\
$ 55206.67500 $ & $  -0.00139 $ & $   0.00145 $ & $  10.80400 $ & $ i$\\
$ 55206.67545 $ & $   0.00030 $ & $   0.00144 $ & $  10.80610 $ & $ i$\\
$ 55206.67610 $ & $  -0.00019 $ & $   0.00142 $ & $  10.80480 $ & $ i$\\
$ 55206.67655 $ & $  -0.00338 $ & $   0.00141 $ & $  10.80110 $ & $ i$\\
$ 55206.67719 $ & $  -0.00146 $ & $   0.00141 $ & $  10.80350 $ & $ i$\\
$ 55206.67764 $ & $  -0.00358 $ & $   0.00139 $ & $  10.80170 $ & $ i$\\
$ 55206.67827 $ & $   0.00294 $ & $   0.00138 $ & $  10.80740 $ & $ i$\\
$ 55206.67873 $ & $  -0.00076 $ & $   0.00139 $ & $  10.80370 $ & $ i$\\
$ 55206.67939 $ & $   0.00076 $ & $   0.00139 $ & $  10.80620 $ & $ i$\\
$ 55206.67984 $ & $   0.00345 $ & $   0.00144 $ & $  10.80710 $ & $ i$\\
$ 55206.68048 $ & $  -0.00391 $ & $   0.00147 $ & $  10.80010 $ & $ i$\\
$ 55206.68093 $ & $   0.00310 $ & $   0.00148 $ & $  10.80520 $ & $ i$\\
$ 55206.68157 $ & $   0.00090 $ & $   0.00150 $ & $  10.80460 $ & $ i$\\
$ 55206.68202 $ & $   0.00212 $ & $   0.00149 $ & $  10.80570 $ & $ i$\\
$ 55206.68264 $ & $   0.00154 $ & $   0.00152 $ & $  10.80670 $ & $ i$\\
$ 55206.68309 $ & $   0.00130 $ & $   0.00156 $ & $  10.80530 $ & $ i$\\
$ 55206.68373 $ & $  -0.00466 $ & $   0.00158 $ & $  10.80150 $ & $ i$\\
$ 55206.68419 $ & $  -0.00298 $ & $   0.00153 $ & $  10.80040 $ & $ i$\\
$ 55206.68484 $ & $   0.00412 $ & $   0.00145 $ & $  10.80720 $ & $ i$\\
$ 55206.68530 $ & $  -0.00324 $ & $   0.00144 $ & $  10.80110 $ & $ i$\\
$ 55206.68595 $ & $  -0.00480 $ & $   0.00144 $ & $  10.80030 $ & $ i$\\
$ 55206.68640 $ & $   0.00075 $ & $   0.00144 $ & $  10.80420 $ & $ i$\\
$ 55206.68703 $ & $  -0.00137 $ & $   0.00146 $ & $  10.80210 $ & $ i$\\
$ 55206.68749 $ & $  -0.00018 $ & $   0.00154 $ & $  10.80530 $ & $ i$\\
$ 55206.68814 $ & $   0.00009 $ & $   0.00157 $ & $  10.80350 $ & $ i$\\
$ 55206.68858 $ & $   0.00144 $ & $   0.00155 $ & $  10.80550 $ & $ i$\\
$ 55206.68922 $ & $  -0.00044 $ & $   0.00149 $ & $  10.80430 $ & $ i$\\
$ 55206.68967 $ & $   0.00194 $ & $   0.00144 $ & $  10.80560 $ & $ i$\\
$ 55206.69033 $ & $  -0.00005 $ & $   0.00143 $ & $  10.80440 $ & $ i$\\
$ 55206.69077 $ & $  -0.00047 $ & $   0.00140 $ & $  10.80270 $ & $ i$\\
$ 55206.69140 $ & $  -0.00563 $ & $   0.00134 $ & $  10.79960 $ & $ i$\\
$ 55206.69186 $ & $   0.00071 $ & $   0.00133 $ & $  10.80490 $ & $ i$\\
$ 55206.69249 $ & $  -0.00157 $ & $   0.00132 $ & $  10.80240 $ & $ i$\\
$ 55206.69294 $ & $   0.00081 $ & $   0.00133 $ & $  10.80470 $ & $ i$\\
$ 55206.69359 $ & $  -0.00004 $ & $   0.00130 $ & $  10.80430 $ & $ i$\\
$ 55206.69404 $ & $   0.00056 $ & $   0.00130 $ & $  10.80390 $ & $ i$\\
$ 55206.69468 $ & $  -0.00011 $ & $   0.00130 $ & $  10.80480 $ & $ i$\\
$ 55206.69512 $ & $   0.00010 $ & $   0.00130 $ & $  10.80450 $ & $ i$\\
$ 55206.69579 $ & $   0.00247 $ & $   0.00130 $ & $  10.80740 $ & $ i$\\
$ 55206.69623 $ & $   0.00032 $ & $   0.00130 $ & $  10.80510 $ & $ i$\\
$ 55206.69688 $ & $   0.00097 $ & $   0.00131 $ & $  10.80470 $ & $ i$\\
$ 55206.69734 $ & $   0.00215 $ & $   0.00130 $ & $  10.80550 $ & $ i$\\
$ 55206.69798 $ & $   0.00389 $ & $   0.00131 $ & $  10.80730 $ & $ i$\\
$ 55206.69844 $ & $   0.00449 $ & $   0.00131 $ & $  10.80780 $ & $ i$\\
$ 55206.69907 $ & $   0.00251 $ & $   0.00132 $ & $  10.80670 $ & $ i$\\
$ 55206.69951 $ & $  -0.00112 $ & $   0.00133 $ & $  10.80260 $ & $ i$\\
$ 55206.70015 $ & $   0.00188 $ & $   0.00132 $ & $  10.80540 $ & $ i$\\
$ 55206.70059 $ & $  -0.00039 $ & $   0.00133 $ & $  10.80400 $ & $ i$\\
$ 55206.70125 $ & $  -0.00098 $ & $   0.00137 $ & $  10.80370 $ & $ i$\\
$ 55206.70170 $ & $  -0.00076 $ & $   0.00137 $ & $  10.80340 $ & $ i$\\
$ 55206.70233 $ & $   0.00052 $ & $   0.00137 $ & $  10.80370 $ & $ i$\\
$ 55206.70278 $ & $   0.00131 $ & $   0.00139 $ & $  10.80620 $ & $ i$\\
$ 55206.70343 $ & $  -0.00173 $ & $   0.00139 $ & $  10.80220 $ & $ i$\\
$ 55206.70388 $ & $   0.00324 $ & $   0.00142 $ & $  10.80650 $ & $ i$\\
$ 55206.70452 $ & $   0.00191 $ & $   0.00147 $ & $  10.80600 $ & $ i$\\
$ 55206.70497 $ & $  -0.00035 $ & $   0.00149 $ & $  10.80360 $ & $ i$\\
$ 55206.70562 $ & $   0.00347 $ & $   0.00154 $ & $  10.80690 $ & $ i$\\
$ 55206.70605 $ & $   0.00111 $ & $   0.00153 $ & $  10.80540 $ & $ i$\\
$ 55206.70670 $ & $  -0.00218 $ & $   0.00155 $ & $  10.80170 $ & $ i$\\
$ 55206.70716 $ & $   0.00387 $ & $   0.00154 $ & $  10.80850 $ & $ i$\\
$ 55206.70779 $ & $  -0.00029 $ & $   0.00153 $ & $  10.80400 $ & $ i$\\
$ 55206.70824 $ & $  -0.00036 $ & $   0.00150 $ & $  10.80350 $ & $ i$\\
$ 55206.70889 $ & $  -0.00216 $ & $   0.00153 $ & $  10.80130 $ & $ i$\\
$ 55206.70936 $ & $   0.00333 $ & $   0.00153 $ & $  10.80710 $ & $ i$\\
$ 55206.70998 $ & $  -0.00253 $ & $   0.00153 $ & $  10.80210 $ & $ i$\\
$ 55206.71042 $ & $  -0.00312 $ & $   0.00153 $ & $  10.80170 $ & $ i$\\
$ 55206.71103 $ & $   0.00068 $ & $   0.00154 $ & $  10.80520 $ & $ i$\\
$ 55206.71150 $ & $  -0.00014 $ & $   0.00157 $ & $  10.80410 $ & $ i$\\
$ 55206.71216 $ & $  -0.00161 $ & $   0.00161 $ & $  10.80240 $ & $ i$\\
$ 55206.71261 $ & $  -0.00023 $ & $   0.00171 $ & $  10.80490 $ & $ i$\\
$ 55206.71323 $ & $  -0.00451 $ & $   0.00164 $ & $  10.80070 $ & $ i$\\
$ 55206.71366 $ & $  -0.00053 $ & $   0.00173 $ & $  10.80500 $ & $ i$\\
$ 55206.71430 $ & $   0.00353 $ & $   0.00149 $ & $  10.80800 $ & $ i$\\
$ 55206.71475 $ & $  -0.00178 $ & $   0.00153 $ & $  10.80340 $ & $ i$\\
$ 55206.71537 $ & $  -0.00193 $ & $   0.00147 $ & $  10.80230 $ & $ i$\\
$ 55206.71583 $ & $  -0.00129 $ & $   0.00145 $ & $  10.80280 $ & $ i$\\
$ 55206.71646 $ & $   0.00063 $ & $   0.00135 $ & $  10.80460 $ & $ i$\\
$ 55206.71690 $ & $   0.00006 $ & $   0.00133 $ & $  10.80440 $ & $ i$\\
$ 55206.71756 $ & $   0.00251 $ & $   0.00135 $ & $  10.80660 $ & $ i$\\
$ 55206.71802 $ & $  -0.00103 $ & $   0.00137 $ & $  10.80220 $ & $ i$\\
$ 55206.71865 $ & $  -0.00239 $ & $   0.00132 $ & $  10.80260 $ & $ i$\\
$ 55206.71911 $ & $  -0.00376 $ & $   0.00133 $ & $  10.80090 $ & $ i$\\
$ 55206.71975 $ & $   0.00050 $ & $   0.00131 $ & $  10.80470 $ & $ i$\\
$ 55206.72020 $ & $   0.00315 $ & $   0.00132 $ & $  10.80720 $ & $ i$\\
$ 55206.72083 $ & $  -0.00112 $ & $   0.00134 $ & $  10.80390 $ & $ i$\\
$ 55206.72130 $ & $   0.00014 $ & $   0.00135 $ & $  10.80470 $ & $ i$\\
$ 55206.72194 $ & $   0.00057 $ & $   0.00133 $ & $  10.80480 $ & $ i$\\
$ 55206.72240 $ & $  -0.00052 $ & $   0.00135 $ & $  10.80330 $ & $ i$\\
$ 55206.72305 $ & $  -0.00251 $ & $   0.00134 $ & $  10.80140 $ & $ i$\\
$ 55206.72351 $ & $  -0.00180 $ & $   0.00134 $ & $  10.80240 $ & $ i$\\
$ 55206.72414 $ & $   0.00094 $ & $   0.00136 $ & $  10.80560 $ & $ i$\\
$ 55206.72459 $ & $   0.00099 $ & $   0.00135 $ & $  10.80430 $ & $ i$\\
$ 55206.72521 $ & $   0.00139 $ & $   0.00137 $ & $  10.80570 $ & $ i$\\
$ 55206.72567 $ & $   0.00086 $ & $   0.00136 $ & $  10.80570 $ & $ i$\\
$ 55206.72629 $ & $   0.00027 $ & $   0.00137 $ & $  10.80370 $ & $ i$\\
$ 55206.72675 $ & $   0.00168 $ & $   0.00137 $ & $  10.80550 $ & $ i$\\
$ 55206.72738 $ & $  -0.00144 $ & $   0.00136 $ & $  10.80280 $ & $ i$\\
$ 55206.72783 $ & $   0.00160 $ & $   0.00137 $ & $  10.80560 $ & $ i$\\
$ 55206.72849 $ & $   0.00180 $ & $   0.00139 $ & $  10.80580 $ & $ i$\\
$ 55206.72895 $ & $   0.00000 $ & $   0.00150 $ & $  10.80390 $ & $ i$\\
$ 55206.72956 $ & $  -0.00003 $ & $   0.00152 $ & $  10.80380 $ & $ i$\\
$ 55206.73002 $ & $  -0.00080 $ & $   0.00149 $ & $  10.80290 $ & $ i$\\
$ 55206.73064 $ & $   0.00267 $ & $   0.00154 $ & $  10.80630 $ & $ i$\\
$ 55206.73110 $ & $  -0.00287 $ & $   0.00154 $ & $  10.80130 $ & $ i$\\
$ 55206.73174 $ & $   0.00226 $ & $   0.00154 $ & $  10.80790 $ & $ i$\\
$ 55206.73218 $ & $  -0.00250 $ & $   0.00168 $ & $  10.80130 $ & $ i$\\
$ 55206.73283 $ & $  -0.00137 $ & $   0.00175 $ & $  10.80320 $ & $ i$\\
$ 55206.73328 $ & $   0.00052 $ & $   0.00169 $ & $  10.80580 $ & $ i$\\
$ 55206.73392 $ & $   0.00176 $ & $   0.00158 $ & $  10.80470 $ & $ i$\\
$ 55206.73437 $ & $  -0.00263 $ & $   0.00155 $ & $  10.80160 $ & $ i$\\
$ 55206.73500 $ & $   0.00349 $ & $   0.00147 $ & $  10.80750 $ & $ i$\\
$ 55206.73547 $ & $  -0.00090 $ & $   0.00146 $ & $  10.80190 $ & $ i$\\
$ 55206.73611 $ & $   0.00002 $ & $   0.00149 $ & $  10.80420 $ & $ i$\\
$ 55206.73654 $ & $   0.00488 $ & $   0.00153 $ & $  10.80820 $ & $ i$\\
$ 55206.73718 $ & $  -0.00217 $ & $   0.00147 $ & $  10.80330 $ & $ i$\\
$ 55206.73763 $ & $  -0.00250 $ & $   0.00144 $ & $  10.80210 $ & $ i$\\
$ 55206.73827 $ & $  -0.00639 $ & $   0.00148 $ & $  10.79940 $ & $ i$\\
$ 55206.73873 $ & $  -0.00363 $ & $   0.00154 $ & $  10.80190 $ & $ i$\\
$ 55206.73940 $ & $  -0.00130 $ & $   0.00140 $ & $  10.80340 $ & $ i$\\
$ 55206.73985 $ & $  -0.00035 $ & $   0.00136 $ & $  10.80450 $ & $ i$\\
$ 55206.74049 $ & $  -0.00167 $ & $   0.00133 $ & $  10.80360 $ & $ i$\\
$ 55206.74094 $ & $   0.00119 $ & $   0.00128 $ & $  10.80470 $ & $ i$\\
$ 55206.74160 $ & $   0.00262 $ & $   0.00130 $ & $  10.80790 $ & $ i$\\
$ 55206.74204 $ & $   0.00087 $ & $   0.00129 $ & $  10.80500 $ & $ i$\\
$ 55206.74270 $ & $  -0.00122 $ & $   0.00127 $ & $  10.80370 $ & $ i$\\
$ 55206.74317 $ & $  -0.00015 $ & $   0.00127 $ & $  10.80530 $ & $ i$\\
$ 55206.74379 $ & $  -0.00018 $ & $   0.00127 $ & $  10.80440 $ & $ i$\\
$ 55206.74424 $ & $   0.00286 $ & $   0.00126 $ & $  10.80690 $ & $ i$\\
$ 55206.74490 $ & $   0.00133 $ & $   0.00127 $ & $  10.80630 $ & $ i$\\
$ 55206.74534 $ & $  -0.00153 $ & $   0.00126 $ & $  10.80360 $ & $ i$\\
$ 55206.74596 $ & $   0.00247 $ & $   0.00127 $ & $  10.80730 $ & $ i$\\
$ 55206.74643 $ & $   0.00096 $ & $   0.00129 $ & $  10.80510 $ & $ i$\\
$ 55206.74704 $ & $   0.00110 $ & $   0.00131 $ & $  10.80530 $ & $ i$\\
$ 55206.74750 $ & $  -0.00252 $ & $   0.00132 $ & $  10.80280 $ & $ i$\\
$ 55206.74813 $ & $  -0.00288 $ & $   0.00129 $ & $  10.80240 $ & $ i$\\
$ 55206.74858 $ & $  -0.00114 $ & $   0.00129 $ & $  10.80300 $ & $ i$\\
$ 55206.74922 $ & $   0.00067 $ & $   0.00130 $ & $  10.80590 $ & $ i$\\
$ 55206.74967 $ & $  -0.00272 $ & $   0.00131 $ & $  10.80130 $ & $ i$\\
$ 55206.75032 $ & $  -0.00038 $ & $   0.00131 $ & $  10.80370 $ & $ i$\\
$ 55206.75074 $ & $   0.00258 $ & $   0.00131 $ & $  10.80640 $ & $ i$\\
$ 55206.75137 $ & $  -0.00184 $ & $   0.00133 $ & $  10.80300 $ & $ i$\\
$ 55206.75183 $ & $  -0.00103 $ & $   0.00133 $ & $  10.80390 $ & $ i$\\
$ 55206.75248 $ & $  -0.00129 $ & $   0.00134 $ & $  10.80260 $ & $ i$\\
$ 55206.75293 $ & $  -0.00284 $ & $   0.00135 $ & $  10.80220 $ & $ i$\\
$ 55206.75358 $ & $   0.00022 $ & $   0.00136 $ & $  10.80530 $ & $ i$\\
$ 55206.75403 $ & $  -0.00054 $ & $   0.00135 $ & $  10.80440 $ & $ i$\\
$ 55206.75468 $ & $   0.00474 $ & $   0.00136 $ & $  10.80930 $ & $ i$\\
$ 55206.75513 $ & $   0.00103 $ & $   0.00135 $ & $  10.80580 $ & $ i$\\
$ 55206.75580 $ & $   0.00277 $ & $   0.00134 $ & $  10.80700 $ & $ i$\\
$ 55206.75624 $ & $   0.00023 $ & $   0.00136 $ & $  10.80500 $ & $ i$\\
$ 55206.75688 $ & $  -0.00136 $ & $   0.00138 $ & $  10.80370 $ & $ i$\\
$ 55206.75732 $ & $  -0.00005 $ & $   0.00136 $ & $  10.80490 $ & $ i$\\
$ 55206.75797 $ & $   0.00155 $ & $   0.00137 $ & $  10.80620 $ & $ i$\\
$ 55206.75842 $ & $   0.00015 $ & $   0.00139 $ & $  10.80450 $ & $ i$\\
$ 55206.75904 $ & $  -0.00033 $ & $   0.00139 $ & $  10.80400 $ & $ i$\\
$ 55206.75949 $ & $  -0.00144 $ & $   0.00139 $ & $  10.80240 $ & $ i$\\
$ 55206.76012 $ & $   0.00150 $ & $   0.00138 $ & $  10.80580 $ & $ i$\\
$ 55206.76057 $ & $  -0.00195 $ & $   0.00136 $ & $  10.80340 $ & $ i$\\
$ 55206.76123 $ & $  -0.00171 $ & $   0.00135 $ & $  10.80260 $ & $ i$\\
$ 55206.76168 $ & $   0.00126 $ & $   0.00138 $ & $  10.80610 $ & $ i$\\
$ 55206.76232 $ & $  -0.00041 $ & $   0.00138 $ & $  10.80450 $ & $ i$\\
$ 55206.76277 $ & $   0.00038 $ & $   0.00138 $ & $  10.80420 $ & $ i$\\
$ 55206.76339 $ & $  -0.00185 $ & $   0.00137 $ & $  10.80290 $ & $ i$\\
$ 55206.76385 $ & $   0.00088 $ & $   0.00134 $ & $  10.80570 $ & $ i$\\
$ 55206.76448 $ & $   0.00213 $ & $   0.00132 $ & $  10.80690 $ & $ i$\\
$ 55206.76495 $ & $  -0.00174 $ & $   0.00132 $ & $  10.80240 $ & $ i$\\
$ 55206.76557 $ & $  -0.00078 $ & $   0.00131 $ & $  10.80380 $ & $ i$\\
$ 55206.76603 $ & $  -0.00032 $ & $   0.00131 $ & $  10.80310 $ & $ i$\\
$ 55206.76668 $ & $  -0.00094 $ & $   0.00135 $ & $  10.80270 $ & $ i$\\
$ 55206.76714 $ & $  -0.00004 $ & $   0.00137 $ & $  10.80420 $ & $ i$\\
$ 55206.76778 $ & $   0.00005 $ & $   0.00135 $ & $  10.80430 $ & $ i$\\
$ 55206.76824 $ & $  -0.00168 $ & $   0.00138 $ & $  10.80210 $ & $ i$\\
$ 55206.76887 $ & $   0.00041 $ & $   0.00132 $ & $  10.80520 $ & $ i$\\
$ 55206.76932 $ & $  -0.00024 $ & $   0.00130 $ & $  10.80430 $ & $ i$\\
$ 55206.76996 $ & $   0.00055 $ & $   0.00134 $ & $  10.80450 $ & $ i$\\
$ 55206.77041 $ & $   0.00164 $ & $   0.00131 $ & $  10.80630 $ & $ i$\\
$ 55206.77105 $ & $   0.00204 $ & $   0.00131 $ & $  10.80650 $ & $ i$\\
$ 55206.77147 $ & $  -0.00012 $ & $   0.00134 $ & $  10.80410 $ & $ i$\\
$ 55206.77213 $ & $   0.00032 $ & $   0.00127 $ & $  10.80440 $ & $ i$\\
$ 55206.77257 $ & $   0.00050 $ & $   0.00126 $ & $  10.80580 $ & $ i$\\
$ 55206.77320 $ & $   0.00138 $ & $   0.00126 $ & $  10.80540 $ & $ i$\\
$ 55206.77365 $ & $   0.00335 $ & $   0.00127 $ & $  10.80740 $ & $ i$\\
$ 55206.77427 $ & $   0.00110 $ & $   0.00126 $ & $  10.80460 $ & $ i$\\
$ 55206.77474 $ & $   0.00092 $ & $   0.00126 $ & $  10.80540 $ & $ i$\\
$ 55206.77539 $ & $   0.00004 $ & $   0.00126 $ & $  10.80480 $ & $ i$\\
$ 55206.77584 $ & $   0.00036 $ & $   0.00127 $ & $  10.80480 $ & $ i$\\
$ 55206.77646 $ & $   0.00061 $ & $   0.00128 $ & $  10.80480 $ & $ i$\\
$ 55206.77691 $ & $   0.00011 $ & $   0.00130 $ & $  10.80420 $ & $ i$\\
$ 55206.77756 $ & $  -0.00116 $ & $   0.00130 $ & $  10.80300 $ & $ i$\\
$ 55206.77801 $ & $   0.00236 $ & $   0.00131 $ & $  10.80670 $ & $ i$\\
$ 55206.77865 $ & $   0.00322 $ & $   0.00131 $ & $  10.80770 $ & $ i$\\
$ 55206.77911 $ & $  -0.00028 $ & $   0.00130 $ & $  10.80430 $ & $ i$\\
$ 55206.77974 $ & $   0.00072 $ & $   0.00127 $ & $  10.80440 $ & $ i$\\
$ 55206.78019 $ & $   0.00078 $ & $   0.00125 $ & $  10.80500 $ & $ i$\\
$ 55206.78081 $ & $   0.00228 $ & $   0.00124 $ & $  10.80710 $ & $ i$\\
$ 55206.78128 $ & $  -0.00347 $ & $   0.00124 $ & $  10.80110 $ & $ i$\\
$ 55206.78190 $ & $  -0.00067 $ & $   0.00123 $ & $  10.80280 $ & $ i$\\
$ 55206.78235 $ & $  -0.00118 $ & $   0.00123 $ & $  10.80310 $ & $ i$\\
$ 55206.78302 $ & $   0.00044 $ & $   0.00123 $ & $  10.80540 $ & $ i$\\
$ 55206.78345 $ & $  -0.00016 $ & $   0.00122 $ & $  10.80380 $ & $ i$\\
$ 55206.78409 $ & $  -0.00047 $ & $   0.00122 $ & $  10.80400 $ & $ i$\\
$ 55206.78454 $ & $   0.00011 $ & $   0.00122 $ & $  10.80450 $ & $ i$\\
$ 55206.78518 $ & $  -0.00368 $ & $   0.00122 $ & $  10.80120 $ & $ i$\\
$ 55206.78563 $ & $  -0.00033 $ & $   0.00122 $ & $  10.80450 $ & $ i$\\
$ 55206.78625 $ & $  -0.00073 $ & $   0.00122 $ & $  10.80370 $ & $ i$\\
$ 55206.78668 $ & $   0.00166 $ & $   0.00122 $ & $  10.80570 $ & $ i$\\
$ 55206.78732 $ & $   0.00147 $ & $   0.00122 $ & $  10.80550 $ & $ i$\\
$ 55206.78777 $ & $   0.00113 $ & $   0.00123 $ & $  10.80650 $ & $ i$\\
$ 55206.78843 $ & $   0.00103 $ & $   0.00123 $ & $  10.80660 $ & $ i$\\
$ 55206.78889 $ & $  -0.00044 $ & $   0.00123 $ & $  10.80450 $ & $ i$\\
$ 55206.78952 $ & $   0.00132 $ & $   0.00123 $ & $  10.80570 $ & $ i$\\
$ 55206.78997 $ & $   0.00110 $ & $   0.00123 $ & $  10.80610 $ & $ i$\\
$ 55206.79063 $ & $   0.00010 $ & $   0.00122 $ & $  10.80450 $ & $ i$\\
$ 55206.79107 $ & $  -0.00370 $ & $   0.00122 $ & $  10.80120 $ & $ i$\\
$ 55206.79170 $ & $  -0.00066 $ & $   0.00122 $ & $  10.80470 $ & $ i$\\
$ 55206.79216 $ & $   0.00124 $ & $   0.00122 $ & $  10.80530 $ & $ i$\\
$ 55206.79278 $ & $   0.00199 $ & $   0.00123 $ & $  10.80630 $ & $ i$\\
$ 55206.79324 $ & $   0.00387 $ & $   0.00123 $ & $  10.80820 $ & $ i$\\
$ 55206.79389 $ & $   0.00081 $ & $   0.00123 $ & $  10.80510 $ & $ i$\\
$ 55206.79436 $ & $  -0.00100 $ & $   0.00123 $ & $  10.80290 $ & $ i$\\
$ 55206.79500 $ & $  -0.00056 $ & $   0.00123 $ & $  10.80470 $ & $ i$\\
$ 55206.79548 $ & $   0.00124 $ & $   0.00123 $ & $  10.80530 $ & $ i$\\
$ 55206.79613 $ & $   0.00031 $ & $   0.00123 $ & $  10.80400 $ & $ i$\\
$ 55206.79658 $ & $  -0.00152 $ & $   0.00123 $ & $  10.80280 $ & $ i$\\
$ 55206.79720 $ & $  -0.00122 $ & $   0.00123 $ & $  10.80410 $ & $ i$\\
$ 55206.79765 $ & $   0.00170 $ & $   0.00124 $ & $  10.80570 $ & $ i$\\
$ 55206.79830 $ & $   0.00078 $ & $   0.00124 $ & $  10.80560 $ & $ i$\\
$ 55206.79874 $ & $  -0.00089 $ & $   0.00124 $ & $  10.80390 $ & $ i$\\
$ 55206.79941 $ & $   0.00186 $ & $   0.00125 $ & $  10.80680 $ & $ i$\\
$ 55206.79985 $ & $   0.00075 $ & $   0.00124 $ & $  10.80500 $ & $ i$\\
$ 55206.80049 $ & $  -0.00002 $ & $   0.00124 $ & $  10.80530 $ & $ i$\\
$ 55206.80094 $ & $  -0.00116 $ & $   0.00124 $ & $  10.80380 $ & $ i$\\
$ 55206.80159 $ & $   0.00076 $ & $   0.00123 $ & $  10.80570 $ & $ i$\\
$ 55206.80205 $ & $   0.00095 $ & $   0.00123 $ & $  10.80560 $ & $ i$\\
$ 55206.80269 $ & $   0.00051 $ & $   0.00122 $ & $  10.80500 $ & $ i$\\
$ 55206.80315 $ & $  -0.00063 $ & $   0.00122 $ & $  10.80390 $ & $ i$\\
$ 55206.80380 $ & $   0.00120 $ & $   0.00122 $ & $  10.80490 $ & $ i$\\
$ 55206.80426 $ & $  -0.00169 $ & $   0.00122 $ & $  10.80290 $ & $ i$\\
$ 55206.80491 $ & $  -0.00113 $ & $   0.00122 $ & $  10.80350 $ & $ i$\\
$ 55206.80535 $ & $   0.00006 $ & $   0.00123 $ & $  10.80410 $ & $ i$\\
$ 55206.80599 $ & $   0.00334 $ & $   0.00123 $ & $  10.80710 $ & $ i$\\
$ 55206.80640 $ & $  -0.00042 $ & $   0.00123 $ & $  10.80400 $ & $ i$\\
$ 55206.80704 $ & $  -0.00045 $ & $   0.00123 $ & $  10.80430 $ & $ i$\\
$ 55206.80747 $ & $   0.00159 $ & $   0.00124 $ & $  10.80630 $ & $ i$\\
$ 55206.80809 $ & $  -0.00196 $ & $   0.00124 $ & $  10.80180 $ & $ i$\\
$ 55206.80852 $ & $  -0.00320 $ & $   0.00123 $ & $  10.80130 $ & $ i$\\
$ 55206.80916 $ & $  -0.00085 $ & $   0.00123 $ & $  10.80380 $ & $ i$\\
$ 55206.80961 $ & $   0.00252 $ & $   0.00123 $ & $  10.80720 $ & $ i$\\
$ 55206.81027 $ & $  -0.00098 $ & $   0.00124 $ & $  10.80370 $ & $ i$\\
$ 55206.81070 $ & $  -0.00190 $ & $   0.00124 $ & $  10.80300 $ & $ i$\\
$ 55206.81133 $ & $  -0.00007 $ & $   0.00126 $ & $  10.80430 $ & $ i$\\
$ 55206.81179 $ & $   0.00023 $ & $   0.00127 $ & $  10.80620 $ & $ i$\\
$ 55206.81243 $ & $  -0.00136 $ & $   0.00127 $ & $  10.80250 $ & $ i$\\
$ 55206.81289 $ & $  -0.00135 $ & $   0.00126 $ & $  10.80320 $ & $ i$\\
$ 55206.81353 $ & $  -0.00016 $ & $   0.00128 $ & $  10.80410 $ & $ i$\\
$ 55206.81396 $ & $   0.00049 $ & $   0.00127 $ & $  10.80570 $ & $ i$\\
$ 55206.81461 $ & $  -0.00014 $ & $   0.00128 $ & $  10.80400 $ & $ i$\\
$ 55206.81506 $ & $   0.00029 $ & $   0.00130 $ & $  10.80550 $ & $ i$\\
$ 55206.81571 $ & $  -0.00062 $ & $   0.00131 $ & $  10.80460 $ & $ i$\\
$ 55206.81617 $ & $  -0.00123 $ & $   0.00132 $ & $  10.80390 $ & $ i$\\
$ 55206.81681 $ & $   0.00114 $ & $   0.00133 $ & $  10.80640 $ & $ i$\\
$ 55206.81727 $ & $  -0.00266 $ & $   0.00132 $ & $  10.80400 $ & $ i$\\
$ 55206.81790 $ & $   0.00086 $ & $   0.00130 $ & $  10.80670 $ & $ i$\\
$ 55206.81836 $ & $   0.00238 $ & $   0.00128 $ & $  10.80650 $ & $ i$\\
$ 55206.81897 $ & $   0.00044 $ & $   0.00131 $ & $  10.80580 $ & $ i$\\
$ 55206.81942 $ & $  -0.00097 $ & $   0.00133 $ & $  10.80390 $ & $ i$\\
$ 55206.82007 $ & $   0.00162 $ & $   0.00131 $ & $  10.80620 $ & $ i$\\
$ 55206.82051 $ & $   0.00211 $ & $   0.00133 $ & $  10.80720 $ & $ i$\\
$ 55206.82118 $ & $  -0.00262 $ & $   0.00128 $ & $  10.80270 $ & $ i$\\
$ 55206.82165 $ & $  -0.00095 $ & $   0.00129 $ & $  10.80370 $ & $ i$\\
$ 55206.82228 $ & $  -0.00148 $ & $   0.00134 $ & $  10.80360 $ & $ i$\\
$ 55206.82273 $ & $  -0.00233 $ & $   0.00133 $ & $  10.80220 $ & $ i$\\
$ 55206.82337 $ & $   0.00170 $ & $   0.00132 $ & $  10.80580 $ & $ i$\\
$ 55206.82381 $ & $  -0.00062 $ & $   0.00133 $ & $  10.80400 $ & $ i$\\
$ 55206.82445 $ & $  -0.00113 $ & $   0.00133 $ & $  10.80400 $ & $ i$\\
$ 55206.82489 $ & $   0.00079 $ & $   0.00134 $ & $  10.80580 $ & $ i$\\
$ 55206.82552 $ & $  -0.00344 $ & $   0.00137 $ & $  10.80190 $ & $ i$\\
$ 55206.82598 $ & $  -0.00214 $ & $   0.00141 $ & $  10.80280 $ & $ i$\\
$ 55206.82665 $ & $  -0.00162 $ & $   0.00146 $ & $  10.80360 $ & $ i$\\
$ 55206.82710 $ & $  -0.00019 $ & $   0.00142 $ & $  10.80550 $ & $ i$\\
$ 55206.82772 $ & $  -0.00074 $ & $   0.00143 $ & $  10.80370 $ & $ i$\\
$ 55206.82819 $ & $   0.00037 $ & $   0.00145 $ & $  10.80390 $ & $ i$\\
$ 55206.82881 $ & $   0.00273 $ & $   0.00148 $ & $  10.80780 $ & $ i$\\
$ 55206.82924 $ & $   0.00229 $ & $   0.00151 $ & $  10.80670 $ & $ i$\\
$ 55206.82986 $ & $   0.00054 $ & $   0.00146 $ & $  10.80470 $ & $ i$\\
$ 55206.83033 $ & $  -0.00152 $ & $   0.00147 $ & $  10.80390 $ & $ i$\\
$ 55206.83095 $ & $   0.00180 $ & $   0.00152 $ & $  10.80730 $ & $ i$\\
$ 55206.83138 $ & $  -0.00140 $ & $   0.00146 $ & $  10.80340 $ & $ i$\\
$ 55206.83204 $ & $   0.00068 $ & $   0.00143 $ & $  10.80540 $ & $ i$\\
$ 55206.83249 $ & $  -0.00177 $ & $   0.00144 $ & $  10.80270 $ & $ i$\\
$ 55206.83313 $ & $  -0.00253 $ & $   0.00146 $ & $  10.80200 $ & $ i$\\
$ 55206.83358 $ & $   0.00060 $ & $   0.00148 $ & $  10.80510 $ & $ i$\\
$ 55206.83420 $ & $  -0.00121 $ & $   0.00148 $ & $  10.80400 $ & $ i$\\
$ 55206.83466 $ & $  -0.00003 $ & $   0.00146 $ & $  10.80390 $ & $ i$\\
$ 55206.83528 $ & $  -0.00061 $ & $   0.00150 $ & $  10.80360 $ & $ i$\\
$ 55206.83574 $ & $  -0.00221 $ & $   0.00152 $ & $  10.80370 $ & $ i$\\
$ 55206.83638 $ & $   0.00092 $ & $   0.00148 $ & $  10.80490 $ & $ i$\\
$ 55206.83683 $ & $  -0.00082 $ & $   0.00146 $ & $  10.80300 $ & $ i$\\
$ 55206.83749 $ & $  -0.00058 $ & $   0.00143 $ & $  10.80410 $ & $ i$\\
$ 55206.83794 $ & $   0.00380 $ & $   0.00145 $ & $  10.80820 $ & $ i$\\
$ 55206.83859 $ & $   0.00358 $ & $   0.00144 $ & $  10.80820 $ & $ i$\\
$ 55206.83904 $ & $   0.00181 $ & $   0.00143 $ & $  10.80650 $ & $ i$\\
$ 55206.83968 $ & $   0.00375 $ & $   0.00149 $ & $  10.80850 $ & $ i$\\
$ 55206.84013 $ & $   0.00296 $ & $   0.00147 $ & $  10.80790 $ & $ i$\\
$ 55206.84077 $ & $   0.00169 $ & $   0.00151 $ & $  10.80580 $ & $ i$\\
$ 55206.84121 $ & $   0.00808 $ & $   0.00160 $ & $  10.81240 $ & $ i$\\
$ 55206.84184 $ & $   0.00644 $ & $   0.00148 $ & $  10.81100 $ & $ i$\\
$ 55206.84231 $ & $   0.00221 $ & $   0.00153 $ & $  10.80650 $ & $ i$\\
$ 55206.84295 $ & $   0.00323 $ & $   0.00152 $ & $  10.80800 $ & $ i$\\
$ 55206.84339 $ & $   0.00812 $ & $   0.00150 $ & $  10.81280 $ & $ i$\\
$ 55206.84405 $ & $   0.00350 $ & $   0.00146 $ & $  10.80810 $ & $ i$\\
$ 55206.84452 $ & $   0.00562 $ & $   0.00151 $ & $  10.81020 $ & $ i$\\
$ 55206.84517 $ & $   0.00902 $ & $   0.00157 $ & $  10.81310 $ & $ i$\\
$ 55206.84559 $ & $   0.00570 $ & $   0.00157 $ & $  10.80990 $ & $ i$\\
$ 55206.84624 $ & $   0.00875 $ & $   0.00153 $ & $  10.81320 $ & $ i$\\
$ 55206.84668 $ & $   0.01197 $ & $   0.00154 $ & $  10.81670 $ & $ i$\\
$ 55206.84733 $ & $   0.00830 $ & $   0.00150 $ & $  10.81270 $ & $ i$\\
$ 55206.84777 $ & $   0.01264 $ & $   0.00146 $ & $  10.81600 $ & $ i$\\
$ 55206.84842 $ & $   0.00905 $ & $   0.00143 $ & $  10.81310 $ & $ i$\\
$ 55206.84886 $ & $   0.01002 $ & $   0.00144 $ & $  10.81410 $ & $ i$\\
$ 55206.84949 $ & $   0.01105 $ & $   0.00140 $ & $  10.81560 $ & $ i$\\
$ 55206.84993 $ & $   0.01186 $ & $   0.00139 $ & $  10.81640 $ & $ i$\\
$ 55206.85056 $ & $   0.00965 $ & $   0.00139 $ & $  10.81320 $ & $ i$\\
$ 55206.85102 $ & $   0.00885 $ & $   0.00138 $ & $  10.81350 $ & $ i$\\
$ 55206.85165 $ & $   0.00843 $ & $   0.00136 $ & $  10.81270 $ & $ i$\\
$ 55206.85210 $ & $   0.01252 $ & $   0.00133 $ & $  10.81720 $ & $ i$\\
$ 55206.85272 $ & $   0.01006 $ & $   0.00132 $ & $  10.81430 $ & $ i$\\
$ 55206.85315 $ & $   0.01316 $ & $   0.00134 $ & $  10.81770 $ & $ i$\\
$ 55206.85381 $ & $   0.01053 $ & $   0.00135 $ & $  10.81520 $ & $ i$\\
$ 55206.85425 $ & $   0.01262 $ & $   0.00136 $ & $  10.81660 $ & $ i$\\
$ 55206.85488 $ & $   0.00925 $ & $   0.00134 $ & $  10.81430 $ & $ i$\\
$ 55206.85534 $ & $   0.00579 $ & $   0.00134 $ & $  10.81140 $ & $ i$\\
$ 55206.85602 $ & $   0.01047 $ & $   0.00135 $ & $  10.81510 $ & $ i$\\
$ 55206.85647 $ & $   0.00694 $ & $   0.00135 $ & $  10.81100 $ & $ i$\\
$ 55206.85717 $ & $   0.00919 $ & $   0.00137 $ & $  10.81340 $ & $ i$\\
$ 55206.85764 $ & $   0.00967 $ & $   0.00138 $ & $  10.81400 $ & $ i$\\
$ 55206.85827 $ & $   0.01172 $ & $   0.00140 $ & $  10.81660 $ & $ i$\\
$ 55206.85871 $ & $   0.00777 $ & $   0.00141 $ & $  10.81250 $ & $ i$\\
$ 55206.85936 $ & $   0.01137 $ & $   0.00139 $ & $  10.81600 $ & $ i$\\
$ 55206.85981 $ & $   0.01001 $ & $   0.00140 $ & $  10.81430 $ & $ i$\\
$ 55206.86045 $ & $   0.00859 $ & $   0.00140 $ & $  10.81290 $ & $ i$\\
$ 55206.86091 $ & $   0.00797 $ & $   0.00141 $ & $  10.81250 $ & $ i$\\
$ 55206.86153 $ & $   0.00929 $ & $   0.00143 $ & $  10.81340 $ & $ i$\\
$ 55206.86197 $ & $   0.00967 $ & $   0.00145 $ & $  10.81400 $ & $ i$\\
$ 55206.86262 $ & $   0.01069 $ & $   0.00144 $ & $  10.81560 $ & $ i$\\
$ 55206.86307 $ & $   0.01180 $ & $   0.00146 $ & $  10.81550 $ & $ i$\\
$ 55206.86370 $ & $   0.00973 $ & $   0.00141 $ & $  10.81490 $ & $ i$\\
$ 55206.86416 $ & $   0.01099 $ & $   0.00142 $ & $  10.81540 $ & $ i$\\
$ 55206.86481 $ & $   0.00784 $ & $   0.00142 $ & $  10.81280 $ & $ i$\\
$ 55206.86525 $ & $   0.00989 $ & $   0.00140 $ & $  10.81370 $ & $ i$\\
$ 55206.86589 $ & $   0.00851 $ & $   0.00143 $ & $  10.81280 $ & $ i$\\
$ 55206.86635 $ & $   0.01189 $ & $   0.00143 $ & $  10.81640 $ & $ i$\\
$ 55206.86698 $ & $   0.00685 $ & $   0.00140 $ & $  10.81160 $ & $ i$\\
$ 55206.86743 $ & $   0.01137 $ & $   0.00139 $ & $  10.81590 $ & $ i$\\
$ 55206.86807 $ & $   0.01115 $ & $   0.00137 $ & $  10.81520 $ & $ i$\\
$ 55206.86850 $ & $   0.01248 $ & $   0.00139 $ & $  10.81710 $ & $ i$\\
$ 55206.86914 $ & $   0.01190 $ & $   0.00141 $ & $  10.81600 $ & $ i$\\
$ 55206.86959 $ & $   0.01019 $ & $   0.00141 $ & $  10.81530 $ & $ i$\\
$ 55206.87025 $ & $   0.00921 $ & $   0.00145 $ & $  10.81410 $ & $ i$\\
$ 55206.87066 $ & $   0.01054 $ & $   0.00150 $ & $  10.81390 $ & $ i$\\
$ 55206.87130 $ & $   0.01124 $ & $   0.00153 $ & $  10.81520 $ & $ i$\\
$ 55206.87174 $ & $   0.00735 $ & $   0.00152 $ & $  10.81230 $ & $ i$\\
$ 55206.87238 $ & $   0.01180 $ & $   0.00148 $ & $  10.81700 $ & $ i$\\
$ 55206.87283 $ & $   0.01640 $ & $   0.00151 $ & $  10.81980 $ & $ i$\\
$ 55206.87346 $ & $   0.01129 $ & $   0.00146 $ & $  10.81600 $ & $ i$\\
$ 55206.87390 $ & $   0.00821 $ & $   0.00133 $ & $  10.81320 $ & $ i$\\
$ 55206.87456 $ & $   0.00994 $ & $   0.00132 $ & $  10.81380 $ & $ i$\\
$ 55206.87499 $ & $   0.00995 $ & $   0.00130 $ & $  10.81470 $ & $ i$\\
$ 55206.87565 $ & $   0.00932 $ & $   0.00129 $ & $  10.81370 $ & $ i$\\
$ 55206.87610 $ & $   0.01091 $ & $   0.00130 $ & $  10.81490 $ & $ i$\\
$ 55206.87675 $ & $   0.01085 $ & $   0.00131 $ & $  10.81530 $ & $ i$\\
$ 55206.87721 $ & $   0.01179 $ & $   0.00132 $ & $  10.81610 $ & $ i$\\
$ 55206.87784 $ & $   0.01364 $ & $   0.00133 $ & $  10.81820 $ & $ i$\\
$ 55206.87826 $ & $   0.01516 $ & $   0.00135 $ & $  10.81910 $ & $ i$\\
$ 55206.87892 $ & $   0.01122 $ & $   0.00141 $ & $  10.81590 $ & $ i$\\
$ 55206.87936 $ & $   0.01269 $ & $   0.00140 $ & $  10.81820 $ & $ i$\\
$ 55206.87999 $ & $   0.01170 $ & $   0.00145 $ & $  10.81650 $ & $ i$\\
$ 55206.88042 $ & $   0.01149 $ & $   0.00142 $ & $  10.81560 $ & $ i$\\
$ 55206.88108 $ & $   0.01420 $ & $   0.00141 $ & $  10.81740 $ & $ i$\\
$ 55206.88153 $ & $   0.01221 $ & $   0.00143 $ & $  10.81580 $ & $ i$\\
$ 55206.88218 $ & $   0.01345 $ & $   0.00144 $ & $  10.81790 $ & $ i$\\
$ 55206.88261 $ & $   0.01085 $ & $   0.00145 $ & $  10.81500 $ & $ i$\\
$ 55206.88326 $ & $   0.01132 $ & $   0.00154 $ & $  10.81560 $ & $ i$\\
$ 55206.88368 $ & $   0.01102 $ & $   0.00179 $ & $  10.81610 $ & $ i$\\
$ 55206.88432 $ & $   0.01090 $ & $   0.00176 $ & $  10.81680 $ & $ i$\\
$ 55206.88477 $ & $   0.01649 $ & $   0.00159 $ & $  10.82050 $ & $ i$\\
$ 55206.88541 $ & $   0.01036 $ & $   0.00162 $ & $  10.81520 $ & $ i$\\
$ 55206.88581 $ & $   0.00976 $ & $   0.00153 $ & $  10.81490 $ & $ i$\\
$ 55206.88648 $ & $   0.01123 $ & $   0.00152 $ & $  10.81570 $ & $ i$\\
$ 55206.88692 $ & $   0.01461 $ & $   0.00156 $ & $  10.81960 $ & $ i$\\
$ 55206.88757 $ & $   0.01508 $ & $   0.00161 $ & $  10.81950 $ & $ i$\\
$ 55206.88802 $ & $   0.01054 $ & $   0.00165 $ & $  10.81520 $ & $ i$\\
$ 55206.88866 $ & $   0.01351 $ & $   0.00164 $ & $  10.81710 $ & $ i$\\
$ 55206.88911 $ & $   0.00838 $ & $   0.00164 $ & $  10.81360 $ & $ i$\\
$ 55206.88975 $ & $   0.01243 $ & $   0.00172 $ & $  10.81720 $ & $ i$\\
$ 55206.89020 $ & $   0.01512 $ & $   0.00169 $ & $  10.81960 $ & $ i$\\
$ 55206.89084 $ & $   0.01355 $ & $   0.00175 $ & $  10.81820 $ & $ i$\\
$ 55206.89129 $ & $   0.01024 $ & $   0.00175 $ & $  10.81410 $ & $ i$\\
$ 55206.89785 $ & $   0.00823 $ & $   0.00178 $ & $  10.81240 $ & $ i$\\
$ 55206.89849 $ & $   0.00674 $ & $   0.00176 $ & $  10.81170 $ & $ i$\\
$ 55206.89893 $ & $   0.01276 $ & $   0.00173 $ & $  10.81650 $ & $ i$\\
$ 55206.89956 $ & $   0.00958 $ & $   0.00176 $ & $  10.81420 $ & $ i$\\
$ 55206.90003 $ & $   0.01039 $ & $   0.00176 $ & $  10.81530 $ & $ i$\\
$ 55206.90390 $ & $   0.00809 $ & $   0.00172 $ & $  10.81210 $ & $ i$\\
$ 55206.90434 $ & $   0.01120 $ & $   0.00170 $ & $  10.81620 $ & $ i$\\
$ 55206.90497 $ & $   0.01585 $ & $   0.00164 $ & $  10.82120 $ & $ i$\\
$ 55206.90541 $ & $   0.01482 $ & $   0.00165 $ & $  10.81860 $ & $ i$\\
$ 55206.90603 $ & $   0.01325 $ & $   0.00159 $ & $  10.81710 $ & $ i$\\
$ 55206.90646 $ & $   0.01129 $ & $   0.00157 $ & $  10.81500 $ & $ i$\\
$ 55206.90710 $ & $   0.01268 $ & $   0.00161 $ & $  10.81580 $ & $ i$\\
$ 55206.90754 $ & $   0.00752 $ & $   0.00167 $ & $  10.81210 $ & $ i$\\
$ 55206.90821 $ & $   0.00680 $ & $   0.00167 $ & $  10.81150 $ & $ i$\\
$ 55206.90864 $ & $   0.01467 $ & $   0.00163 $ & $  10.81940 $ & $ i$\\
$ 55206.90927 $ & $   0.00812 $ & $   0.00157 $ & $  10.81280 $ & $ i$\\
$ 55206.90974 $ & $   0.01199 $ & $   0.00161 $ & $  10.81660 $ & $ i$\\
$ 55206.91039 $ & $   0.01011 $ & $   0.00162 $ & $  10.81390 $ & $ i$\\
$ 55206.91081 $ & $   0.01448 $ & $   0.00163 $ & $  10.81800 $ & $ i$\\
$ 55206.91145 $ & $   0.00894 $ & $   0.00160 $ & $  10.81340 $ & $ i$\\
$ 55206.91189 $ & $   0.01243 $ & $   0.00158 $ & $  10.81620 $ & $ i$\\
$ 55206.91250 $ & $   0.00966 $ & $   0.00162 $ & $  10.81430 $ & $ i$\\
$ 55206.91293 $ & $   0.01149 $ & $   0.00166 $ & $  10.81570 $ & $ i$\\
$ 55206.91359 $ & $   0.01291 $ & $   0.00163 $ & $  10.81740 $ & $ i$\\
$ 55206.91402 $ & $   0.01324 $ & $   0.00161 $ & $  10.81770 $ & $ i$\\
$ 55206.91469 $ & $   0.01369 $ & $   0.00157 $ & $  10.81880 $ & $ i$\\
$ 55206.91513 $ & $   0.01129 $ & $   0.00165 $ & $  10.81580 $ & $ i$\\
$ 55206.91575 $ & $   0.00899 $ & $   0.00165 $ & $  10.81380 $ & $ i$\\
$ 55206.91619 $ & $   0.00937 $ & $   0.00160 $ & $  10.81380 $ & $ i$\\
$ 55206.91682 $ & $   0.00972 $ & $   0.00160 $ & $  10.81320 $ & $ i$\\
$ 55206.91725 $ & $   0.01278 $ & $   0.00158 $ & $  10.81710 $ & $ i$\\
$ 55206.91788 $ & $   0.01361 $ & $   0.00158 $ & $  10.81700 $ & $ i$\\
$ 55206.91834 $ & $   0.01386 $ & $   0.00155 $ & $  10.81860 $ & $ i$\\
$ 55206.91901 $ & $   0.01343 $ & $   0.00155 $ & $  10.81630 $ & $ i$\\
$ 55206.91946 $ & $   0.00885 $ & $   0.00154 $ & $  10.81360 $ & $ i$\\
$ 55206.92010 $ & $   0.01363 $ & $   0.00154 $ & $  10.81780 $ & $ i$\\
$ 55206.92053 $ & $   0.01689 $ & $   0.00149 $ & $  10.82090 $ & $ i$\\
$ 55206.92118 $ & $   0.01160 $ & $   0.00151 $ & $  10.81620 $ & $ i$\\
$ 55206.92163 $ & $   0.01217 $ & $   0.00150 $ & $  10.81610 $ & $ i$\\
$ 55206.92227 $ & $   0.01175 $ & $   0.00152 $ & $  10.81590 $ & $ i$\\
$ 55206.92272 $ & $   0.01206 $ & $   0.00151 $ & $  10.81540 $ & $ i$\\
$ 55206.92336 $ & $   0.01059 $ & $   0.00151 $ & $  10.81520 $ & $ i$\\
$ 55206.92380 $ & $   0.01161 $ & $   0.00152 $ & $  10.81670 $ & $ i$\\
$ 55206.92447 $ & $   0.01145 $ & $   0.00153 $ & $  10.81580 $ & $ i$\\
$ 55206.92492 $ & $   0.01140 $ & $   0.00156 $ & $  10.81580 $ & $ i$\\
$ 55206.92556 $ & $   0.00743 $ & $   0.00156 $ & $  10.81200 $ & $ i$\\
$ 55206.92602 $ & $   0.01200 $ & $   0.00153 $ & $  10.81640 $ & $ i$\\
$ 55206.92663 $ & $   0.01389 $ & $   0.00155 $ & $  10.81800 $ & $ i$\\
$ 55206.92710 $ & $   0.01302 $ & $   0.00155 $ & $  10.81720 $ & $ i$\\
$ 55206.92772 $ & $   0.00892 $ & $   0.00155 $ & $  10.81300 $ & $ i$\\
$ 55206.92817 $ & $   0.01084 $ & $   0.00161 $ & $  10.81570 $ & $ i$\\
$ 55206.92924 $ & $   0.01176 $ & $   0.00154 $ & $  10.81590 $ & $ i$\\
$ 55206.92989 $ & $   0.01078 $ & $   0.00151 $ & $  10.81530 $ & $ i$\\
$ 55206.93033 $ & $   0.01139 $ & $   0.00149 $ & $  10.81560 $ & $ i$\\
$ 55206.93097 $ & $   0.01136 $ & $   0.00148 $ & $  10.81560 $ & $ i$\\
$ 55206.93144 $ & $   0.01290 $ & $   0.00150 $ & $  10.81760 $ & $ i$\\
$ 55206.93207 $ & $   0.01230 $ & $   0.00147 $ & $  10.81620 $ & $ i$\\
$ 55206.93253 $ & $   0.01395 $ & $   0.00146 $ & $  10.81910 $ & $ i$\\
$ 55206.93316 $ & $   0.01214 $ & $   0.00146 $ & $  10.81750 $ & $ i$\\
$ 55206.93363 $ & $   0.01282 $ & $   0.00147 $ & $  10.81610 $ & $ i$\\
$ 55206.93426 $ & $   0.01332 $ & $   0.00147 $ & $  10.81730 $ & $ i$\\
$ 55206.93471 $ & $   0.01173 $ & $   0.00149 $ & $  10.81590 $ & $ i$\\
$ 55206.93540 $ & $   0.00912 $ & $   0.00154 $ & $  10.81330 $ & $ i$\\
$ 55206.93586 $ & $   0.01591 $ & $   0.00156 $ & $  10.82130 $ & $ i$\\
$ 55206.93650 $ & $   0.01024 $ & $   0.00160 $ & $  10.81260 $ & $ i$\\
$ 55206.93691 $ & $   0.00804 $ & $   0.00170 $ & $  10.81210 $ & $ i$\\
$ 55206.93757 $ & $   0.00715 $ & $   0.00170 $ & $  10.81140 $ & $ i$\\
$ 55206.93802 $ & $   0.01182 $ & $   0.00171 $ & $  10.81640 $ & $ i$\\
$ 55206.93865 $ & $   0.01117 $ & $   0.00178 $ & $  10.81500 $ & $ i$\\
$ 55213.61564 $ & $   0.00905 $ & $   0.00103 $ & $  10.65150 $ & $ i$\\
$ 55213.61626 $ & $   0.00783 $ & $   0.00103 $ & $  10.65120 $ & $ i$\\
$ 55213.61688 $ & $   0.00998 $ & $   0.00103 $ & $  10.65080 $ & $ i$\\
$ 55213.61810 $ & $   0.01010 $ & $   0.00103 $ & $  10.65220 $ & $ i$\\
$ 55213.61890 $ & $   0.01592 $ & $   0.00103 $ & $  10.65770 $ & $ i$\\
$ 55213.61951 $ & $   0.01021 $ & $   0.00103 $ & $  10.65350 $ & $ i$\\
$ 55213.62012 $ & $   0.01210 $ & $   0.00102 $ & $  10.65270 $ & $ i$\\
$ 55213.62074 $ & $   0.01505 $ & $   0.00102 $ & $  10.65880 $ & $ i$\\
$ 55213.62136 $ & $   0.01395 $ & $   0.00102 $ & $  10.65590 $ & $ i$\\
$ 55213.62216 $ & $   0.01276 $ & $   0.00102 $ & $  10.65470 $ & $ i$\\
$ 55213.62277 $ & $   0.01062 $ & $   0.00102 $ & $  10.65220 $ & $ i$\\
$ 55213.62339 $ & $   0.01507 $ & $   0.00102 $ & $  10.65740 $ & $ i$\\
$ 55213.62401 $ & $   0.01098 $ & $   0.00102 $ & $  10.65260 $ & $ i$\\
$ 55213.62464 $ & $   0.01089 $ & $   0.00102 $ & $  10.65280 $ & $ i$\\
$ 55213.62547 $ & $   0.01315 $ & $   0.00102 $ & $  10.65440 $ & $ i$\\
$ 55213.62608 $ & $   0.01359 $ & $   0.00102 $ & $  10.65560 $ & $ i$\\
$ 55213.62672 $ & $   0.01283 $ & $   0.00102 $ & $  10.65470 $ & $ i$\\
$ 55213.62735 $ & $   0.01181 $ & $   0.00102 $ & $  10.65500 $ & $ i$\\
$ 55213.62797 $ & $   0.01232 $ & $   0.00102 $ & $  10.65440 $ & $ i$\\
$ 55213.62876 $ & $   0.01235 $ & $   0.00101 $ & $  10.65350 $ & $ i$\\
$ 55213.62938 $ & $   0.01512 $ & $   0.00102 $ & $  10.65580 $ & $ i$\\
$ 55213.63001 $ & $   0.01170 $ & $   0.00102 $ & $  10.65390 $ & $ i$\\
$ 55213.63063 $ & $   0.00872 $ & $   0.00102 $ & $  10.65010 $ & $ i$\\
$ 55213.63127 $ & $   0.01102 $ & $   0.00102 $ & $  10.65180 $ & $ i$\\
$ 55213.63207 $ & $   0.01394 $ & $   0.00101 $ & $  10.65610 $ & $ i$\\
$ 55213.63268 $ & $   0.00958 $ & $   0.00102 $ & $  10.65260 $ & $ i$\\
$ 55213.63330 $ & $   0.01098 $ & $   0.00101 $ & $  10.65320 $ & $ i$\\
$ 55213.63392 $ & $   0.00978 $ & $   0.00101 $ & $  10.65290 $ & $ i$\\
$ 55213.63455 $ & $   0.01158 $ & $   0.00102 $ & $  10.65420 $ & $ i$\\
$ 55213.63537 $ & $   0.00819 $ & $   0.00101 $ & $  10.65110 $ & $ i$\\
$ 55213.63598 $ & $   0.01115 $ & $   0.00101 $ & $  10.65300 $ & $ i$\\
$ 55213.63658 $ & $   0.01618 $ & $   0.00101 $ & $  10.65730 $ & $ i$\\
$ 55213.63718 $ & $   0.01157 $ & $   0.00101 $ & $  10.65410 $ & $ i$\\
$ 55213.63780 $ & $   0.01380 $ & $   0.00101 $ & $  10.65390 $ & $ i$\\
$ 55213.63861 $ & $   0.01235 $ & $   0.00101 $ & $  10.65380 $ & $ i$\\
$ 55213.63923 $ & $   0.00971 $ & $   0.00101 $ & $  10.65210 $ & $ i$\\
$ 55213.63986 $ & $   0.00987 $ & $   0.00101 $ & $  10.65090 $ & $ i$\\
$ 55213.64048 $ & $   0.01040 $ & $   0.00101 $ & $  10.65180 $ & $ i$\\
$ 55213.64111 $ & $   0.01179 $ & $   0.00101 $ & $  10.65370 $ & $ i$\\
$ 55213.64191 $ & $   0.01120 $ & $   0.00100 $ & $  10.65280 $ & $ i$\\
$ 55213.64253 $ & $   0.01512 $ & $   0.00101 $ & $  10.65710 $ & $ i$\\
$ 55213.64314 $ & $   0.01068 $ & $   0.00101 $ & $  10.65240 $ & $ i$\\
$ 55213.64376 $ & $   0.01281 $ & $   0.00100 $ & $  10.65310 $ & $ i$\\
$ 55213.64438 $ & $   0.01399 $ & $   0.00101 $ & $  10.65460 $ & $ i$\\
$ 55213.64522 $ & $   0.01143 $ & $   0.00100 $ & $  10.65300 $ & $ i$\\
$ 55213.64583 $ & $   0.01080 $ & $   0.00100 $ & $  10.65150 $ & $ i$\\
$ 55213.64647 $ & $   0.01204 $ & $   0.00101 $ & $  10.65270 $ & $ i$\\
$ 55213.64709 $ & $   0.00984 $ & $   0.00100 $ & $  10.65210 $ & $ i$\\
$ 55213.64771 $ & $   0.01292 $ & $   0.00100 $ & $  10.65380 $ & $ i$\\
$ 55213.64852 $ & $   0.00876 $ & $   0.00100 $ & $  10.65040 $ & $ i$\\
$ 55213.64913 $ & $   0.00970 $ & $   0.00100 $ & $  10.65070 $ & $ i$\\
$ 55213.64974 $ & $   0.00968 $ & $   0.00100 $ & $  10.65240 $ & $ i$\\
$ 55213.65036 $ & $   0.01152 $ & $   0.00100 $ & $  10.65230 $ & $ i$\\
$ 55213.65099 $ & $   0.00833 $ & $   0.00100 $ & $  10.64930 $ & $ i$\\
$ 55213.65180 $ & $   0.01352 $ & $   0.00100 $ & $  10.65470 $ & $ i$\\
$ 55213.65243 $ & $   0.01289 $ & $   0.00100 $ & $  10.65350 $ & $ i$\\
$ 55213.65304 $ & $   0.01016 $ & $   0.00100 $ & $  10.65040 $ & $ i$\\
$ 55213.65367 $ & $   0.01005 $ & $   0.00100 $ & $  10.65150 $ & $ i$\\
$ 55213.65428 $ & $   0.00766 $ & $   0.00100 $ & $  10.64890 $ & $ i$\\
$ 55213.65509 $ & $   0.01081 $ & $   0.00101 $ & $  10.65200 $ & $ i$\\
$ 55213.65570 $ & $   0.01159 $ & $   0.00100 $ & $  10.65220 $ & $ i$\\
$ 55213.65630 $ & $   0.00893 $ & $   0.00100 $ & $  10.65030 $ & $ i$\\
$ 55213.65692 $ & $   0.00981 $ & $   0.00100 $ & $  10.64910 $ & $ i$\\
$ 55213.65754 $ & $   0.00898 $ & $   0.00100 $ & $  10.65010 $ & $ i$\\
$ 55213.65839 $ & $   0.00818 $ & $   0.00100 $ & $  10.64970 $ & $ i$\\
$ 55213.65900 $ & $   0.01257 $ & $   0.00100 $ & $  10.65290 $ & $ i$\\
$ 55213.65960 $ & $   0.01182 $ & $   0.00101 $ & $  10.65350 $ & $ i$\\
$ 55213.66022 $ & $   0.01061 $ & $   0.00100 $ & $  10.65210 $ & $ i$\\
$ 55213.66083 $ & $   0.01050 $ & $   0.00100 $ & $  10.65290 $ & $ i$\\
$ 55213.66163 $ & $   0.01016 $ & $   0.00100 $ & $  10.65140 $ & $ i$\\
$ 55213.66224 $ & $   0.01026 $ & $   0.00100 $ & $  10.65150 $ & $ i$\\
$ 55213.66286 $ & $   0.01155 $ & $   0.00100 $ & $  10.65280 $ & $ i$\\
$ 55213.66347 $ & $   0.01159 $ & $   0.00100 $ & $  10.65270 $ & $ i$\\
$ 55213.66409 $ & $   0.01150 $ & $   0.00100 $ & $  10.65250 $ & $ i$\\
$ 55213.66490 $ & $   0.01103 $ & $   0.00100 $ & $  10.65280 $ & $ i$\\
$ 55213.66553 $ & $   0.01195 $ & $   0.00101 $ & $  10.65360 $ & $ i$\\
$ 55213.66615 $ & $   0.01107 $ & $   0.00100 $ & $  10.65240 $ & $ i$\\
$ 55213.66676 $ & $   0.01176 $ & $   0.00100 $ & $  10.65390 $ & $ i$\\
$ 55213.66738 $ & $   0.01185 $ & $   0.00100 $ & $  10.65300 $ & $ i$\\
$ 55213.66825 $ & $   0.01241 $ & $   0.00100 $ & $  10.65280 $ & $ i$\\
$ 55213.66887 $ & $   0.00864 $ & $   0.00101 $ & $  10.64990 $ & $ i$\\
$ 55213.66949 $ & $   0.01422 $ & $   0.00101 $ & $  10.65460 $ & $ i$\\
$ 55213.67010 $ & $   0.01201 $ & $   0.00101 $ & $  10.65410 $ & $ i$\\
$ 55213.67071 $ & $   0.01332 $ & $   0.00101 $ & $  10.65440 $ & $ i$\\
$ 55213.67151 $ & $   0.01026 $ & $   0.00101 $ & $  10.65150 $ & $ i$\\
$ 55213.67214 $ & $   0.01039 $ & $   0.00101 $ & $  10.65140 $ & $ i$\\
$ 55213.67276 $ & $   0.00831 $ & $   0.00101 $ & $  10.65040 $ & $ i$\\
$ 55213.67339 $ & $   0.00951 $ & $   0.00103 $ & $  10.65150 $ & $ i$\\
$ 55213.67399 $ & $   0.00984 $ & $   0.00100 $ & $  10.65070 $ & $ i$\\
$ 55213.67479 $ & $   0.01076 $ & $   0.00104 $ & $  10.65150 $ & $ i$\\
$ 55213.67541 $ & $   0.00992 $ & $   0.00102 $ & $  10.65100 $ & $ i$\\
$ 55213.67604 $ & $   0.01189 $ & $   0.00101 $ & $  10.65250 $ & $ i$\\
$ 55213.67665 $ & $   0.00926 $ & $   0.00101 $ & $  10.64980 $ & $ i$\\
$ 55213.67728 $ & $   0.01056 $ & $   0.00100 $ & $  10.65130 $ & $ i$\\
$ 55213.67810 $ & $   0.01136 $ & $   0.00101 $ & $  10.65210 $ & $ i$\\
$ 55213.67872 $ & $   0.00741 $ & $   0.00101 $ & $  10.64790 $ & $ i$\\
$ 55213.67935 $ & $   0.01336 $ & $   0.00106 $ & $  10.65360 $ & $ i$\\
$ 55213.67996 $ & $   0.00957 $ & $   0.00101 $ & $  10.65050 $ & $ i$\\
$ 55213.68057 $ & $   0.01105 $ & $   0.00099 $ & $  10.65040 $ & $ i$\\
$ 55213.68140 $ & $   0.01048 $ & $   0.00100 $ & $  10.65190 $ & $ i$\\
$ 55213.68201 $ & $   0.01030 $ & $   0.00099 $ & $  10.65200 $ & $ i$\\
$ 55213.68263 $ & $   0.00558 $ & $   0.00100 $ & $  10.64660 $ & $ i$\\
$ 55213.68326 $ & $   0.00789 $ & $   0.00099 $ & $  10.64860 $ & $ i$\\
$ 55213.68388 $ & $   0.00899 $ & $   0.00100 $ & $  10.64870 $ & $ i$\\
$ 55213.68468 $ & $   0.00695 $ & $   0.00100 $ & $  10.64760 $ & $ i$\\
$ 55213.68530 $ & $   0.01099 $ & $   0.00100 $ & $  10.65200 $ & $ i$\\
$ 55213.68590 $ & $   0.00829 $ & $   0.00100 $ & $  10.64930 $ & $ i$\\
$ 55213.68651 $ & $   0.01063 $ & $   0.00099 $ & $  10.65070 $ & $ i$\\
$ 55213.68714 $ & $   0.00738 $ & $   0.00099 $ & $  10.64840 $ & $ i$\\
$ 55213.68795 $ & $   0.00531 $ & $   0.00099 $ & $  10.64580 $ & $ i$\\
$ 55213.68858 $ & $   0.00737 $ & $   0.00099 $ & $  10.64760 $ & $ i$\\
$ 55213.68920 $ & $   0.00535 $ & $   0.00099 $ & $  10.64640 $ & $ i$\\
$ 55213.68981 $ & $   0.00587 $ & $   0.00099 $ & $  10.64680 $ & $ i$\\
$ 55213.69044 $ & $   0.00124 $ & $   0.00099 $ & $  10.64200 $ & $ i$\\
$ 55213.69127 $ & $   0.00274 $ & $   0.00099 $ & $  10.64420 $ & $ i$\\
$ 55213.69188 $ & $   0.00439 $ & $   0.00099 $ & $  10.64650 $ & $ i$\\
$ 55213.69251 $ & $   0.00183 $ & $   0.00099 $ & $  10.64300 $ & $ i$\\
$ 55213.69312 $ & $  -0.00031 $ & $   0.00099 $ & $  10.64100 $ & $ i$\\
$ 55213.69373 $ & $   0.00016 $ & $   0.00099 $ & $  10.64060 $ & $ i$\\
$ 55213.69453 $ & $   0.00245 $ & $   0.00100 $ & $  10.64280 $ & $ i$\\
$ 55213.69515 $ & $   0.00213 $ & $   0.00101 $ & $  10.64270 $ & $ i$\\
$ 55213.69575 $ & $  -0.00001 $ & $   0.00106 $ & $  10.64130 $ & $ i$\\
$ 55213.70177 $ & $   0.00258 $ & $   0.00121 $ & $  10.64450 $ & $ i$\\
$ 55213.70239 $ & $  -0.00121 $ & $   0.00114 $ & $  10.64050 $ & $ i$\\
$ 55213.70302 $ & $  -0.00243 $ & $   0.00108 $ & $  10.63900 $ & $ i$\\
$ 55213.70365 $ & $  -0.00155 $ & $   0.00102 $ & $  10.63850 $ & $ i$\\
$ 55213.70447 $ & $  -0.00023 $ & $   0.00103 $ & $  10.64060 $ & $ i$\\
$ 55213.70510 $ & $   0.00127 $ & $   0.00106 $ & $  10.64210 $ & $ i$\\
$ 55213.70571 $ & $   0.00168 $ & $   0.00108 $ & $  10.64130 $ & $ i$\\
$ 55213.70633 $ & $  -0.00140 $ & $   0.00111 $ & $  10.63910 $ & $ i$\\
$ 55213.70773 $ & $   0.00078 $ & $   0.00113 $ & $  10.64170 $ & $ i$\\
$ 55213.71020 $ & $   0.00344 $ & $   0.00120 $ & $  10.64210 $ & $ i$\\
$ 55213.71290 $ & $   0.00037 $ & $   0.00123 $ & $  10.64160 $ & $ i$\\
$ 55213.71351 $ & $  -0.00023 $ & $   0.00123 $ & $  10.63990 $ & $ i$\\
$ 55213.71434 $ & $  -0.00001 $ & $   0.00119 $ & $  10.64300 $ & $ i$\\
$ 55213.71496 $ & $  -0.00115 $ & $   0.00119 $ & $  10.63970 $ & $ i$\\
$ 55213.71556 $ & $  -0.00049 $ & $   0.00107 $ & $  10.64000 $ & $ i$\\
$ 55213.71616 $ & $   0.00094 $ & $   0.00107 $ & $  10.64100 $ & $ i$\\
$ 55213.71680 $ & $   0.00115 $ & $   0.00102 $ & $  10.64020 $ & $ i$\\
$ 55213.71761 $ & $  -0.00037 $ & $   0.00102 $ & $  10.63920 $ & $ i$\\
$ 55213.71822 $ & $   0.00377 $ & $   0.00102 $ & $  10.64220 $ & $ i$\\
$ 55213.71885 $ & $   0.00138 $ & $   0.00106 $ & $  10.64160 $ & $ i$\\
$ 55213.71947 $ & $  -0.00213 $ & $   0.00106 $ & $  10.63830 $ & $ i$\\
$ 55213.72009 $ & $  -0.00006 $ & $   0.00114 $ & $  10.64070 $ & $ i$\\
$ 55213.72149 $ & $  -0.00166 $ & $   0.00115 $ & $  10.63980 $ & $ i$\\
$ 55213.72210 $ & $   0.00392 $ & $   0.00111 $ & $  10.64490 $ & $ i$\\
$ 55213.72273 $ & $   0.00237 $ & $   0.00110 $ & $  10.64330 $ & $ i$\\
$ 55213.72336 $ & $  -0.00037 $ & $   0.00104 $ & $  10.64000 $ & $ i$\\
$ 55213.72420 $ & $  -0.00171 $ & $   0.00111 $ & $  10.63930 $ & $ i$\\
$ 55213.72481 $ & $  -0.00241 $ & $   0.00114 $ & $  10.63870 $ & $ i$\\
$ 55213.72542 $ & $   0.00191 $ & $   0.00107 $ & $  10.64320 $ & $ i$\\
$ 55213.72604 $ & $  -0.00097 $ & $   0.00104 $ & $  10.63960 $ & $ i$\\
$ 55213.72665 $ & $   0.00189 $ & $   0.00106 $ & $  10.64290 $ & $ i$\\
$ 55213.72747 $ & $  -0.00201 $ & $   0.00106 $ & $  10.63810 $ & $ i$\\
$ 55213.72810 $ & $   0.00026 $ & $   0.00111 $ & $  10.64200 $ & $ i$\\
$ 55213.73794 $ & $  -0.00027 $ & $   0.00115 $ & $  10.63940 $ & $ i$\\
$ 55213.73855 $ & $  -0.00016 $ & $   0.00109 $ & $  10.64100 $ & $ i$\\
$ 55213.73919 $ & $  -0.00127 $ & $   0.00109 $ & $  10.63920 $ & $ i$\\
$ 55213.73980 $ & $  -0.00165 $ & $   0.00122 $ & $  10.64000 $ & $ i$\\
$ 55213.74061 $ & $   0.00048 $ & $   0.00108 $ & $  10.64030 $ & $ i$\\
$ 55213.74122 $ & $   0.00278 $ & $   0.00106 $ & $  10.64520 $ & $ i$\\
$ 55213.74184 $ & $   0.00225 $ & $   0.00103 $ & $  10.64230 $ & $ i$\\
$ 55213.74245 $ & $   0.00152 $ & $   0.00100 $ & $  10.64180 $ & $ i$\\
$ 55213.74306 $ & $   0.00229 $ & $   0.00098 $ & $  10.64130 $ & $ i$\\
$ 55213.74390 $ & $   0.00232 $ & $   0.00098 $ & $  10.64210 $ & $ i$\\
$ 55213.74451 $ & $   0.00092 $ & $   0.00098 $ & $  10.64040 $ & $ i$\\
$ 55213.74512 $ & $   0.00010 $ & $   0.00098 $ & $  10.64010 $ & $ i$\\
$ 55213.74572 $ & $  -0.00040 $ & $   0.00098 $ & $  10.64050 $ & $ i$\\
$ 55213.74636 $ & $   0.00085 $ & $   0.00098 $ & $  10.64090 $ & $ i$\\
$ 55213.74718 $ & $  -0.00123 $ & $   0.00098 $ & $  10.63890 $ & $ i$\\
$ 55213.74779 $ & $   0.00036 $ & $   0.00098 $ & $  10.64090 $ & $ i$\\
$ 55213.74839 $ & $   0.00059 $ & $   0.00099 $ & $  10.64050 $ & $ i$\\
$ 55213.74902 $ & $  -0.00034 $ & $   0.00098 $ & $  10.64100 $ & $ i$\\
$ 55213.74966 $ & $   0.00035 $ & $   0.00098 $ & $  10.64120 $ & $ i$\\
$ 55213.75046 $ & $  -0.00117 $ & $   0.00098 $ & $  10.63910 $ & $ i$\\
$ 55213.75107 $ & $   0.00068 $ & $   0.00098 $ & $  10.64160 $ & $ i$\\
$ 55213.75168 $ & $   0.00129 $ & $   0.00098 $ & $  10.64160 $ & $ i$\\
$ 55213.75229 $ & $   0.00096 $ & $   0.00097 $ & $  10.64050 $ & $ i$\\
$ 55213.75290 $ & $   0.00048 $ & $   0.00098 $ & $  10.64010 $ & $ i$\\
$ 55213.75371 $ & $  -0.00178 $ & $   0.00098 $ & $  10.63900 $ & $ i$\\
$ 55213.75434 $ & $  -0.00028 $ & $   0.00098 $ & $  10.64030 $ & $ i$\\
$ 55213.75496 $ & $  -0.00208 $ & $   0.00098 $ & $  10.63890 $ & $ i$\\
$ 55213.75557 $ & $  -0.00016 $ & $   0.00097 $ & $  10.64050 $ & $ i$\\
$ 55213.75619 $ & $  -0.00169 $ & $   0.00098 $ & $  10.63880 $ & $ i$\\
$ 55213.75701 $ & $   0.00144 $ & $   0.00098 $ & $  10.64190 $ & $ i$\\
$ 55213.75761 $ & $  -0.00006 $ & $   0.00098 $ & $  10.64010 $ & $ i$\\
$ 55213.75825 $ & $  -0.00127 $ & $   0.00098 $ & $  10.64040 $ & $ i$\\
$ 55213.75886 $ & $   0.00307 $ & $   0.00098 $ & $  10.64390 $ & $ i$\\
$ 55213.75947 $ & $   0.00164 $ & $   0.00098 $ & $  10.64160 $ & $ i$\\
$ 55213.76028 $ & $   0.00070 $ & $   0.00098 $ & $  10.64110 $ & $ i$\\
$ 55213.76089 $ & $   0.00156 $ & $   0.00098 $ & $  10.64190 $ & $ i$\\
$ 55213.76151 $ & $   0.00145 $ & $   0.00097 $ & $  10.64180 $ & $ i$\\
$ 55213.76214 $ & $   0.00031 $ & $   0.00098 $ & $  10.64150 $ & $ i$\\
$ 55213.76277 $ & $  -0.00100 $ & $   0.00098 $ & $  10.63960 $ & $ i$\\
$ 55213.76358 $ & $  -0.00211 $ & $   0.00098 $ & $  10.63950 $ & $ i$\\
$ 55213.76420 $ & $  -0.00094 $ & $   0.00098 $ & $  10.64000 $ & $ i$\\
$ 55213.76481 $ & $  -0.00013 $ & $   0.00098 $ & $  10.64050 $ & $ i$\\
$ 55213.76540 $ & $  -0.00092 $ & $   0.00097 $ & $  10.64000 $ & $ i$\\
$ 55213.76600 $ & $   0.00081 $ & $   0.00098 $ & $  10.64060 $ & $ i$\\
$ 55213.76685 $ & $   0.00004 $ & $   0.00098 $ & $  10.64020 $ & $ i$\\
$ 55213.76746 $ & $   0.00134 $ & $   0.00098 $ & $  10.64210 $ & $ i$\\
$ 55213.76806 $ & $   0.00069 $ & $   0.00098 $ & $  10.64170 $ & $ i$\\
$ 55213.76868 $ & $  -0.00092 $ & $   0.00098 $ & $  10.63920 $ & $ i$\\
$ 55213.76930 $ & $  -0.00044 $ & $   0.00099 $ & $  10.63920 $ & $ i$\\
$ 55213.77010 $ & $   0.00017 $ & $   0.00102 $ & $  10.64080 $ & $ i$\\
$ 55213.77071 $ & $  -0.00149 $ & $   0.00101 $ & $  10.63970 $ & $ i$\\
$ 55213.77134 $ & $  -0.00320 $ & $   0.00098 $ & $  10.63630 $ & $ i$\\
$ 55213.77195 $ & $  -0.00003 $ & $   0.00098 $ & $  10.63990 $ & $ i$\\
$ 55213.77258 $ & $  -0.00030 $ & $   0.00098 $ & $  10.63930 $ & $ i$\\
$ 55213.77341 $ & $  -0.00220 $ & $   0.00098 $ & $  10.63820 $ & $ i$\\
$ 55213.77405 $ & $   0.00010 $ & $   0.00098 $ & $  10.64210 $ & $ i$\\
$ 55213.77468 $ & $   0.00121 $ & $   0.00101 $ & $  10.64220 $ & $ i$\\
$ 55213.77532 $ & $   0.00065 $ & $   0.00101 $ & $  10.64140 $ & $ i$\\
$ 55213.77594 $ & $  -0.00231 $ & $   0.00108 $ & $  10.64020 $ & $ i$\\
$ 55213.77677 $ & $  -0.00194 $ & $   0.00123 $ & $  10.64230 $ & $ i$\\
$ 55213.77740 $ & $   0.00008 $ & $   0.00119 $ & $  10.64270 $ & $ i$\\
$ 55213.77802 $ & $  -0.00063 $ & $   0.00114 $ & $  10.64080 $ & $ i$\\
$ 55213.77863 $ & $  -0.00163 $ & $   0.00103 $ & $  10.64000 $ & $ i$\\
$ 55213.77924 $ & $  -0.00212 $ & $   0.00100 $ & $  10.63910 $ & $ i$\\
$ 55213.78006 $ & $   0.00103 $ & $   0.00104 $ & $  10.64200 $ & $ i$\\
$ 55213.78070 $ & $  -0.00239 $ & $   0.00112 $ & $  10.64020 $ & $ i$\\
$ 55213.78193 $ & $   0.00024 $ & $   0.00099 $ & $  10.64090 $ & $ i$\\
$ 55213.78256 $ & $  -0.00101 $ & $   0.00098 $ & $  10.63910 $ & $ i$\\
$ 55213.78337 $ & $  -0.00185 $ & $   0.00099 $ & $  10.63880 $ & $ i$\\
$ 55213.78399 $ & $   0.00033 $ & $   0.00098 $ & $  10.64100 $ & $ i$\\
$ 55213.78460 $ & $   0.00047 $ & $   0.00098 $ & $  10.64160 $ & $ i$\\
$ 55213.78521 $ & $   0.00110 $ & $   0.00098 $ & $  10.64300 $ & $ i$\\
$ 55213.78582 $ & $   0.00520 $ & $   0.00100 $ & $  10.64760 $ & $ i$\\
$ 55213.78662 $ & $   0.00172 $ & $   0.00097 $ & $  10.64210 $ & $ i$\\
$ 55213.78724 $ & $  -0.00118 $ & $   0.00097 $ & $  10.63920 $ & $ i$\\
$ 55213.78785 $ & $   0.00102 $ & $   0.00098 $ & $  10.64150 $ & $ i$\\
$ 55213.78848 $ & $   0.00094 $ & $   0.00098 $ & $  10.64140 $ & $ i$\\
$ 55213.78912 $ & $   0.00298 $ & $   0.00098 $ & $  10.64340 $ & $ i$\\
$ 55213.78994 $ & $   0.00004 $ & $   0.00098 $ & $  10.64020 $ & $ i$\\
$ 55213.79056 $ & $   0.00036 $ & $   0.00098 $ & $  10.64140 $ & $ i$\\
$ 55213.79119 $ & $   0.00458 $ & $   0.00099 $ & $  10.64470 $ & $ i$\\
$ 55213.79182 $ & $  -0.00086 $ & $   0.00098 $ & $  10.63860 $ & $ i$\\
$ 55213.79244 $ & $  -0.00107 $ & $   0.00098 $ & $  10.63970 $ & $ i$\\
$ 55213.79324 $ & $  -0.00035 $ & $   0.00098 $ & $  10.64100 $ & $ i$\\
$ 55213.79386 $ & $  -0.00222 $ & $   0.00098 $ & $  10.63920 $ & $ i$\\
$ 55213.79449 $ & $   0.00005 $ & $   0.00097 $ & $  10.64130 $ & $ i$\\
$ 55213.79511 $ & $  -0.00164 $ & $   0.00098 $ & $  10.63910 $ & $ i$\\
$ 55213.79574 $ & $  -0.00181 $ & $   0.00098 $ & $  10.63930 $ & $ i$\\
$ 55213.79653 $ & $  -0.00089 $ & $   0.00098 $ & $  10.64020 $ & $ i$\\
$ 55233.59370 $ & $  -0.00158 $ & $   0.00135 $ & $  10.64150 $ & $ i$\\
$ 55233.59415 $ & $  -0.00214 $ & $   0.00140 $ & $  10.64030 $ & $ i$\\
$ 55233.59476 $ & $   0.00469 $ & $   0.00133 $ & $  10.65150 $ & $ i$\\
$ 55233.59521 $ & $  -0.00314 $ & $   0.00134 $ & $  10.64220 $ & $ i$\\
$ 55233.59796 $ & $  -0.00108 $ & $   0.00133 $ & $  10.64880 $ & $ i$\\
$ 55233.59840 $ & $   0.00515 $ & $   0.00132 $ & $  10.64970 $ & $ i$\\
$ 55233.59905 $ & $  -0.00009 $ & $   0.00131 $ & $  10.64710 $ & $ i$\\
$ 55233.59950 $ & $   0.00136 $ & $   0.00130 $ & $  10.64780 $ & $ i$\\
$ 55233.60011 $ & $   0.00143 $ & $   0.00130 $ & $  10.64730 $ & $ i$\\
$ 55233.60056 $ & $  -0.00176 $ & $   0.00130 $ & $  10.64550 $ & $ i$\\
$ 55233.60120 $ & $  -0.00468 $ & $   0.00131 $ & $  10.64150 $ & $ i$\\
$ 55233.60376 $ & $   0.00123 $ & $   0.00131 $ & $  10.64710 $ & $ i$\\
$ 55233.60439 $ & $   0.00187 $ & $   0.00130 $ & $  10.64930 $ & $ i$\\
$ 55233.60484 $ & $   0.00122 $ & $   0.00129 $ & $  10.64600 $ & $ i$\\
$ 55233.60546 $ & $   0.00006 $ & $   0.00130 $ & $  10.64630 $ & $ i$\\
$ 55233.60591 $ & $   0.00031 $ & $   0.00130 $ & $  10.64340 $ & $ i$\\
$ 55233.60652 $ & $   0.00138 $ & $   0.00130 $ & $  10.64550 $ & $ i$\\
$ 55233.60697 $ & $   0.00099 $ & $   0.00131 $ & $  10.64680 $ & $ i$\\
$ 55233.60759 $ & $  -0.00238 $ & $   0.00132 $ & $  10.64340 $ & $ i$\\
$ 55233.60805 $ & $  -0.00080 $ & $   0.00131 $ & $  10.64450 $ & $ i$\\
$ 55233.60865 $ & $  -0.00264 $ & $   0.00129 $ & $  10.64290 $ & $ i$\\
$ 55233.60910 $ & $   0.00020 $ & $   0.00129 $ & $  10.64640 $ & $ i$\\
$ 55233.60975 $ & $  -0.00095 $ & $   0.00129 $ & $  10.64670 $ & $ i$\\
$ 55233.61021 $ & $  -0.00238 $ & $   0.00132 $ & $  10.63620 $ & $ i$\\
$ 55233.61131 $ & $   0.00312 $ & $   0.00140 $ & $  10.65070 $ & $ i$\\
$ 55233.61344 $ & $  -0.00085 $ & $   0.00139 $ & $  10.64090 $ & $ i$\\
$ 55233.62487 $ & $   0.00063 $ & $   0.00128 $ & $  10.64700 $ & $ i$\\
$ 55233.62533 $ & $  -0.00201 $ & $   0.00129 $ & $  10.64540 $ & $ i$\\
$ 55233.63636 $ & $   0.00311 $ & $   0.00142 $ & $  10.64690 $ & $ i$\\
$ 55233.63681 $ & $  -0.00403 $ & $   0.00133 $ & $  10.64250 $ & $ i$\\
$ 55233.63742 $ & $  -0.00008 $ & $   0.00131 $ & $  10.64710 $ & $ i$\\
$ 55233.63786 $ & $   0.00115 $ & $   0.00134 $ & $  10.64570 $ & $ i$\\
$ 55233.63849 $ & $   0.00004 $ & $   0.00141 $ & $  10.64850 $ & $ i$\\
$ 55233.63894 $ & $   0.00001 $ & $   0.00138 $ & $  10.64970 $ & $ i$\\
$ 55233.63959 $ & $   0.00240 $ & $   0.00138 $ & $  10.64920 $ & $ i$\\
$ 55233.66165 $ & $   0.00386 $ & $   0.00132 $ & $  10.65190 $ & $ i$\\
$ 55233.66227 $ & $  -0.00015 $ & $   0.00132 $ & $  10.64560 $ & $ i$\\
$ 55233.66272 $ & $  -0.00014 $ & $   0.00132 $ & $  10.64630 $ & $ i$\\
$ 55233.66334 $ & $  -0.00160 $ & $   0.00128 $ & $  10.64480 $ & $ i$\\
$ 55233.66380 $ & $   0.00025 $ & $   0.00133 $ & $  10.64520 $ & $ i$\\
$ 55233.66555 $ & $   0.00045 $ & $   0.00132 $ & $  10.64580 $ & $ i$\\
$ 55233.66600 $ & $  -0.00069 $ & $   0.00130 $ & $  10.64670 $ & $ i$\\
$ 55233.66661 $ & $  -0.00095 $ & $   0.00130 $ & $  10.64730 $ & $ i$\\
$ 55233.66708 $ & $   0.00299 $ & $   0.00128 $ & $  10.64830 $ & $ i$\\
$ 55233.66770 $ & $  -0.00056 $ & $   0.00128 $ & $  10.64500 $ & $ i$\\
$ 55233.66814 $ & $   0.00003 $ & $   0.00128 $ & $  10.64510 $ & $ i$\\
$ 55233.66876 $ & $  -0.00275 $ & $   0.00129 $ & $  10.64390 $ & $ i$\\
$ 55233.66922 $ & $  -0.00313 $ & $   0.00128 $ & $  10.64380 $ & $ i$\\
$ 55233.66985 $ & $   0.00033 $ & $   0.00131 $ & $  10.64660 $ & $ i$\\
$ 55233.67030 $ & $  -0.00244 $ & $   0.00134 $ & $  10.64280 $ & $ i$\\
$ 55233.68070 $ & $  -0.00274 $ & $   0.00137 $ & $  10.64180 $ & $ i$\\
$ 55233.68374 $ & $   0.00679 $ & $   0.00138 $ & $  10.65180 $ & $ i$\\
$ 55233.68435 $ & $   0.00598 $ & $   0.00138 $ & $  10.65270 $ & $ i$\\
$ 55233.68479 $ & $   0.00458 $ & $   0.00132 $ & $  10.65050 $ & $ i$\\
$ 55233.68544 $ & $   0.00435 $ & $   0.00132 $ & $  10.65160 $ & $ i$\\
$ 55233.68588 $ & $   0.00166 $ & $   0.00133 $ & $  10.64590 $ & $ i$\\
$ 55233.68651 $ & $   0.00802 $ & $   0.00128 $ & $  10.65430 $ & $ i$\\
$ 55233.68696 $ & $   0.00951 $ & $   0.00130 $ & $  10.65520 $ & $ i$\\
$ 55233.68757 $ & $   0.00513 $ & $   0.00128 $ & $  10.65210 $ & $ i$\\
$ 55233.68801 $ & $   0.01013 $ & $   0.00127 $ & $  10.65670 $ & $ i$\\
$ 55233.68864 $ & $   0.00755 $ & $   0.00128 $ & $  10.65420 $ & $ i$\\
$ 55233.68909 $ & $   0.01245 $ & $   0.00128 $ & $  10.65750 $ & $ i$\\
$ 55233.68969 $ & $   0.01114 $ & $   0.00128 $ & $  10.65780 $ & $ i$\\
$ 55233.69015 $ & $   0.00822 $ & $   0.00128 $ & $  10.65450 $ & $ i$\\
$ 55233.69079 $ & $   0.00688 $ & $   0.00128 $ & $  10.65250 $ & $ i$\\
$ 55233.69124 $ & $   0.00736 $ & $   0.00128 $ & $  10.65430 $ & $ i$\\
$ 55233.69184 $ & $   0.00907 $ & $   0.00128 $ & $  10.65630 $ & $ i$\\
$ 55233.69231 $ & $   0.00972 $ & $   0.00128 $ & $  10.65550 $ & $ i$\\
$ 55233.69291 $ & $   0.01350 $ & $   0.00128 $ & $  10.65970 $ & $ i$\\
$ 55233.69334 $ & $   0.01276 $ & $   0.00128 $ & $  10.65960 $ & $ i$\\
$ 55233.69397 $ & $   0.00739 $ & $   0.00128 $ & $  10.65430 $ & $ i$\\
$ 55233.69445 $ & $   0.01061 $ & $   0.00128 $ & $  10.65610 $ & $ i$\\
$ 55233.69508 $ & $   0.01162 $ & $   0.00129 $ & $  10.65690 $ & $ i$\\
$ 55233.69556 $ & $   0.00900 $ & $   0.00129 $ & $  10.65560 $ & $ i$\\
$ 55233.69621 $ & $   0.01129 $ & $   0.00128 $ & $  10.65790 $ & $ i$\\
$ 55233.69666 $ & $   0.01242 $ & $   0.00129 $ & $  10.65820 $ & $ i$\\
$ 55233.69727 $ & $   0.01326 $ & $   0.00129 $ & $  10.65970 $ & $ i$\\
$ 55233.69772 $ & $   0.01235 $ & $   0.00129 $ & $  10.65870 $ & $ i$\\
$ 55233.69833 $ & $   0.01102 $ & $   0.00128 $ & $  10.65770 $ & $ i$\\
$ 55233.69879 $ & $   0.00903 $ & $   0.00129 $ & $  10.65480 $ & $ i$\\
$ 55233.69940 $ & $   0.00903 $ & $   0.00129 $ & $  10.65700 $ & $ i$\\
$ 55233.69985 $ & $   0.01263 $ & $   0.00129 $ & $  10.65870 $ & $ i$\\
$ 55233.70046 $ & $   0.00848 $ & $   0.00128 $ & $  10.65590 $ & $ i$\\
$ 55233.70092 $ & $   0.01156 $ & $   0.00129 $ & $  10.65780 $ & $ i$\\
$ 55233.70155 $ & $   0.00956 $ & $   0.00129 $ & $  10.65690 $ & $ i$\\
$ 55233.70199 $ & $   0.01091 $ & $   0.00128 $ & $  10.65790 $ & $ i$\\
$ 55233.70261 $ & $   0.01206 $ & $   0.00129 $ & $  10.65870 $ & $ i$\\
$ 55233.70306 $ & $   0.01360 $ & $   0.00129 $ & $  10.65960 $ & $ i$\\
$ 55233.70368 $ & $   0.01021 $ & $   0.00129 $ & $  10.65680 $ & $ i$\\
$ 55233.70413 $ & $   0.00985 $ & $   0.00129 $ & $  10.65610 $ & $ i$\\
$ 55233.70475 $ & $   0.00995 $ & $   0.00129 $ & $  10.65650 $ & $ i$\\
$ 55233.70521 $ & $   0.01092 $ & $   0.00129 $ & $  10.65670 $ & $ i$\\
$ 55233.70583 $ & $   0.01468 $ & $   0.00129 $ & $  10.66140 $ & $ i$\\
$ 55233.70629 $ & $   0.00934 $ & $   0.00129 $ & $  10.65690 $ & $ i$\\
$ 55233.70692 $ & $   0.01233 $ & $   0.00129 $ & $  10.65750 $ & $ i$\\
$ 55233.70739 $ & $   0.00905 $ & $   0.00129 $ & $  10.65630 $ & $ i$\\
$ 55233.70801 $ & $   0.00986 $ & $   0.00129 $ & $  10.65600 $ & $ i$\\
$ 55233.70844 $ & $   0.00958 $ & $   0.00129 $ & $  10.65690 $ & $ i$\\
$ 55233.70905 $ & $   0.01192 $ & $   0.00129 $ & $  10.65870 $ & $ i$\\
$ 55233.70950 $ & $   0.01229 $ & $   0.00129 $ & $  10.65870 $ & $ i$\\
$ 55233.71012 $ & $   0.00632 $ & $   0.00129 $ & $  10.65310 $ & $ i$\\
$ 55233.71057 $ & $   0.00963 $ & $   0.00129 $ & $  10.65750 $ & $ i$\\
$ 55233.71118 $ & $   0.01097 $ & $   0.00131 $ & $  10.65670 $ & $ i$\\
$ 55233.71162 $ & $   0.01223 $ & $   0.00135 $ & $  10.65940 $ & $ i$\\
$ 55233.71227 $ & $   0.01316 $ & $   0.00134 $ & $  10.65940 $ & $ i$\\
$ 55233.71272 $ & $   0.01180 $ & $   0.00133 $ & $  10.65810 $ & $ i$\\
$ 55233.71333 $ & $   0.01227 $ & $   0.00131 $ & $  10.65720 $ & $ i$\\
$ 55233.71379 $ & $   0.01200 $ & $   0.00132 $ & $  10.65890 $ & $ i$\\
$ 55233.71440 $ & $   0.01102 $ & $   0.00130 $ & $  10.65770 $ & $ i$\\
$ 55233.71485 $ & $   0.01012 $ & $   0.00130 $ & $  10.65780 $ & $ i$\\
$ 55233.71546 $ & $   0.01405 $ & $   0.00130 $ & $  10.65980 $ & $ i$\\
$ 55233.71590 $ & $   0.00996 $ & $   0.00130 $ & $  10.65690 $ & $ i$\\
$ 55233.71652 $ & $   0.01125 $ & $   0.00130 $ & $  10.65720 $ & $ i$\\
$ 55233.71696 $ & $   0.00972 $ & $   0.00130 $ & $  10.65610 $ & $ i$\\
$ 55233.71761 $ & $   0.01222 $ & $   0.00130 $ & $  10.65750 $ & $ i$\\
$ 55233.71806 $ & $   0.01202 $ & $   0.00130 $ & $  10.65840 $ & $ i$\\
$ 55233.71869 $ & $   0.01164 $ & $   0.00130 $ & $  10.65800 $ & $ i$\\
$ 55233.71913 $ & $   0.00874 $ & $   0.00131 $ & $  10.65590 $ & $ i$\\
$ 55233.71975 $ & $   0.00715 $ & $   0.00134 $ & $  10.65350 $ & $ i$\\
$ 55233.72020 $ & $   0.00736 $ & $   0.00136 $ & $  10.65510 $ & $ i$\\
$ 55233.72185 $ & $   0.01020 $ & $   0.00135 $ & $  10.65710 $ & $ i$\\
$ 55233.72230 $ & $   0.01351 $ & $   0.00135 $ & $  10.66040 $ & $ i$\\
$ 55233.72295 $ & $   0.01188 $ & $   0.00133 $ & $  10.65730 $ & $ i$\\
$ 55233.72340 $ & $   0.00945 $ & $   0.00133 $ & $  10.65520 $ & $ i$\\
$ 55233.72402 $ & $   0.00776 $ & $   0.00134 $ & $  10.65440 $ & $ i$\\
$ 55233.72446 $ & $   0.00789 $ & $   0.00135 $ & $  10.65520 $ & $ i$\\
$ 55233.72508 $ & $   0.01294 $ & $   0.00136 $ & $  10.65800 $ & $ i$\\
$ 55233.72553 $ & $   0.00662 $ & $   0.00137 $ & $  10.64210 $ & $ i$\\
$ 55233.72613 $ & $   0.01063 $ & $   0.00132 $ & $  10.65580 $ & $ i$\\
$ 55233.72659 $ & $   0.01129 $ & $   0.00137 $ & $  10.65600 $ & $ i$\\
$ 55233.72721 $ & $   0.01578 $ & $   0.00137 $ & $  10.65990 $ & $ i$\\
$ 55233.72766 $ & $   0.01395 $ & $   0.00139 $ & $  10.66580 $ & $ i$\\
$ 55233.72830 $ & $   0.01398 $ & $   0.00139 $ & $  10.66540 $ & $ i$\\
$ 55233.72936 $ & $   0.01035 $ & $   0.00133 $ & $  10.65440 $ & $ i$\\
$ 55233.72982 $ & $   0.00984 $ & $   0.00133 $ & $  10.65600 $ & $ i$\\
$ 55233.73043 $ & $   0.01495 $ & $   0.00134 $ & $  10.66140 $ & $ i$\\
$ 55233.73088 $ & $   0.01058 $ & $   0.00140 $ & $  10.65750 $ & $ i$\\
$ 55233.73301 $ & $   0.00798 $ & $   0.00138 $ & $  10.65060 $ & $ i$\\
$ 55233.73365 $ & $   0.01209 $ & $   0.00133 $ & $  10.65890 $ & $ i$\\
$ 55233.73409 $ & $   0.01145 $ & $   0.00136 $ & $  10.66110 $ & $ i$\\
$ 55233.73471 $ & $   0.01085 $ & $   0.00132 $ & $  10.65810 $ & $ i$\\
$ 55233.73516 $ & $   0.00704 $ & $   0.00131 $ & $  10.65490 $ & $ i$\\
$ 55233.73576 $ & $   0.01005 $ & $   0.00131 $ & $  10.65730 $ & $ i$\\
$ 55233.73619 $ & $   0.01440 $ & $   0.00131 $ & $  10.66210 $ & $ i$\\
$ 55233.73682 $ & $   0.01633 $ & $   0.00131 $ & $  10.66220 $ & $ i$\\
$ 55233.73727 $ & $   0.01453 $ & $   0.00131 $ & $  10.66240 $ & $ i$\\
$ 55233.73788 $ & $   0.00914 $ & $   0.00131 $ & $  10.65630 $ & $ i$\\
$ 55233.73832 $ & $   0.01006 $ & $   0.00131 $ & $  10.65780 $ & $ i$\\
$ 55233.73897 $ & $   0.01113 $ & $   0.00131 $ & $  10.65800 $ & $ i$\\
$ 55233.73941 $ & $   0.01454 $ & $   0.00131 $ & $  10.66180 $ & $ i$\\
$ 55233.74004 $ & $   0.01192 $ & $   0.00130 $ & $  10.65890 $ & $ i$\\
$ 55233.74049 $ & $   0.01148 $ & $   0.00131 $ & $  10.65970 $ & $ i$\\
$ 55233.74109 $ & $   0.01325 $ & $   0.00132 $ & $  10.66030 $ & $ i$\\
$ 55233.74153 $ & $   0.01634 $ & $   0.00132 $ & $  10.66350 $ & $ i$\\
$ 55233.74214 $ & $   0.01245 $ & $   0.00131 $ & $  10.66030 $ & $ i$\\
$ 55233.74258 $ & $   0.01246 $ & $   0.00132 $ & $  10.65920 $ & $ i$\\
$ 55233.74319 $ & $   0.01395 $ & $   0.00131 $ & $  10.66130 $ & $ i$\\
$ 55233.74365 $ & $   0.00949 $ & $   0.00131 $ & $  10.65700 $ & $ i$\\
$ 55233.74429 $ & $   0.01030 $ & $   0.00132 $ & $  10.65630 $ & $ i$\\
$ 55233.74473 $ & $   0.01357 $ & $   0.00132 $ & $  10.66070 $ & $ i$\\
$ 55233.74536 $ & $   0.01164 $ & $   0.00132 $ & $  10.65850 $ & $ i$\\
$ 55233.74580 $ & $   0.01104 $ & $   0.00132 $ & $  10.65920 $ & $ i$\\
$ 55233.74641 $ & $   0.01441 $ & $   0.00132 $ & $  10.66280 $ & $ i$\\
$ 55233.74687 $ & $   0.00740 $ & $   0.00132 $ & $  10.65650 $ & $ i$\\
$ 55233.74749 $ & $   0.01130 $ & $   0.00132 $ & $  10.65780 $ & $ i$\\
$ 55233.74795 $ & $   0.01166 $ & $   0.00133 $ & $  10.65850 $ & $ i$\\
$ 55233.74855 $ & $   0.01386 $ & $   0.00132 $ & $  10.66110 $ & $ i$\\
$ 55233.74900 $ & $   0.01350 $ & $   0.00132 $ & $  10.65990 $ & $ i$\\
$ 55233.74964 $ & $   0.00802 $ & $   0.00132 $ & $  10.65500 $ & $ i$\\
$ 55233.75008 $ & $   0.01126 $ & $   0.00133 $ & $  10.66020 $ & $ i$\\
$ 55233.75071 $ & $   0.01041 $ & $   0.00132 $ & $  10.65870 $ & $ i$\\
$ 55233.75116 $ & $   0.01400 $ & $   0.00133 $ & $  10.66180 $ & $ i$\\
$ 55233.75177 $ & $   0.01288 $ & $   0.00133 $ & $  10.65950 $ & $ i$\\
$ 55233.75223 $ & $   0.01418 $ & $   0.00133 $ & $  10.66030 $ & $ i$\\
$ 55233.75286 $ & $   0.01079 $ & $   0.00132 $ & $  10.65810 $ & $ i$\\
$ 55233.75331 $ & $   0.00988 $ & $   0.00132 $ & $  10.65710 $ & $ i$\\
$ 55233.75395 $ & $   0.01314 $ & $   0.00133 $ & $  10.66130 $ & $ i$\\
$ 55233.75440 $ & $   0.01268 $ & $   0.00133 $ & $  10.66060 $ & $ i$\\
$ 55233.75507 $ & $   0.01100 $ & $   0.00133 $ & $  10.65790 $ & $ i$\\
$ 55233.75552 $ & $   0.01055 $ & $   0.00133 $ & $  10.65830 $ & $ i$\\
$ 55233.75612 $ & $   0.01092 $ & $   0.00133 $ & $  10.65800 $ & $ i$\\
$ 55233.75657 $ & $   0.01252 $ & $   0.00133 $ & $  10.65970 $ & $ i$\\
$ 55233.75720 $ & $   0.01140 $ & $   0.00133 $ & $  10.65740 $ & $ i$\\
$ 55233.75765 $ & $   0.01172 $ & $   0.00133 $ & $  10.66050 $ & $ i$\\
$ 55233.75826 $ & $   0.01144 $ & $   0.00132 $ & $  10.65980 $ & $ i$\\
$ 55233.75870 $ & $   0.00920 $ & $   0.00133 $ & $  10.65730 $ & $ i$\\
$ 55233.75932 $ & $   0.00774 $ & $   0.00133 $ & $  10.65520 $ & $ i$\\
$ 55233.75978 $ & $   0.01077 $ & $   0.00133 $ & $  10.65940 $ & $ i$\\
$ 55233.76044 $ & $   0.01326 $ & $   0.00135 $ & $  10.66090 $ & $ i$\\
$ 55233.76089 $ & $   0.01087 $ & $   0.00135 $ & $  10.66010 $ & $ i$\\
$ 55233.76150 $ & $   0.01230 $ & $   0.00135 $ & $  10.66020 $ & $ i$\\
$ 55233.76197 $ & $   0.01089 $ & $   0.00137 $ & $  10.65890 $ & $ i$\\
$ 55233.76900 $ & $   0.01067 $ & $   0.00140 $ & $  10.66050 $ & $ i$\\
$ 55233.76945 $ & $   0.01222 $ & $   0.00137 $ & $  10.65890 $ & $ i$\\
$ 55233.79082 $ & $   0.01085 $ & $   0.00152 $ & $  10.66250 $ & $ i$\\
$ 55233.79125 $ & $   0.00693 $ & $   0.00141 $ & $  10.65310 $ & $ i$\\
$ 55233.79186 $ & $   0.00861 $ & $   0.00141 $ & $  10.65630 $ & $ i$\\
$ 55233.79231 $ & $   0.00733 $ & $   0.00141 $ & $  10.65700 $ & $ i$\\
$ 55233.79293 $ & $   0.01044 $ & $   0.00140 $ & $  10.65740 $ & $ i$\\
$ 55233.79337 $ & $   0.01024 $ & $   0.00140 $ & $  10.65780 $ & $ i$\\
$ 55233.79399 $ & $   0.00850 $ & $   0.00145 $ & $  10.65270 $ & $ i$\\
$ 55233.79445 $ & $   0.01201 $ & $   0.00144 $ & $  10.65920 $ & $ i$\\
$ 55233.79506 $ & $   0.01167 $ & $   0.00147 $ & $  10.65780 $ & $ i$\\
$ 55233.79551 $ & $   0.01145 $ & $   0.00142 $ & $  10.65920 $ & $ i$\\
$ 55233.79614 $ & $   0.01343 $ & $   0.00143 $ & $  10.66070 $ & $ i$\\
$ 55233.79661 $ & $   0.01313 $ & $   0.00145 $ & $  10.65890 $ & $ i$\\
$ 55233.79723 $ & $   0.00749 $ & $   0.00144 $ & $  10.65420 $ & $ i$\\
$ 55233.79768 $ & $   0.00964 $ & $   0.00143 $ & $  10.65680 $ & $ i$\\
$ 55233.79830 $ & $   0.01114 $ & $   0.00143 $ & $  10.65780 $ & $ i$\\
$ 55233.79875 $ & $   0.01331 $ & $   0.00144 $ & $  10.66190 $ & $ i$\\
$ 55233.79937 $ & $   0.00961 $ & $   0.00145 $ & $  10.65730 $ & $ i$\\
$ 55233.79982 $ & $   0.01661 $ & $   0.00146 $ & $  10.66270 $ & $ i$\\
$ 55233.80044 $ & $   0.01183 $ & $   0.00145 $ & $  10.65900 $ & $ i$\\
$ 55233.80089 $ & $   0.00941 $ & $   0.00146 $ & $  10.65560 $ & $ i$\\
$ 55233.80153 $ & $   0.01067 $ & $   0.00148 $ & $  10.65900 $ & $ i$\\
$ 55233.80194 $ & $   0.01066 $ & $   0.00146 $ & $  10.65540 $ & $ i$\\
$ 55233.80257 $ & $   0.00618 $ & $   0.00146 $ & $  10.65150 $ & $ i$\\
$ 55233.80303 $ & $   0.00873 $ & $   0.00148 $ & $  10.65630 $ & $ i$\\
$ 55233.80365 $ & $   0.01256 $ & $   0.00148 $ & $  10.65790 $ & $ i$\\
$ 55233.80411 $ & $   0.01168 $ & $   0.00149 $ & $  10.65800 $ & $ i$\\
$ 55233.80473 $ & $   0.00941 $ & $   0.00152 $ & $  10.65590 $ & $ i$\\
$ 55233.80518 $ & $   0.00955 $ & $   0.00151 $ & $  10.65620 $ & $ i$\\
$ 55233.80581 $ & $   0.00882 $ & $   0.00151 $ & $  10.65800 $ & $ i$\\
$ 55233.80626 $ & $   0.01396 $ & $   0.00150 $ & $  10.66110 $ & $ i$\\
$ 55233.80689 $ & $   0.01187 $ & $   0.00148 $ & $  10.65780 $ & $ i$\\
$ 55233.80735 $ & $   0.01388 $ & $   0.00148 $ & $  10.66050 $ & $ i$\\
$ 55233.80796 $ & $   0.01037 $ & $   0.00148 $ & $  10.65740 $ & $ i$\\
$ 55233.80841 $ & $   0.00698 $ & $   0.00147 $ & $  10.65470 $ & $ i$\\
$ 55233.80902 $ & $   0.00978 $ & $   0.00154 $ & $  10.65410 $ & $ i$\\
$ 55233.86332 $ & $   0.00261 $ & $   0.00150 $ & $  10.65440 $ & $ i$\\
$ 55233.86379 $ & $  -0.00258 $ & $   0.00149 $ & $  10.64050 $ & $ i$\\
$ 55233.86442 $ & $   0.00312 $ & $   0.00145 $ & $  10.64920 $ & $ i$\\
$ 55233.86487 $ & $  -0.00023 $ & $   0.00142 $ & $  10.64340 $ & $ i$\\
$ 55233.86547 $ & $   0.00010 $ & $   0.00144 $ & $  10.64720 $ & $ i$\\
$ 55233.86592 $ & $   0.00160 $ & $   0.00136 $ & $  10.64550 $ & $ i$\\
$ 55233.86657 $ & $  -0.00373 $ & $   0.00142 $ & $  10.63660 $ & $ i$\\
$ 55233.86703 $ & $   0.00092 $ & $   0.00150 $ & $  10.64720 $ & $ i$\\
$ 55233.86766 $ & $   0.00189 $ & $   0.00147 $ & $  10.64810 $ & $ i$\\
$ 55233.86811 $ & $  -0.00101 $ & $   0.00142 $ & $  10.64830 $ & $ i$\\
$ 55233.86872 $ & $   0.00028 $ & $   0.00144 $ & $  10.64440 $ & $ i$\\
$ 55233.86917 $ & $   0.00316 $ & $   0.00146 $ & $  10.65090 $ & $ i$\\
$ 55233.86978 $ & $   0.00294 $ & $   0.00139 $ & $  10.64230 $ & $ i$\\
$ 55233.87024 $ & $   0.00190 $ & $   0.00138 $ & $  10.64960 $ & $ i$\\
$ 55233.87085 $ & $  -0.00080 $ & $   0.00136 $ & $  10.64360 $ & $ i$\\
$ 55233.87129 $ & $  -0.00636 $ & $   0.00137 $ & $  10.62570 $ & $ i$\\
$ 55233.87194 $ & $   0.00118 $ & $   0.00153 $ & $  10.64480 $ & $ i$\\
$ 55233.87239 $ & $  -0.00300 $ & $   0.00139 $ & $  10.63360 $ & $ i$\\
$ 55233.87300 $ & $   0.00006 $ & $   0.00138 $ & $  10.63860 $ & $ i$\\
$ 55233.87343 $ & $   0.00115 $ & $   0.00142 $ & $  10.64980 $ & $ i$\\
$ 55233.87404 $ & $   0.00233 $ & $   0.00134 $ & $  10.63380 $ & $ i$\\
$ 55233.87446 $ & $  -0.00351 $ & $   0.00134 $ & $  10.63680 $ & $ i$\\
$ 55233.87509 $ & $   0.00129 $ & $   0.00136 $ & $  10.64210 $ & $ i$\\
$ 55233.87555 $ & $   0.00056 $ & $   0.00137 $ & $  10.64290 $ & $ i$\\
$ 55233.87726 $ & $   0.00061 $ & $   0.00144 $ & $  10.64710 $ & $ i$\\
$ 55233.87772 $ & $  -0.00100 $ & $   0.00156 $ & $  10.63560 $ & $ i$\\
$ 55233.87835 $ & $  -0.00053 $ & $   0.00154 $ & $  10.66140 $ & $ i$\\
$ 55243.72943 $ & $   0.00153 $ & $   0.00090 $ & $   9.16218 $ & $ i$\\
$ 55243.72979 $ & $   0.00040 $ & $   0.00090 $ & $   9.16132 $ & $ i$\\
$ 55243.73013 $ & $   0.00200 $ & $   0.00090 $ & $   9.16304 $ & $ i$\\
$ 55243.73048 $ & $   0.00143 $ & $   0.00090 $ & $   9.16218 $ & $ i$\\
$ 55243.73083 $ & $  -0.00022 $ & $   0.00090 $ & $   9.16034 $ & $ i$\\
$ 55243.73118 $ & $  -0.00186 $ & $   0.00090 $ & $   9.15942 $ & $ i$\\
$ 55243.73153 $ & $   0.00033 $ & $   0.00090 $ & $   9.16111 $ & $ i$\\
$ 55243.73189 $ & $   0.00227 $ & $   0.00090 $ & $   9.16358 $ & $ i$\\
$ 55243.73224 $ & $   0.00247 $ & $   0.00090 $ & $   9.16328 $ & $ i$\\
$ 55243.73259 $ & $   0.00037 $ & $   0.00090 $ & $   9.16009 $ & $ i$\\
$ 55243.73295 $ & $   0.00123 $ & $   0.00090 $ & $   9.16190 $ & $ i$\\
$ 55243.73333 $ & $  -0.00093 $ & $   0.00090 $ & $   9.16046 $ & $ i$\\
$ 55243.73372 $ & $   0.00071 $ & $   0.00090 $ & $   9.16006 $ & $ i$\\
$ 55243.73447 $ & $   0.00038 $ & $   0.00090 $ & $   9.16009 $ & $ i$\\
$ 55243.73483 $ & $   0.00094 $ & $   0.00090 $ & $   9.16175 $ & $ i$\\
$ 55243.73522 $ & $   0.00141 $ & $   0.00090 $ & $   9.16219 $ & $ i$\\
$ 55243.73563 $ & $  -0.00298 $ & $   0.00090 $ & $   9.15802 $ & $ i$\\
$ 55243.73598 $ & $  -0.00061 $ & $   0.00090 $ & $   9.15849 $ & $ i$\\
$ 55243.73633 $ & $   0.00147 $ & $   0.00090 $ & $   9.16114 $ & $ i$\\
$ 55243.73670 $ & $   0.00075 $ & $   0.00090 $ & $   9.16156 $ & $ i$\\
$ 55243.73705 $ & $  -0.00192 $ & $   0.00090 $ & $   9.15928 $ & $ i$\\
$ 55243.73741 $ & $   0.00013 $ & $   0.00090 $ & $   9.16109 $ & $ i$\\
$ 55243.73777 $ & $   0.00033 $ & $   0.00090 $ & $   9.16127 $ & $ i$\\
$ 55243.73812 $ & $   0.00097 $ & $   0.00090 $ & $   9.16256 $ & $ i$\\
$ 55243.73847 $ & $   0.00066 $ & $   0.00090 $ & $   9.16087 $ & $ i$\\
$ 55243.73883 $ & $   0.00048 $ & $   0.00090 $ & $   9.16157 $ & $ i$\\
$ 55243.73918 $ & $  -0.00124 $ & $   0.00090 $ & $   9.15977 $ & $ i$\\
$ 55243.73957 $ & $   0.00103 $ & $   0.00090 $ & $   9.16084 $ & $ i$\\
$ 55243.73997 $ & $   0.00114 $ & $   0.00090 $ & $   9.16252 $ & $ i$\\
$ 55243.74033 $ & $  -0.00079 $ & $   0.00089 $ & $   9.15930 $ & $ i$\\
$ 55243.74068 $ & $  -0.00273 $ & $   0.00090 $ & $   9.15746 $ & $ i$\\
$ 55243.74105 $ & $  -0.00181 $ & $   0.00090 $ & $   9.15885 $ & $ i$\\
$ 55243.74144 $ & $   0.00128 $ & $   0.00090 $ & $   9.16300 $ & $ i$\\
$ 55243.74219 $ & $   0.00164 $ & $   0.00090 $ & $   9.16255 $ & $ i$\\
$ 55243.74254 $ & $  -0.00123 $ & $   0.00090 $ & $   9.15927 $ & $ i$\\
$ 55243.74289 $ & $   0.00287 $ & $   0.00090 $ & $   9.16258 $ & $ i$\\
$ 55243.74325 $ & $  -0.00310 $ & $   0.00089 $ & $   9.15633 $ & $ i$\\
$ 55243.74360 $ & $   0.00259 $ & $   0.00090 $ & $   9.16192 $ & $ i$\\
$ 55243.74395 $ & $   0.00165 $ & $   0.00090 $ & $   9.16236 $ & $ i$\\
$ 55243.74429 $ & $   0.00101 $ & $   0.00090 $ & $   9.16173 $ & $ i$\\
$ 55243.74464 $ & $   0.00235 $ & $   0.00090 $ & $   9.16369 $ & $ i$\\
$ 55243.74499 $ & $  -0.00053 $ & $   0.00090 $ & $   9.16049 $ & $ i$\\
$ 55243.74535 $ & $   0.00192 $ & $   0.00090 $ & $   9.16212 $ & $ i$\\
$ 55243.74570 $ & $   0.00142 $ & $   0.00090 $ & $   9.16244 $ & $ i$\\
$ 55243.74605 $ & $   0.00416 $ & $   0.00090 $ & $   9.16513 $ & $ i$\\
$ 55243.74640 $ & $   0.00198 $ & $   0.00090 $ & $   9.16380 $ & $ i$\\
$ 55243.74675 $ & $  -0.00001 $ & $   0.00090 $ & $   9.16180 $ & $ i$\\
$ 55243.74711 $ & $   0.00355 $ & $   0.00090 $ & $   9.16452 $ & $ i$\\
$ 55243.74747 $ & $   0.00639 $ & $   0.00090 $ & $   9.16833 $ & $ i$\\
$ 55243.74787 $ & $   0.00560 $ & $   0.00090 $ & $   9.16590 $ & $ i$\\
$ 55243.74827 $ & $   0.00455 $ & $   0.00090 $ & $   9.16548 $ & $ i$\\
$ 55243.74862 $ & $   0.00172 $ & $   0.00090 $ & $   9.16368 $ & $ i$\\
$ 55243.74899 $ & $   0.00652 $ & $   0.00090 $ & $   9.16738 $ & $ i$\\
$ 55243.74934 $ & $   0.00424 $ & $   0.00090 $ & $   9.16547 $ & $ i$\\
$ 55243.74971 $ & $   0.00177 $ & $   0.00090 $ & $   9.16268 $ & $ i$\\
$ 55243.75006 $ & $   0.00234 $ & $   0.00090 $ & $   9.16400 $ & $ i$\\
$ 55243.75042 $ & $   0.00698 $ & $   0.00090 $ & $   9.16705 $ & $ i$\\
$ 55243.75077 $ & $   0.00717 $ & $   0.00090 $ & $   9.16816 $ & $ i$\\
$ 55243.75154 $ & $   0.00603 $ & $   0.00090 $ & $   9.16762 $ & $ i$\\
$ 55243.75193 $ & $   0.00503 $ & $   0.00090 $ & $   9.16634 $ & $ i$\\
$ 55243.75229 $ & $   0.00615 $ & $   0.00090 $ & $   9.16747 $ & $ i$\\
$ 55243.75263 $ & $   0.00619 $ & $   0.00090 $ & $   9.16805 $ & $ i$\\
$ 55243.75302 $ & $   0.00940 $ & $   0.00090 $ & $   9.17080 $ & $ i$\\
$ 55243.75343 $ & $   0.00929 $ & $   0.00090 $ & $   9.16931 $ & $ i$\\
$ 55243.75378 $ & $   0.00695 $ & $   0.00090 $ & $   9.16888 $ & $ i$\\
$ 55243.75414 $ & $   0.00922 $ & $   0.00090 $ & $   9.16947 $ & $ i$\\
$ 55243.75448 $ & $   0.00488 $ & $   0.00090 $ & $   9.16353 $ & $ i$\\
$ 55243.75488 $ & $   0.01113 $ & $   0.00090 $ & $   9.17290 $ & $ i$\\
$ 55243.75529 $ & $   0.00658 $ & $   0.00090 $ & $   9.16655 $ & $ i$\\
$ 55243.75564 $ & $   0.01147 $ & $   0.00090 $ & $   9.17250 $ & $ i$\\
$ 55243.75600 $ & $   0.00935 $ & $   0.00090 $ & $   9.17009 $ & $ i$\\
$ 55243.75634 $ & $   0.01014 $ & $   0.00090 $ & $   9.16775 $ & $ i$\\
$ 55243.75673 $ & $   0.00984 $ & $   0.00090 $ & $   9.17055 $ & $ i$\\
$ 55243.75714 $ & $   0.00856 $ & $   0.00090 $ & $   9.16893 $ & $ i$\\
$ 55243.75749 $ & $   0.00851 $ & $   0.00090 $ & $   9.16801 $ & $ i$\\
$ 55243.75785 $ & $   0.00692 $ & $   0.00090 $ & $   9.16857 $ & $ i$\\
$ 55243.75820 $ & $   0.01170 $ & $   0.00090 $ & $   9.17361 $ & $ i$\\
$ 55243.75859 $ & $   0.01028 $ & $   0.00090 $ & $   9.16927 $ & $ i$\\
$ 55243.75898 $ & $   0.01171 $ & $   0.00090 $ & $   9.17223 $ & $ i$\\
$ 55243.75970 $ & $   0.00988 $ & $   0.00090 $ & $   9.17053 $ & $ i$\\
$ 55243.76005 $ & $   0.00786 $ & $   0.00090 $ & $   9.16910 $ & $ i$\\
$ 55243.76044 $ & $   0.01001 $ & $   0.00090 $ & $   9.17091 $ & $ i$\\
$ 55243.76083 $ & $   0.00835 $ & $   0.00090 $ & $   9.16725 $ & $ i$\\
$ 55243.76119 $ & $   0.01161 $ & $   0.00090 $ & $   9.17112 $ & $ i$\\
$ 55243.76156 $ & $   0.00898 $ & $   0.00090 $ & $   9.16950 $ & $ i$\\
$ 55243.76191 $ & $   0.00897 $ & $   0.00090 $ & $   9.16785 $ & $ i$\\
$ 55243.76226 $ & $   0.00963 $ & $   0.00090 $ & $   9.17164 $ & $ i$\\
$ 55243.76261 $ & $   0.00750 $ & $   0.00090 $ & $   9.16870 $ & $ i$\\
$ 55243.76296 $ & $   0.00720 $ & $   0.00090 $ & $   9.16713 $ & $ i$\\
$ 55243.76330 $ & $   0.01059 $ & $   0.00090 $ & $   9.16989 $ & $ i$\\
$ 55243.76410 $ & $   0.01503 $ & $   0.00090 $ & $   9.17447 $ & $ i$\\
$ 55243.76445 $ & $   0.00976 $ & $   0.00090 $ & $   9.17159 $ & $ i$\\
$ 55243.76481 $ & $   0.00960 $ & $   0.00090 $ & $   9.17058 $ & $ i$\\
$ 55243.76516 $ & $   0.01014 $ & $   0.00090 $ & $   9.17171 $ & $ i$\\
$ 55243.76551 $ & $   0.01358 $ & $   0.00090 $ & $   9.17348 $ & $ i$\\
$ 55243.76586 $ & $   0.00883 $ & $   0.00090 $ & $   9.16961 $ & $ i$\\
$ 55243.76621 $ & $   0.01161 $ & $   0.00090 $ & $   9.17139 $ & $ i$\\
$ 55243.76655 $ & $   0.01163 $ & $   0.00090 $ & $   9.17163 $ & $ i$\\
$ 55243.76690 $ & $   0.00919 $ & $   0.00090 $ & $   9.16911 $ & $ i$\\
$ 55243.76728 $ & $   0.01066 $ & $   0.00090 $ & $   9.17216 $ & $ i$\\
$ 55243.76769 $ & $   0.00931 $ & $   0.00090 $ & $   9.17071 $ & $ i$\\
$ 55243.76809 $ & $   0.00919 $ & $   0.00090 $ & $   9.17001 $ & $ i$\\
$ 55243.76844 $ & $   0.01250 $ & $   0.00090 $ & $   9.17274 $ & $ i$\\
$ 55243.76879 $ & $   0.01015 $ & $   0.00090 $ & $   9.17173 $ & $ i$\\
$ 55243.76949 $ & $   0.01014 $ & $   0.00090 $ & $   9.17153 $ & $ i$\\
$ 55243.76985 $ & $   0.00809 $ & $   0.00090 $ & $   9.16908 $ & $ i$\\
$ 55243.77020 $ & $   0.00796 $ & $   0.00090 $ & $   9.16925 $ & $ i$\\
$ 55243.77056 $ & $   0.01123 $ & $   0.00090 $ & $   9.17199 $ & $ i$\\
$ 55243.77092 $ & $   0.00934 $ & $   0.00090 $ & $   9.17100 $ & $ i$\\
$ 55243.77129 $ & $   0.01015 $ & $   0.00090 $ & $   9.17128 $ & $ i$\\
$ 55243.77164 $ & $   0.00962 $ & $   0.00090 $ & $   9.17146 $ & $ i$\\
$ 55243.77238 $ & $   0.01222 $ & $   0.00090 $ & $   9.17382 $ & $ i$\\
$ 55243.77277 $ & $   0.01386 $ & $   0.00090 $ & $   9.17568 $ & $ i$\\
$ 55243.77314 $ & $   0.01173 $ & $   0.00090 $ & $   9.17347 $ & $ i$\\
$ 55243.77349 $ & $   0.00971 $ & $   0.00090 $ & $   9.17154 $ & $ i$\\
$ 55243.77388 $ & $   0.01206 $ & $   0.00090 $ & $   9.17295 $ & $ i$\\
$ 55243.77428 $ & $   0.01078 $ & $   0.00090 $ & $   9.17301 $ & $ i$\\
$ 55243.77463 $ & $   0.01187 $ & $   0.00090 $ & $   9.17357 $ & $ i$\\
$ 55243.77571 $ & $   0.01223 $ & $   0.00090 $ & $   9.17328 $ & $ i$\\
$ 55243.77609 $ & $   0.01242 $ & $   0.00090 $ & $   9.17382 $ & $ i$\\
$ 55243.77649 $ & $   0.01071 $ & $   0.00090 $ & $   9.17246 $ & $ i$\\
$ 55243.77686 $ & $   0.01294 $ & $   0.00090 $ & $   9.17370 $ & $ i$\\
$ 55243.77721 $ & $   0.01155 $ & $   0.00090 $ & $   9.17268 $ & $ i$\\
$ 55243.77795 $ & $   0.00705 $ & $   0.00090 $ & $   9.16892 $ & $ i$\\
$ 55243.77835 $ & $   0.00819 $ & $   0.00090 $ & $   9.17017 $ & $ i$\\
$ 55243.77907 $ & $   0.01183 $ & $   0.00090 $ & $   9.17300 $ & $ i$\\
$ 55243.77942 $ & $   0.00999 $ & $   0.00090 $ & $   9.17142 $ & $ i$\\
$ 55243.77977 $ & $   0.01277 $ & $   0.00090 $ & $   9.17523 $ & $ i$\\
$ 55243.78013 $ & $   0.00938 $ & $   0.00090 $ & $   9.17057 $ & $ i$\\
$ 55243.78047 $ & $   0.01206 $ & $   0.00090 $ & $   9.17379 $ & $ i$\\
$ 55243.78082 $ & $   0.01343 $ & $   0.00090 $ & $   9.17576 $ & $ i$\\
$ 55243.78117 $ & $   0.00984 $ & $   0.00090 $ & $   9.17086 $ & $ i$\\
$ 55243.78155 $ & $   0.00965 $ & $   0.00090 $ & $   9.17022 $ & $ i$\\
$ 55243.78195 $ & $   0.01192 $ & $   0.00090 $ & $   9.17300 $ & $ i$\\
$ 55243.78231 $ & $   0.00941 $ & $   0.00090 $ & $   9.16761 $ & $ i$\\
$ 55243.78270 $ & $   0.00978 $ & $   0.00090 $ & $   9.17022 $ & $ i$\\
$ 55243.78309 $ & $   0.00821 $ & $   0.00090 $ & $   9.16879 $ & $ i$\\
$ 55243.78346 $ & $   0.01072 $ & $   0.00090 $ & $   9.17062 $ & $ i$\\
$ 55243.78385 $ & $   0.01126 $ & $   0.00090 $ & $   9.17346 $ & $ i$\\
$ 55243.78425 $ & $   0.01183 $ & $   0.00090 $ & $   9.17374 $ & $ i$\\
$ 55243.78460 $ & $   0.00763 $ & $   0.00090 $ & $   9.16884 $ & $ i$\\
$ 55243.78497 $ & $   0.01322 $ & $   0.00090 $ & $   9.17493 $ & $ i$\\
$ 55243.78532 $ & $   0.01081 $ & $   0.00090 $ & $   9.17198 $ & $ i$\\
$ 55243.78572 $ & $   0.01157 $ & $   0.00090 $ & $   9.17325 $ & $ i$\\
$ 55243.78683 $ & $   0.01207 $ & $   0.00090 $ & $   9.17331 $ & $ i$\\
$ 55243.78719 $ & $   0.01148 $ & $   0.00090 $ & $   9.17338 $ & $ i$\\
$ 55243.78757 $ & $   0.01285 $ & $   0.00090 $ & $   9.17487 $ & $ i$\\
$ 55243.78797 $ & $   0.00927 $ & $   0.00090 $ & $   9.17103 $ & $ i$\\
$ 55243.78833 $ & $   0.01197 $ & $   0.00090 $ & $   9.17464 $ & $ i$\\
$ 55243.78869 $ & $   0.01115 $ & $   0.00090 $ & $   9.17269 $ & $ i$\\
$ 55243.78904 $ & $   0.00926 $ & $   0.00090 $ & $   9.17160 $ & $ i$\\
$ 55243.78942 $ & $   0.01010 $ & $   0.00090 $ & $   9.17224 $ & $ i$\\
$ 55243.78982 $ & $   0.01093 $ & $   0.00090 $ & $   9.17278 $ & $ i$\\
$ 55243.79018 $ & $   0.01312 $ & $   0.00090 $ & $   9.17493 $ & $ i$\\
$ 55243.79058 $ & $   0.01039 $ & $   0.00090 $ & $   9.17029 $ & $ i$\\
$ 55243.79097 $ & $   0.01080 $ & $   0.00090 $ & $   9.17160 $ & $ i$\\
$ 55243.79133 $ & $   0.00863 $ & $   0.00090 $ & $   9.17020 $ & $ i$\\
$ 55243.79170 $ & $   0.01418 $ & $   0.00090 $ & $   9.17444 $ & $ i$\\
$ 55243.79205 $ & $   0.01293 $ & $   0.00090 $ & $   9.17497 $ & $ i$\\
$ 55243.79241 $ & $   0.01013 $ & $   0.00090 $ & $   9.17160 $ & $ i$\\
$ 55243.79276 $ & $   0.01146 $ & $   0.00090 $ & $   9.17210 $ & $ i$\\
$ 55243.79311 $ & $   0.01227 $ & $   0.00090 $ & $   9.17440 $ & $ i$\\
$ 55243.79346 $ & $   0.00869 $ & $   0.00090 $ & $   9.16991 $ & $ i$\\
$ 55243.79380 $ & $   0.00940 $ & $   0.00090 $ & $   9.17147 $ & $ i$\\
$ 55243.79416 $ & $   0.00967 $ & $   0.00090 $ & $   9.17108 $ & $ i$\\
$ 55243.79451 $ & $   0.01064 $ & $   0.00090 $ & $   9.17228 $ & $ i$\\
$ 55243.79486 $ & $   0.01081 $ & $   0.00090 $ & $   9.17330 $ & $ i$\\
$ 55243.79555 $ & $   0.01223 $ & $   0.00090 $ & $   9.17268 $ & $ i$\\
$ 55243.79590 $ & $   0.01084 $ & $   0.00090 $ & $   9.17211 $ & $ i$\\
$ 55243.79625 $ & $   0.01353 $ & $   0.00090 $ & $   9.17435 $ & $ i$\\
$ 55243.79659 $ & $   0.01121 $ & $   0.00090 $ & $   9.17284 $ & $ i$\\
$ 55243.79694 $ & $   0.01229 $ & $   0.00090 $ & $   9.17435 $ & $ i$\\
$ 55243.79733 $ & $   0.00940 $ & $   0.00090 $ & $   9.17175 $ & $ i$\\
$ 55243.79772 $ & $   0.01104 $ & $   0.00090 $ & $   9.17089 $ & $ i$\\
$ 55243.79808 $ & $   0.01273 $ & $   0.00090 $ & $   9.17249 $ & $ i$\\
$ 55243.79848 $ & $   0.00859 $ & $   0.00089 $ & $   9.16903 $ & $ i$\\
$ 55243.79887 $ & $   0.00906 $ & $   0.00090 $ & $   9.16833 $ & $ i$\\
$ 55243.79923 $ & $   0.00796 $ & $   0.00090 $ & $   9.16901 $ & $ i$\\
$ 55243.79959 $ & $   0.01291 $ & $   0.00090 $ & $   9.17327 $ & $ i$\\
$ 55243.80072 $ & $   0.01178 $ & $   0.00090 $ & $   9.17396 $ & $ i$\\
$ 55243.80108 $ & $   0.01068 $ & $   0.00090 $ & $   9.17130 $ & $ i$\\
$ 55243.80145 $ & $   0.00982 $ & $   0.00090 $ & $   9.17141 $ & $ i$\\
$ 55243.80180 $ & $   0.01253 $ & $   0.00090 $ & $   9.17455 $ & $ i$\\
$ 55243.80219 $ & $   0.01173 $ & $   0.00090 $ & $   9.17355 $ & $ i$\\
$ 55243.80258 $ & $   0.01316 $ & $   0.00090 $ & $   9.17538 $ & $ i$\\
$ 55243.80294 $ & $   0.01018 $ & $   0.00090 $ & $   9.17126 $ & $ i$\\
$ 55243.80331 $ & $   0.01285 $ & $   0.00090 $ & $   9.17601 $ & $ i$\\
$ 55243.80366 $ & $   0.01052 $ & $   0.00090 $ & $   9.17280 $ & $ i$\\
$ 55243.80401 $ & $   0.01341 $ & $   0.00090 $ & $   9.17537 $ & $ i$\\
$ 55243.80436 $ & $   0.01056 $ & $   0.00090 $ & $   9.17326 $ & $ i$\\
$ 55243.80471 $ & $   0.00922 $ & $   0.00090 $ & $   9.17159 $ & $ i$\\
$ 55243.80506 $ & $   0.01049 $ & $   0.00090 $ & $   9.17217 $ & $ i$\\
$ 55243.80540 $ & $   0.01067 $ & $   0.00090 $ & $   9.17189 $ & $ i$\\
$ 55243.80575 $ & $   0.00891 $ & $   0.00090 $ & $   9.16976 $ & $ i$\\
$ 55243.80610 $ & $   0.01162 $ & $   0.00090 $ & $   9.17283 $ & $ i$\\
$ 55243.80645 $ & $   0.01035 $ & $   0.00090 $ & $   9.17232 $ & $ i$\\
$ 55243.80679 $ & $   0.01213 $ & $   0.00090 $ & $   9.17252 $ & $ i$\\
$ 55243.80714 $ & $   0.00933 $ & $   0.00090 $ & $   9.16965 $ & $ i$\\
$ 55243.80749 $ & $   0.01271 $ & $   0.00090 $ & $   9.17478 $ & $ i$\\
$ 55243.80784 $ & $   0.01398 $ & $   0.00090 $ & $   9.17655 $ & $ i$\\
$ 55243.80819 $ & $   0.01431 $ & $   0.00090 $ & $   9.17669 $ & $ i$\\
$ 55243.80854 $ & $   0.01253 $ & $   0.00090 $ & $   9.17390 $ & $ i$\\
$ 55243.80888 $ & $   0.01013 $ & $   0.00090 $ & $   9.17295 $ & $ i$\\
$ 55243.80923 $ & $   0.01303 $ & $   0.00090 $ & $   9.17615 $ & $ i$\\
$ 55243.80958 $ & $   0.01142 $ & $   0.00090 $ & $   9.17343 $ & $ i$\\
$ 55243.80993 $ & $   0.01057 $ & $   0.00090 $ & $   9.17354 $ & $ i$\\
$ 55243.81027 $ & $   0.01141 $ & $   0.00090 $ & $   9.17328 $ & $ i$\\
$ 55243.81062 $ & $   0.01285 $ & $   0.00090 $ & $   9.17547 $ & $ i$\\
$ 55243.81097 $ & $   0.00975 $ & $   0.00090 $ & $   9.17286 $ & $ i$\\
$ 55243.81132 $ & $   0.00973 $ & $   0.00090 $ & $   9.17208 $ & $ i$\\
$ 55243.81167 $ & $   0.01071 $ & $   0.00090 $ & $   9.17196 $ & $ i$\\
$ 55243.81236 $ & $   0.01212 $ & $   0.00090 $ & $   9.17233 $ & $ i$\\
$ 55243.81271 $ & $   0.01112 $ & $   0.00090 $ & $   9.17275 $ & $ i$\\
$ 55243.81306 $ & $   0.00907 $ & $   0.00090 $ & $   9.17194 $ & $ i$\\
$ 55243.81340 $ & $   0.00833 $ & $   0.00090 $ & $   9.17110 $ & $ i$\\
$ 55243.81421 $ & $   0.01180 $ & $   0.00090 $ & $   9.17427 $ & $ i$\\
$ 55243.81457 $ & $   0.01227 $ & $   0.00090 $ & $   9.17571 $ & $ i$\\
$ 55243.81492 $ & $   0.01275 $ & $   0.00090 $ & $   9.17485 $ & $ i$\\
$ 55243.81526 $ & $   0.01310 $ & $   0.00090 $ & $   9.17519 $ & $ i$\\
$ 55243.81562 $ & $   0.00805 $ & $   0.00090 $ & $   9.17116 $ & $ i$\\
$ 55243.81631 $ & $   0.01216 $ & $   0.00090 $ & $   9.17474 $ & $ i$\\
$ 55243.81666 $ & $   0.01313 $ & $   0.00090 $ & $   9.17516 $ & $ i$\\
$ 55243.81700 $ & $   0.01078 $ & $   0.00090 $ & $   9.17334 $ & $ i$\\
$ 55243.81735 $ & $   0.01080 $ & $   0.00090 $ & $   9.17285 $ & $ i$\\
$ 55243.81770 $ & $   0.01301 $ & $   0.00090 $ & $   9.17522 $ & $ i$\\
$ 55243.81840 $ & $   0.01284 $ & $   0.00090 $ & $   9.17394 $ & $ i$\\
$ 55243.81875 $ & $   0.01116 $ & $   0.00090 $ & $   9.17400 $ & $ i$\\
$ 55243.81909 $ & $   0.01170 $ & $   0.00090 $ & $   9.17417 $ & $ i$\\
$ 55243.81944 $ & $   0.01030 $ & $   0.00090 $ & $   9.17272 $ & $ i$\\
$ 55243.82049 $ & $   0.00905 $ & $   0.00089 $ & $   9.17228 $ & $ i$\\
$ 55243.82118 $ & $   0.01042 $ & $   0.00090 $ & $   9.17324 $ & $ i$\\
$ 55243.82153 $ & $   0.01037 $ & $   0.00090 $ & $   9.17177 $ & $ i$\\
$ 55243.82188 $ & $   0.01009 $ & $   0.00090 $ & $   9.17151 $ & $ i$\\
$ 55243.82223 $ & $   0.01146 $ & $   0.00090 $ & $   9.17371 $ & $ i$\\
$ 55243.82257 $ & $   0.01132 $ & $   0.00090 $ & $   9.17350 $ & $ i$\\
$ 55243.82293 $ & $   0.01440 $ & $   0.00090 $ & $   9.17683 $ & $ i$\\
$ 55243.82327 $ & $   0.01248 $ & $   0.00089 $ & $   9.17536 $ & $ i$\\
$ 55243.82362 $ & $   0.01084 $ & $   0.00089 $ & $   9.17227 $ & $ i$\\
$ 55243.82397 $ & $   0.01317 $ & $   0.00090 $ & $   9.17576 $ & $ i$\\
$ 55243.82432 $ & $   0.00926 $ & $   0.00090 $ & $   9.16878 $ & $ i$\\
$ 55243.82466 $ & $   0.01118 $ & $   0.00090 $ & $   9.17333 $ & $ i$\\
$ 55243.82501 $ & $   0.01536 $ & $   0.00090 $ & $   9.17638 $ & $ i$\\
$ 55243.82536 $ & $   0.01149 $ & $   0.00090 $ & $   9.17213 $ & $ i$\\
$ 55243.82571 $ & $   0.01066 $ & $   0.00090 $ & $   9.17173 $ & $ i$\\
$ 55243.82606 $ & $   0.01363 $ & $   0.00090 $ & $   9.17519 $ & $ i$\\
$ 55243.82640 $ & $   0.01230 $ & $   0.00090 $ & $   9.17495 $ & $ i$\\
$ 55243.82675 $ & $   0.00843 $ & $   0.00090 $ & $   9.17097 $ & $ i$\\
$ 55243.82710 $ & $   0.01094 $ & $   0.00090 $ & $   9.17174 $ & $ i$\\
$ 55243.82744 $ & $   0.01123 $ & $   0.00090 $ & $   9.17341 $ & $ i$\\
$ 55243.82779 $ & $   0.01113 $ & $   0.00090 $ & $   9.17357 $ & $ i$\\
$ 55243.82814 $ & $   0.01131 $ & $   0.00090 $ & $   9.17454 $ & $ i$\\
$ 55243.82849 $ & $   0.01302 $ & $   0.00090 $ & $   9.17411 $ & $ i$\\
$ 55243.82884 $ & $   0.01536 $ & $   0.00090 $ & $   9.17721 $ & $ i$\\
$ 55243.82918 $ & $   0.01063 $ & $   0.00090 $ & $   9.17193 $ & $ i$\\
$ 55243.82988 $ & $   0.00973 $ & $   0.00090 $ & $   9.17256 $ & $ i$\\
$ 55243.83023 $ & $   0.01221 $ & $   0.00090 $ & $   9.17293 $ & $ i$\\
$ 55243.83058 $ & $   0.01205 $ & $   0.00090 $ & $   9.17413 $ & $ i$\\
$ 55243.83093 $ & $   0.01342 $ & $   0.00090 $ & $   9.17468 $ & $ i$\\
$ 55243.83128 $ & $   0.00971 $ & $   0.00090 $ & $   9.17230 $ & $ i$\\
$ 55243.83163 $ & $   0.01123 $ & $   0.00090 $ & $   9.17342 $ & $ i$\\
$ 55243.83197 $ & $   0.01298 $ & $   0.00090 $ & $   9.17641 $ & $ i$\\
$ 55243.83232 $ & $   0.00985 $ & $   0.00090 $ & $   9.17205 $ & $ i$\\
$ 55243.83267 $ & $   0.01123 $ & $   0.00090 $ & $   9.17414 $ & $ i$\\
$ 55243.83301 $ & $   0.01084 $ & $   0.00090 $ & $   9.17230 $ & $ i$\\
$ 55243.83336 $ & $   0.01131 $ & $   0.00090 $ & $   9.17332 $ & $ i$\\
$ 55243.83406 $ & $   0.01221 $ & $   0.00090 $ & $   9.17521 $ & $ i$\\
$ 55243.83440 $ & $   0.01340 $ & $   0.00090 $ & $   9.17481 $ & $ i$\\
$ 55243.83475 $ & $   0.01134 $ & $   0.00090 $ & $   9.17440 $ & $ i$\\
$ 55243.83510 $ & $   0.01208 $ & $   0.00090 $ & $   9.17485 $ & $ i$\\
$ 55243.83545 $ & $   0.01393 $ & $   0.00090 $ & $   9.17687 $ & $ i$\\
$ 55243.83579 $ & $   0.00972 $ & $   0.00090 $ & $   9.17274 $ & $ i$\\
$ 55243.83614 $ & $   0.01105 $ & $   0.00090 $ & $   9.17461 $ & $ i$\\
$ 55243.83649 $ & $   0.00975 $ & $   0.00090 $ & $   9.17313 $ & $ i$\\
$ 55243.83719 $ & $   0.01602 $ & $   0.00090 $ & $   9.17805 $ & $ i$\\
$ 55243.83754 $ & $   0.01364 $ & $   0.00090 $ & $   9.17580 $ & $ i$\\
$ 55243.83788 $ & $   0.00996 $ & $   0.00090 $ & $   9.17336 $ & $ i$\\
$ 55243.83823 $ & $   0.01178 $ & $   0.00090 $ & $   9.17352 $ & $ i$\\
$ 55243.83858 $ & $   0.01034 $ & $   0.00090 $ & $   9.17272 $ & $ i$\\
$ 55243.83893 $ & $   0.01177 $ & $   0.00090 $ & $   9.17382 $ & $ i$\\
$ 55243.83927 $ & $   0.01251 $ & $   0.00090 $ & $   9.17481 $ & $ i$\\
$ 55243.83962 $ & $   0.00961 $ & $   0.00090 $ & $   9.17175 $ & $ i$\\
$ 55243.83997 $ & $   0.01216 $ & $   0.00090 $ & $   9.17543 $ & $ i$\\
$ 55243.84032 $ & $   0.01558 $ & $   0.00090 $ & $   9.17857 $ & $ i$\\
$ 55243.84067 $ & $   0.01324 $ & $   0.00090 $ & $   9.17584 $ & $ i$\\
$ 55243.84138 $ & $   0.01601 $ & $   0.00090 $ & $   9.17864 $ & $ i$\\
$ 55243.84173 $ & $   0.00852 $ & $   0.00089 $ & $   9.16919 $ & $ i$\\
$ 55243.84247 $ & $   0.01031 $ & $   0.00089 $ & $   9.17272 $ & $ i$\\
$ 55243.84290 $ & $   0.01404 $ & $   0.00090 $ & $   9.17404 $ & $ i$\\
$ 55243.84325 $ & $   0.01364 $ & $   0.00090 $ & $   9.17607 $ & $ i$\\
$ 55243.84360 $ & $   0.01101 $ & $   0.00090 $ & $   9.17288 $ & $ i$\\
$ 55243.84395 $ & $   0.01163 $ & $   0.00089 $ & $   9.17407 $ & $ i$\\
$ 55243.84434 $ & $   0.00820 $ & $   0.00089 $ & $   9.17128 $ & $ i$\\
$ 55243.84475 $ & $   0.00972 $ & $   0.00090 $ & $   9.17263 $ & $ i$\\
$ 55243.84511 $ & $   0.01253 $ & $   0.00090 $ & $   9.17506 $ & $ i$\\
$ 55243.84546 $ & $   0.01268 $ & $   0.00090 $ & $   9.17574 $ & $ i$\\
$ 55243.84585 $ & $   0.01137 $ & $   0.00090 $ & $   9.17433 $ & $ i$\\
$ 55243.84626 $ & $   0.01051 $ & $   0.00090 $ & $   9.17306 $ & $ i$\\
$ 55243.84661 $ & $   0.01035 $ & $   0.00090 $ & $   9.17268 $ & $ i$\\
$ 55243.84697 $ & $   0.01532 $ & $   0.00090 $ & $   9.17795 $ & $ i$\\
$ 55243.84732 $ & $   0.00989 $ & $   0.00090 $ & $   9.17312 $ & $ i$\\
$ 55243.84767 $ & $   0.01063 $ & $   0.00090 $ & $   9.17368 $ & $ i$\\
$ 55243.84802 $ & $   0.01208 $ & $   0.00090 $ & $   9.17514 $ & $ i$\\
$ 55243.84837 $ & $   0.01214 $ & $   0.00090 $ & $   9.17568 $ & $ i$\\
$ 55243.84872 $ & $   0.01048 $ & $   0.00090 $ & $   9.17244 $ & $ i$\\
$ 55243.84906 $ & $   0.00870 $ & $   0.00090 $ & $   9.17143 $ & $ i$\\
$ 55243.84941 $ & $   0.01238 $ & $   0.00090 $ & $   9.17560 $ & $ i$\\
$ 55243.84976 $ & $   0.01188 $ & $   0.00090 $ & $   9.17510 $ & $ i$\\
$ 55243.85011 $ & $   0.01175 $ & $   0.00090 $ & $   9.17437 $ & $ i$\\
$ 55243.85046 $ & $   0.01134 $ & $   0.00090 $ & $   9.17512 $ & $ i$\\
$ 55243.85081 $ & $   0.01175 $ & $   0.00089 $ & $   9.17394 $ & $ i$\\
$ 55243.85115 $ & $   0.01222 $ & $   0.00090 $ & $   9.17441 $ & $ i$\\
$ 55243.85150 $ & $   0.01104 $ & $   0.00090 $ & $   9.17429 $ & $ i$\\
$ 55243.85185 $ & $   0.00685 $ & $   0.00090 $ & $   9.17042 $ & $ i$\\
$ 55243.85220 $ & $   0.01285 $ & $   0.00090 $ & $   9.17573 $ & $ i$\\
$ 55243.85255 $ & $   0.01247 $ & $   0.00090 $ & $   9.17626 $ & $ i$\\
$ 55243.85289 $ & $   0.00855 $ & $   0.00090 $ & $   9.17211 $ & $ i$\\
$ 55243.85324 $ & $   0.01094 $ & $   0.00090 $ & $   9.17346 $ & $ i$\\
$ 55243.85359 $ & $   0.01337 $ & $   0.00090 $ & $   9.17675 $ & $ i$\\
$ 55243.85394 $ & $   0.00983 $ & $   0.00090 $ & $   9.17285 $ & $ i$\\
$ 55243.85463 $ & $   0.01024 $ & $   0.00090 $ & $   9.17342 $ & $ i$\\
$ 55243.85498 $ & $   0.00927 $ & $   0.00090 $ & $   9.17224 $ & $ i$\\
$ 55243.85533 $ & $   0.00964 $ & $   0.00090 $ & $   9.17273 $ & $ i$\\
$ 55243.85568 $ & $   0.01056 $ & $   0.00090 $ & $   9.17372 $ & $ i$\\
$ 55243.85602 $ & $   0.00821 $ & $   0.00090 $ & $   9.17184 $ & $ i$\\
$ 55243.85637 $ & $   0.00920 $ & $   0.00090 $ & $   9.17246 $ & $ i$\\
$ 55243.85672 $ & $   0.01283 $ & $   0.00090 $ & $   9.17657 $ & $ i$\\
$ 55243.85707 $ & $   0.01030 $ & $   0.00090 $ & $   9.17272 $ & $ i$\\
$ 55243.85742 $ & $   0.01021 $ & $   0.00090 $ & $   9.17327 $ & $ i$\\
$ 55243.85776 $ & $   0.01111 $ & $   0.00090 $ & $   9.17297 $ & $ i$\\
$ 55243.85846 $ & $   0.01240 $ & $   0.00090 $ & $   9.17550 $ & $ i$\\
$ 55243.85881 $ & $   0.01254 $ & $   0.00090 $ & $   9.17546 $ & $ i$\\
$ 55243.85916 $ & $   0.00826 $ & $   0.00090 $ & $   9.17106 $ & $ i$\\
$ 55243.85951 $ & $   0.01186 $ & $   0.00090 $ & $   9.17530 $ & $ i$\\
$ 55243.85986 $ & $   0.01445 $ & $   0.00090 $ & $   9.17728 $ & $ i$\\
$ 55243.86055 $ & $   0.01207 $ & $   0.00090 $ & $   9.17506 $ & $ i$\\
$ 55243.86090 $ & $   0.01032 $ & $   0.00090 $ & $   9.17299 $ & $ i$\\
$ 55243.86125 $ & $   0.01222 $ & $   0.00090 $ & $   9.17541 $ & $ i$\\
$ 55243.86159 $ & $   0.01105 $ & $   0.00090 $ & $   9.17411 $ & $ i$\\
$ 55243.86194 $ & $   0.01078 $ & $   0.00090 $ & $   9.17336 $ & $ i$\\
$ 55243.86264 $ & $   0.01518 $ & $   0.00090 $ & $   9.17780 $ & $ i$\\
$ 55243.86298 $ & $   0.01056 $ & $   0.00090 $ & $   9.17227 $ & $ i$\\
$ 55243.86333 $ & $   0.01225 $ & $   0.00090 $ & $   9.17465 $ & $ i$\\
$ 55243.86438 $ & $   0.01168 $ & $   0.00089 $ & $   9.17522 $ & $ i$\\
$ 55243.86473 $ & $   0.01323 $ & $   0.00090 $ & $   9.17632 $ & $ i$\\
$ 55243.86507 $ & $   0.01130 $ & $   0.00090 $ & $   9.17370 $ & $ i$\\
$ 55243.86577 $ & $   0.01098 $ & $   0.00090 $ & $   9.17329 $ & $ i$\\
$ 55243.86612 $ & $   0.01179 $ & $   0.00090 $ & $   9.17416 $ & $ i$\\
$ 55243.86646 $ & $   0.00989 $ & $   0.00090 $ & $   9.17300 $ & $ i$\\
$ 55243.86681 $ & $   0.01062 $ & $   0.00090 $ & $   9.17381 $ & $ i$\\
$ 55243.86716 $ & $   0.01259 $ & $   0.00090 $ & $   9.17526 $ & $ i$\\
$ 55243.86751 $ & $   0.01041 $ & $   0.00090 $ & $   9.17415 $ & $ i$\\
$ 55243.86786 $ & $   0.01178 $ & $   0.00090 $ & $   9.17430 $ & $ i$\\
$ 55243.86820 $ & $   0.01094 $ & $   0.00090 $ & $   9.17437 $ & $ i$\\
$ 55243.86855 $ & $   0.01119 $ & $   0.00090 $ & $   9.17406 $ & $ i$\\
$ 55243.86890 $ & $   0.00939 $ & $   0.00090 $ & $   9.17249 $ & $ i$\\
$ 55243.86960 $ & $   0.01168 $ & $   0.00090 $ & $   9.17455 $ & $ i$\\
$ 55243.86995 $ & $   0.01327 $ & $   0.00090 $ & $   9.17635 $ & $ i$\\
$ 55243.87064 $ & $   0.01195 $ & $   0.00090 $ & $   9.17517 $ & $ i$\\
$ 55243.87168 $ & $   0.01064 $ & $   0.00090 $ & $   9.17302 $ & $ i$\\
$ 55243.87203 $ & $   0.01301 $ & $   0.00090 $ & $   9.17596 $ & $ i$\\
$ 55243.87238 $ & $   0.01062 $ & $   0.00090 $ & $   9.17373 $ & $ i$\\
$ 55243.87273 $ & $   0.00953 $ & $   0.00090 $ & $   9.17382 $ & $ i$\\
$ 55243.87307 $ & $   0.01105 $ & $   0.00090 $ & $   9.17422 $ & $ i$\\
$ 55243.87377 $ & $   0.01030 $ & $   0.00089 $ & $   9.17269 $ & $ i$\\
$ 55243.87412 $ & $   0.01278 $ & $   0.00090 $ & $   9.17504 $ & $ i$\\
$ 55243.87447 $ & $   0.00885 $ & $   0.00090 $ & $   9.17105 $ & $ i$\\
$ 55243.87551 $ & $   0.01327 $ & $   0.00090 $ & $   9.17443 $ & $ i$\\
$ 55243.87586 $ & $   0.00922 $ & $   0.00089 $ & $   9.17095 $ & $ i$\\
$ 55243.87656 $ & $   0.00596 $ & $   0.00089 $ & $   9.16877 $ & $ i$\\
$ 55243.87726 $ & $   0.01076 $ & $   0.00090 $ & $   9.17320 $ & $ i$\\
$ 55243.87760 $ & $   0.00822 $ & $   0.00090 $ & $   9.17114 $ & $ i$\\
$ 55243.87795 $ & $   0.01060 $ & $   0.00090 $ & $   9.17424 $ & $ i$\\
$ 55243.87830 $ & $   0.01094 $ & $   0.00090 $ & $   9.17408 $ & $ i$\\
$ 55243.87865 $ & $   0.01182 $ & $   0.00090 $ & $   9.17390 $ & $ i$\\
$ 55243.87900 $ & $   0.01160 $ & $   0.00089 $ & $   9.17377 $ & $ i$\\
$ 55243.87934 $ & $   0.01131 $ & $   0.00090 $ & $   9.17274 $ & $ i$\\
$ 55243.87969 $ & $   0.01167 $ & $   0.00090 $ & $   9.17398 $ & $ i$\\
$ 55243.88004 $ & $   0.01034 $ & $   0.00090 $ & $   9.17396 $ & $ i$\\
$ 55243.88039 $ & $   0.01225 $ & $   0.00090 $ & $   9.17529 $ & $ i$\\
$ 55243.88074 $ & $   0.01124 $ & $   0.00090 $ & $   9.17346 $ & $ i$\\
$ 55243.88108 $ & $   0.00476 $ & $   0.00090 $ & $   9.16632 $ & $ i$\\
$ 55243.88143 $ & $   0.00893 $ & $   0.00090 $ & $   9.17217 $ & $ i$\\
$ 55243.88213 $ & $   0.00726 $ & $   0.00090 $ & $   9.17056 $ & $ i$\\
$ 55243.88247 $ & $   0.01231 $ & $   0.00090 $ & $   9.17486 $ & $ i$\\
$ 55243.88282 $ & $   0.00987 $ & $   0.00090 $ & $   9.17184 $ & $ i$\\
$ 55243.88317 $ & $   0.00793 $ & $   0.00090 $ & $   9.17065 $ & $ i$\\
$ 55243.88352 $ & $   0.00928 $ & $   0.00089 $ & $   9.17187 $ & $ i$\\
$ 55243.88387 $ & $   0.00867 $ & $   0.00090 $ & $   9.17147 $ & $ i$\\
$ 55243.88422 $ & $   0.00755 $ & $   0.00090 $ & $   9.17026 $ & $ i$\\
$ 55243.88456 $ & $   0.00870 $ & $   0.00090 $ & $   9.17176 $ & $ i$\\
$ 55243.88491 $ & $   0.00931 $ & $   0.00090 $ & $   9.17196 $ & $ i$\\
$ 55243.88526 $ & $   0.00589 $ & $   0.00089 $ & $   9.16747 $ & $ i$\\
$ 55243.88561 $ & $   0.00816 $ & $   0.00089 $ & $   9.16938 $ & $ i$\\
$ 55243.88596 $ & $   0.00459 $ & $   0.00089 $ & $   9.16734 $ & $ i$\\
$ 55243.88630 $ & $   0.00535 $ & $   0.00089 $ & $   9.16848 $ & $ i$\\
$ 55243.88665 $ & $   0.00680 $ & $   0.00090 $ & $   9.16980 $ & $ i$\\
$ 55243.88700 $ & $   0.00572 $ & $   0.00089 $ & $   9.16813 $ & $ i$\\
$ 55243.88735 $ & $   0.00500 $ & $   0.00089 $ & $   9.16773 $ & $ i$\\
$ 55243.88770 $ & $   0.00462 $ & $   0.00089 $ & $   9.16657 $ & $ i$\\
$ 55243.88805 $ & $   0.00228 $ & $   0.00089 $ & $   9.16397 $ & $ i$\\
$ 55243.88840 $ & $   0.00275 $ & $   0.00089 $ & $   9.16583 $ & $ i$\\
$ 55243.88874 $ & $   0.00643 $ & $   0.00089 $ & $   9.16896 $ & $ i$\\
$ 55243.88909 $ & $   0.00692 $ & $   0.00089 $ & $   9.16977 $ & $ i$\\
$ 55243.88944 $ & $   0.00415 $ & $   0.00090 $ & $   9.16746 $ & $ i$\\
$ 55243.88979 $ & $   0.00330 $ & $   0.00089 $ & $   9.16689 $ & $ i$\\
$ 55243.89013 $ & $   0.00101 $ & $   0.00089 $ & $   9.16325 $ & $ i$\\
$ 55243.89048 $ & $   0.00250 $ & $   0.00089 $ & $   9.16552 $ & $ i$\\
$ 55243.89118 $ & $   0.00240 $ & $   0.00089 $ & $   9.16514 $ & $ i$\\
$ 55243.89153 $ & $   0.00149 $ & $   0.00089 $ & $   9.16440 $ & $ i$\\
$ 55243.89187 $ & $   0.00368 $ & $   0.00089 $ & $   9.16684 $ & $ i$\\
$ 55243.89222 $ & $  -0.00188 $ & $   0.00089 $ & $   9.16009 $ & $ i$\\
$ 55243.89256 $ & $   0.00304 $ & $   0.00089 $ & $   9.16584 $ & $ i$\\
$ 55243.89291 $ & $   0.00019 $ & $   0.00089 $ & $   9.16319 $ & $ i$\\
$ 55243.89326 $ & $  -0.00094 $ & $   0.00089 $ & $   9.16139 $ & $ i$\\
$ 55243.89361 $ & $  -0.00282 $ & $   0.00090 $ & $   9.15811 $ & $ i$\\
$ 55243.89430 $ & $  -0.00078 $ & $   0.00089 $ & $   9.16271 $ & $ i$\\
$ 55243.89466 $ & $   0.00153 $ & $   0.00089 $ & $   9.16320 $ & $ i$\\
$ 55243.89501 $ & $   0.00177 $ & $   0.00089 $ & $   9.16428 $ & $ i$\\
$ 55243.89535 $ & $  -0.00087 $ & $   0.00089 $ & $   9.16246 $ & $ i$\\
$ 55243.89570 $ & $   0.00065 $ & $   0.00089 $ & $   9.16412 $ & $ i$\\
$ 55243.89604 $ & $   0.00043 $ & $   0.00089 $ & $   9.16329 $ & $ i$\\
$ 55243.89639 $ & $   0.00053 $ & $   0.00089 $ & $   9.16323 $ & $ i$\\
$ 55243.89674 $ & $   0.00154 $ & $   0.00089 $ & $   9.16380 $ & $ i$\\
$ 55243.89709 $ & $   0.00232 $ & $   0.00089 $ & $   9.16475 $ & $ i$\\
$ 55243.89744 $ & $  -0.00230 $ & $   0.00089 $ & $   9.16053 $ & $ i$\\
$ 55243.89778 $ & $   0.00068 $ & $   0.00089 $ & $   9.16412 $ & $ i$\\
$ 55243.89883 $ & $   0.00394 $ & $   0.00089 $ & $   9.16636 $ & $ i$\\
$ 55243.89918 $ & $  -0.00127 $ & $   0.00089 $ & $   9.16175 $ & $ i$\\
$ 55243.89952 $ & $   0.00186 $ & $   0.00089 $ & $   9.16435 $ & $ i$\\
$ 55243.89987 $ & $  -0.00073 $ & $   0.00090 $ & $   9.16217 $ & $ i$\\
$ 55243.90022 $ & $  -0.00073 $ & $   0.00090 $ & $   9.16263 $ & $ i$\\
$ 55243.90057 $ & $   0.00001 $ & $   0.00089 $ & $   9.16317 $ & $ i$\\
$ 55243.90092 $ & $   0.00291 $ & $   0.00090 $ & $   9.16527 $ & $ i$\\
$ 55243.90126 $ & $  -0.00124 $ & $   0.00089 $ & $   9.16166 $ & $ i$\\
$ 55243.90161 $ & $   0.00007 $ & $   0.00090 $ & $   9.16282 $ & $ i$\\
$ 55243.90196 $ & $  -0.00271 $ & $   0.00089 $ & $   9.15968 $ & $ i$\\
$ 55243.90231 $ & $  -0.00059 $ & $   0.00089 $ & $   9.16187 $ & $ i$\\
$ 55243.90266 $ & $  -0.00011 $ & $   0.00089 $ & $   9.16271 $ & $ i$\\
$ 55243.90300 $ & $   0.00115 $ & $   0.00089 $ & $   9.16286 $ & $ i$\\
$ 55243.90335 $ & $   0.00172 $ & $   0.00090 $ & $   9.16487 $ & $ i$\\
$ 55243.90370 $ & $   0.00039 $ & $   0.00089 $ & $   9.16375 $ & $ i$\\
$ 55243.90405 $ & $   0.00119 $ & $   0.00089 $ & $   9.16459 $ & $ i$\\
$ 55243.90440 $ & $  -0.00055 $ & $   0.00089 $ & $   9.16198 $ & $ i$\\
$ 55243.90474 $ & $  -0.00192 $ & $   0.00089 $ & $   9.16079 $ & $ i$\\
$ 55243.90510 $ & $   0.00081 $ & $   0.00089 $ & $   9.16284 $ & $ i$\\
$ 55243.90580 $ & $  -0.00055 $ & $   0.00089 $ & $   9.15897 $ & $ i$\\
$ 55243.90614 $ & $  -0.00077 $ & $   0.00089 $ & $   9.15898 $ & $ i$\\
$ 55243.90649 $ & $   0.00019 $ & $   0.00089 $ & $   9.16351 $ & $ i$\\
$ 55243.90719 $ & $  -0.00164 $ & $   0.00089 $ & $   9.16048 $ & $ i$\\
$ 55243.90788 $ & $   0.00026 $ & $   0.00089 $ & $   9.16232 $ & $ i$\\
$ 55243.90823 $ & $  -0.00118 $ & $   0.00089 $ & $   9.15942 $ & $ i$\\
$ 55243.90858 $ & $   0.00098 $ & $   0.00089 $ & $   9.16297 $ & $ i$\\
$ 55243.90892 $ & $   0.00163 $ & $   0.00089 $ & $   9.16296 $ & $ i$\\
$ 55243.90927 $ & $   0.00314 $ & $   0.00089 $ & $   9.16620 $ & $ i$\\
$ 55243.90962 $ & $   0.00063 $ & $   0.00089 $ & $   9.16346 $ & $ i$\\
$ 55243.90997 $ & $  -0.00111 $ & $   0.00089 $ & $   9.15974 $ & $ i$\\
$ 55243.91032 $ & $  -0.00134 $ & $   0.00089 $ & $   9.15792 $ & $ i$\\
$ 55243.91066 $ & $  -0.00039 $ & $   0.00089 $ & $   9.15889 $ & $ i$\\
$ 55243.91101 $ & $  -0.00269 $ & $   0.00089 $ & $   9.15996 $ & $ i$\\
$ 55243.91136 $ & $  -0.00121 $ & $   0.00089 $ & $   9.16016 $ & $ i$\\
$ 55243.91170 $ & $  -0.00027 $ & $   0.00089 $ & $   9.16155 $ & $ i$\\
$ 55243.91206 $ & $  -0.00171 $ & $   0.00089 $ & $   9.15913 $ & $ i$\\
$ 55243.91240 $ & $  -0.00129 $ & $   0.00089 $ & $   9.16178 $ & $ i$\\
$ 55243.91310 $ & $  -0.00206 $ & $   0.00089 $ & $   9.16004 $ & $ i$\\
$ 55243.91345 $ & $   0.00197 $ & $   0.00089 $ & $   9.16446 $ & $ i$\\
$ 55243.91380 $ & $   0.00009 $ & $   0.00089 $ & $   9.16226 $ & $ i$\\
$ 55243.91415 $ & $  -0.00093 $ & $   0.00089 $ & $   9.15755 $ & $ i$\\
$ 55243.91449 $ & $  -0.00155 $ & $   0.00089 $ & $   9.15958 $ & $ i$\\
$ 55243.91519 $ & $   0.00038 $ & $   0.00089 $ & $   9.16197 $ & $ i$\\
$ 55243.91554 $ & $   0.00079 $ & $   0.00089 $ & $   9.16273 $ & $ i$\\
$ 55243.91588 $ & $  -0.00140 $ & $   0.00089 $ & $   9.16034 $ & $ i$\\
$ 55243.91623 $ & $   0.00054 $ & $   0.00089 $ & $   9.15999 $ & $ i$\\
$ 55243.91693 $ & $  -0.00241 $ & $   0.00089 $ & $   9.15821 $ & $ i$\\
$ 55243.91728 $ & $   0.00141 $ & $   0.00089 $ & $   9.16217 $ & $ i$\\
$ 55243.91762 $ & $  -0.00088 $ & $   0.00089 $ & $   9.16018 $ & $ i$\\
$ 55243.91797 $ & $   0.00270 $ & $   0.00089 $ & $   9.16481 $ & $ i$\\
$ 55243.91831 $ & $   0.00213 $ & $   0.00089 $ & $   9.16497 $ & $ i$\\
$ 55243.91867 $ & $  -0.00258 $ & $   0.00089 $ & $   9.15752 $ & $ i$\\
$ 55243.91902 $ & $   0.00181 $ & $   0.00089 $ & $   9.16372 $ & $ i$\\
$ 55243.91936 $ & $  -0.00353 $ & $   0.00089 $ & $   9.15505 $ & $ i$\\
$ 55243.91971 $ & $  -0.00066 $ & $   0.00089 $ & $   9.15903 $ & $ i$\\
$ 55243.92005 $ & $  -0.00351 $ & $   0.00089 $ & $   9.15899 $ & $ i$\\
$ 55243.92044 $ & $  -0.00315 $ & $   0.00090 $ & $   9.15960 $ & $ i$\\
$ 55243.92085 $ & $   0.00048 $ & $   0.00090 $ & $   9.16121 $ & $ i$\\
$ 55243.92124 $ & $  -0.00138 $ & $   0.00089 $ & $   9.16034 $ & $ i$\\
$ 55243.92168 $ & $   0.00144 $ & $   0.00090 $ & $   9.16304 $ & $ i$\\
$ 55243.92203 $ & $   0.00236 $ & $   0.00089 $ & $   9.16424 $ & $ i$\\
$ 55243.92238 $ & $  -0.00013 $ & $   0.00089 $ & $   9.16302 $ & $ i$\\
$ 55243.92273 $ & $  -0.00226 $ & $   0.00089 $ & $   9.15943 $ & $ i$\\
$ 55243.92308 $ & $  -0.00069 $ & $   0.00090 $ & $   9.16146 $ & $ i$\\
$ 55243.92342 $ & $  -0.00159 $ & $   0.00089 $ & $   9.15839 $ & $ i$\\
$ 55243.92377 $ & $   0.00080 $ & $   0.00089 $ & $   9.15932 $ & $ i$\\
$ 55243.92412 $ & $   0.00302 $ & $   0.00089 $ & $   9.16278 $ & $ i$\\
$ 55243.92447 $ & $  -0.00069 $ & $   0.00089 $ & $   9.16151 $ & $ i$\\
$ 55243.92482 $ & $   0.00132 $ & $   0.00089 $ & $   9.16261 $ & $ i$\\
$ 55243.92516 $ & $   0.00209 $ & $   0.00089 $ & $   9.16321 $ & $ i$\\
$ 55243.92551 $ & $   0.00153 $ & $   0.00089 $ & $   9.16352 $ & $ i$\\
$ 55243.92586 $ & $   0.00300 $ & $   0.00090 $ & $   9.16486 $ & $ i$\\
$ 55243.92621 $ & $  -0.00220 $ & $   0.00089 $ & $   9.15963 $ & $ i$\\
$ 55243.92656 $ & $   0.00013 $ & $   0.00090 $ & $   9.16287 $ & $ i$\\
$ 55243.92691 $ & $  -0.00140 $ & $   0.00089 $ & $   9.16031 $ & $ i$\\
$ 55243.92725 $ & $   0.00134 $ & $   0.00089 $ & $   9.16406 $ & $ i$\\
$ 55243.92761 $ & $   0.00038 $ & $   0.00089 $ & $   9.16224 $ & $ i$\\
$ 55243.92795 $ & $   0.00014 $ & $   0.00089 $ & $   9.16081 $ & $ i$\\
$ 55243.92830 $ & $   0.00006 $ & $   0.00089 $ & $   9.16137 $ & $ i$\\
$ 55243.92865 $ & $   0.00017 $ & $   0.00089 $ & $   9.15672 $ & $ i$\\
$ 55243.92899 $ & $  -0.00028 $ & $   0.00089 $ & $   9.16133 $ & $ i$\\
$ 55243.92934 $ & $   0.00022 $ & $   0.00089 $ & $   9.16278 $ & $ i$\\
$ 55243.92969 $ & $  -0.00355 $ & $   0.00089 $ & $   9.15456 $ & $ i$\\
$ 55243.93004 $ & $   0.00147 $ & $   0.00090 $ & $   9.16332 $ & $ i$\\
$ 55243.93039 $ & $  -0.00104 $ & $   0.00090 $ & $   9.15992 $ & $ i$\\
$ 55243.93074 $ & $  -0.00183 $ & $   0.00089 $ & $   9.15745 $ & $ i$\\
$ 55243.93109 $ & $   0.00177 $ & $   0.00089 $ & $   9.16263 $ & $ i$\\
$ 55243.93143 $ & $   0.00026 $ & $   0.00089 $ & $   9.15944 $ & $ i$\\
$ 55243.93178 $ & $  -0.00123 $ & $   0.00089 $ & $   9.16038 $ & $ i$\\
$ 55243.93213 $ & $   0.00181 $ & $   0.00089 $ & $   9.15824 $ & $ i$\\
$ 55243.93248 $ & $  -0.00416 $ & $   0.00089 $ & $   9.15386 $ & $ i$\\
$ 55243.93283 $ & $   0.00128 $ & $   0.00090 $ & $   9.16201 $ & $ i$\\
$ 55243.93317 $ & $  -0.00028 $ & $   0.00089 $ & $   9.16002 $ & $ i$\\
$ 55243.93352 $ & $   0.00134 $ & $   0.00089 $ & $   9.16219 $ & $ i$\\
$ 55243.93387 $ & $  -0.00002 $ & $   0.00089 $ & $   9.16148 $ & $ i$\\
$ 55243.93457 $ & $   0.00184 $ & $   0.00090 $ & $   9.16374 $ & $ i$\\
$ 55243.93491 $ & $  -0.00360 $ & $   0.00089 $ & $   9.15611 $ & $ i$\\
$ 55243.93526 $ & $   0.00194 $ & $   0.00090 $ & $   9.16327 $ & $ i$\\
$ 55243.93561 $ & $   0.00166 $ & $   0.00089 $ & $   9.16440 $ & $ i$\\
$ 55243.93596 $ & $  -0.00143 $ & $   0.00089 $ & $   9.16006 $ & $ i$\\
$ 55243.93631 $ & $  -0.00422 $ & $   0.00089 $ & $   9.15233 $ & $ i$\\
$ 55243.93666 $ & $   0.00231 $ & $   0.00089 $ & $   9.16146 $ & $ i$\\
$ 55243.93700 $ & $  -0.00107 $ & $   0.00089 $ & $   9.15973 $ & $ i$\\
$ 55243.93735 $ & $  -0.00474 $ & $   0.00089 $ & $   9.15330 $ & $ i$\\
$ 55243.93769 $ & $   0.00122 $ & $   0.00089 $ & $   9.16178 $ & $ i$\\
$ 55243.93805 $ & $   0.00077 $ & $   0.00090 $ & $   9.16330 $ & $ i$\\


==> phfu_tab_short0.tex <==
$ 55206.63289 $ & $  -0.00145 $ & $   0.00176 $ & $  10.80170 $ & $ i$\\
$ 55206.63724 $ & $   0.00220 $ & $   0.00181 $ & $  10.80640 $ & $ i$\\
$ 55206.63790 $ & $  -0.00278 $ & $   0.00173 $ & $  10.80040 $ & $ i$\\
$ 55206.64440 $ & $  -0.00213 $ & $   0.00174 $ & $  10.80220 $ & $ i$\\
$ 55206.64485 $ & $   0.00093 $ & $   0.00171 $ & $  10.80450 $ & $ i$\\
$ 55206.64548 $ & $  -0.00051 $ & $   0.00161 $ & $  10.80300 $ & $ i$\\
$ 55206.64594 $ & $   0.00535 $ & $   0.00161 $ & $  10.80670 $ & $ i$\\
$ 55206.64659 $ & $  -0.00391 $ & $   0.00141 $ & $  10.80170 $ & $ i$\\
$ 55206.64703 $ & $   0.00162 $ & $   0.00140 $ & $  10.80520 $ & $ i$\\
$ 55206.64767 $ & $  -0.00023 $ & $   0.00134 $ & $  10.80330 $ & $ i$\\

